TRUST-TECH based Methods for Optimization and Learning

Many problems that arise in machine learning domain deal with nonlinearity and quite often demand users to obtain global optimal solutions rather than local optimal ones. Optimization problems are inherent in machine learning algorithms and hence many methods in machine learning were inherited from the optimization literature. Popularly known as the initialization problem, the ideal set of parameters required will significantly depend on the given initialization values. The recently developed TRUST-TECH (TRansformation Under STability-reTaining Equilibria CHaracterization) methodology systematically explores the subspace of the parameters to obtain a complete set of local optimal solutions. In this thesis work, we propose TRUST-TECH based methods for solving several optimization and machine learning problems. Two stages namely, the local stage and the neighborhood-search stage, are repeated alternatively in the solution space to achieve improvements in the quality of the solutions. Our methods were tested on both synthetic and real datasets and the advantages of using this novel framework are clearly manifested. This framework not only reduces the sensitivity to initialization, but also allows the flexibility for the practitioners to use various global and local methods that work well for a particular problem of interest. Other hierarchical stochastic algorithms like evolutionary algorithms and smoothing algorithms are also studied and frameworks for combining these methods with TRUST-TECH have been proposed and evaluated on several test systems.

==> orig/README <==
This package provides a "style file" for producing Ph.D. dissertations
at Cornell University using the new version of LaTeX, LaTeX 2e
which is now the only officially supported one. (If you haven't
upgraded to it yet, this file won't be of much use to you. Consider
upgrading.)

The distribution contains two files:
cornell.dtx -- self-documenting LaTeX source code for the style file.
cornell.ins -- installation "script" for the docstrip package.

To install, you need to say "latex cornell.ins", then move the resulting
cornell.cls file somewhere where latex will find it.

Detailed (albeit still incomplete in places) documentation can be generated
by saying "latex cornell.dtx" (probably twice, since there is a table of
contents).

This style file does not have official status: I just happen to have
typeset my thesis with the new LateX 2e, using this style file, and
the thesis secretary seemed fairly pleased with the result. I am making
it available in the hope that the horror stories about people's encounters
with the thesis secretary may become a thing of the past... but remember:
requirements do change, and this style file doesn't remove the need for
you to heed TeX's warning messages about overfull boxes and pages.

An older style file for LaTeX 2.09 is still available in various places
on campus. I used it as a starting point, but added a few enhancements
of my own.

I have no plans to maintain this thing. Users are on their own.
But at least I tried to document it as fully as time allowed me.

Change Log

v1.0d Converted ## to # as per changes in June 1995 LaTeX release.
v1.1  Changed openbib conditionals to a single command as per changes
           in December 1995 LaTeX release.
v1.2  Moved headers for opening pages to top of page.
v2.0  Chapter headers now consistent throughout.
      Fixed margins.
v2.1  Bug fix for titles containing \\
v2.5  Addition of halfcornellheadings and smallerheadings options
v2.6  Addition of draft, semifinal and final options


==> orig/discrete.tex <==
\section {Discretization} \label{sec:discrete}


==> orig/displaysetup.tex <==
\subsection {3D Teleimmersion}

The Tele-immersion is achieved by using Head Mounted Projective
Displays (HMPDs). First, the differences between the conventional
Head Mounted Display and the HMPD is clearly discussed.  Figure
~\ref{fig:conventHMD} illustrates the working of the Conventional
Head Mounted Display. In the conventional Head Mounted Display,
the virtual object is generated in front of the eyepiece and the
user can view the virtual image directly in front of him. Figure
~\ref {fig:conceptHMPD} explains the working of the projective
Head Mounted Displays. As seen from the figure, the virtual object
is being generated in a direction perpendicular to the eye and it
is being projected onto the beam splitter. The beam splitter
reflects the object onto the retro-reflective material which in
turn reflects the image back onto the eye. The projected image is
formed on the retro-reflective material. The main difference
between the HMPDs from conventional HMDs and stereoscopic
projection systems is the usage of a projection lens instead of an
eyepiece and the replacement of a diffusing projection screen with
a retro-reflective screen.

\begin{figure}[htp]
\centerline{\epsfig{figure=Figures/conventHMD.ps, width=4.0in} }
\caption{The concept of Conventional HMD} \label{fig:conventHMD}
\end{figure}

An HMPD, consists of a miniature projection lens and display
mounted on the head and a supple, non-distorting and durable
retro-reflective sheeting material placed strategically in the
environment. A miniature display, located beyond the focal point
of the lens rather than between the lens and the focal point as in
the configuration of a conventional HMD, is used to display a
computer-generated image. Through a projection lens, an
intermediary image is formed. A beamsplitter is placed after the
projection lens at 45 degrees with respect to the optical axis to
bend the rays at 90 degrees as done in an optical see-through HMD,
but the attitude of the beamsplitter is perpendicular to that of
an optical See Through HMD.

\begin{figure}[htp]
\centerline{\epsfig{figure=Figures/conceptHMPD.ps, width=5in} }
\caption{The Concept of Head Mounted Projective Display}
\label{fig:conceptHMPD}
\end{figure}

A retro-reflective screen is located on either side of the
projected image.  Because of the special characteristics of
retro-reflective materials, the rays hitting the surface are
reflected back onto themselves in the opposite direction. Ideally,
the location and size of the image is independent of the location
and shape of the retro-reflective screen. Furthermore, rays
hitting a retro-reflective surface will be reflected independently
of the incident angle . The difference between a diffusing
surface, a mirror surface and a retro-reflective surface is
illustrated in Figure ~\ref {fig:diffsurf}. ~\ref {fig:diffsurf}.a
reflected rays by a diffusing surface can be in all possible
directions; ~\ref {fig:diffsurf}.b reflected rays by a mirror
surface are symmetrical to the incident rays with respect to the
surface normal; ~\ref {fig:diffsurf}.c reflected rays by a
retro-reflective surface follow the opposites of the incident
rays.

\begin{figure}[htp]
\centerline{
   \epsfig{figure=Figures/diffsurf.ps, width=3.0in}}
\caption{Different kinds of surfaces (a) diffusing surface (b)
Mirror (c) Retro-reflective surface} \label{fig:diffsurf}
\end{figure}

The retro-reflective material is flexible enough to be clothed
around most surfaces, thus creating a great potential for
designing or transforming any existing objects or displays into a
projective AR display. Figure ~\ref{fig:retrosurf} shows some
examples of retro-reflective materials. Retro-reflective paint is
also available with which different kinds of surfaces can be
coated.


\begin{figure}[tb]
\centerline{
  \hspace{0.2in} \epsfig{figure=Figures/Microbeads.ps, width=1.5in}
  \hspace{0.2in} \epsfig{figure=Figures/Cornercube.ps, width=1.5in}
}
 \caption{Examples of Retro-reflective materials (a) Micro-beads
(b) Corner cubes } \label{fig:retrosurf}
\end{figure}

%\subsection {High-bandwidth Internet2 connection}


==> orig/figtable.tex <==
\newpage

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/figure1a.ps, width=3.5in}
} \caption{The surface and contour plots of a two-dimensional
energy function.A saddle point ($x_d$) is located between two
local minima ($x_s^1$ and $x_s^2$). $x_m^1$ and $x_m^2$ are two
local minima located in the orthogonal direction.}
\label{fig:saddlepoint}
\end{figure}

\newpage
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/figure1b.ps, width=3.5in}
} \caption{Phase potrait of the gradient system corresponding to
Fig. \ref{fig:saddlepoint}. The solid lines represent the basin
boundary which shows that $\partial A_p(x_s^1) = \bigcup_{i=1}^{3}
\overline{W^s(x_d^i)}$. The local minima $x_s^1$ and $x_s^2$
correspond to the stable equilibrium points of the gradient
system. The saddle point ($x_d^1$) corresponds to the
decomposition point of the gradient
system.}\label{fig:saddlepoint1}
\end{figure}


\newpage

\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/myleps2.ps, width=3.5in}
}\caption {Contour plot of a 2-D LEPS potential (described in
appendix-A). Each line represents the values of a constant
potential. $A$ and $B$ are the two local minima. $DP$ is the
decomposition point to be computed. The search direction is the
direction of the vector joining AB. The exit point ($X_{ex}$) is
obtained by finding the peak of the function value along this
vector. The dotted line indicates the stability boundary. The
dashed line indicates the search direction.} \label{fig:myleps2}
\end{figure}
\newpage
\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/myleps3aa.ps, width=3.5in} }
\caption {Illustration of the step 3 of our algorithm. $m_1$ is
integrated till $m'_1$ is reached and traced back along the vector
$m'_1B$ to get $m_2$, and so on... $m_n$ are the n points on the
stability boundary. The $n^{th}$ point is the Minimum Gradient
Point where the magnitude of the gradient ($G_M$) is the minimum.
DP is the decomposition point.} \label{fig:energy}
\end{figure}
\newpage

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/myleps2aa.ps, width=2.5in} } \caption{The plot of the function value along
the vector $AB$. The curve monotonically increases starting from
$A$ and then decreases till it reaches $B$. $X_{ex}$ is the exit
point where the function attains its peak value. $a_1$, $a_2$, ...
$a_9$ are the interval points. The marked circles indicate that
the function has been evaluated at these points. The empty circles
indicate the points where the function is yet to be evaluated.}
\label{fig:enecurve}
\end{figure}

\newpage

\begin{figure}
\begin{center}
 \epsfig{figure=Figures/peak2.ps, width=3.5in}\\
 \hspace{1.0in} (a) \hspace{1.8in} (b)\\
\end{center}\caption {The interval point $a_5$ can be present
either to the left or to the right of the peak. When $a_6$ is
reached, the golden section search method is invoked with $a_6$
and $a_4$ as the interval.} \label{fig:energycurve}
\end{figure}

\newpage
\pagebreak[4]

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/mullerbrown_results.ps, width=3.5in}
} \caption{Two dimensional contour plot of the potential energy
surface corresponding to the muller-brown function described on
Eq. (\ref{eq:mullerbrown}). A,B,C - stable equilibrium points and
DP1,DP2 - two decomposition points. The dashed lines indicate the
initial search direction. The dots indicate the results of the
trajectory adjustment procedure. These points are the points on
the stability boundary that reach the MGP.}
\label{fig:mullerbrownresult}
\end{figure}
\newpage
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/gradientcurve.ps, width=3.5in}
} \caption{The gradient curve corresponding to the various points
obtained from the trajectory adjustment procedure. The graph shows
that the magnitude of the gradient slowly increases in the initial
phases and then starts to reduce. The highlighted point
corresponds to the gradient at the MGP. }
\label{fig:gradientcurve}
\end{figure}
\newpage
\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/ljmorse.ps, width=3.5in}}
 \caption{Characteristic curves of Lennard-Jones potential and the Morse potential with all parameters set to unity.
 Solid line represents Lennard-Jones potential (\ref{eq:lennjones}) and the dashed line represents the Morse potential (\ref{eq:morsepotential}).} \label{fig:lennardjones}
\end{figure}

\newpage

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/atoms.ps, width=2.5in}
} \caption{Top view of the surface and the seven atom island on
the surface of an FCC crystal. The shading indicates the height of
the atoms.} \label{fig:minimum1}
\end{figure}

\newpage
\begin{figure}[htp]
\begin{center}
\epsfig{figure=Figures/sample.ps, width=3.5in}
\end{center}
\caption{Some sample configurations of the heptamer island on the
surface of the FCC crystal. First row- saddle points
configurations. Second row- other local minimum energy
configurations corresponding to the above saddle point
configurations.} \label{fig:atoms}
\end{figure}

\newpage

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/gradientcurve2.ps, width=3.5in}
} \caption{The gradient curve obtained in one of the higher
dimensional test cases.} \label{fig:gradientcurve2}
\end{figure}
\newpage

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/eckhardt2.ps, width=3.5in}
} \caption{Two dimensional contour plot of the potential energy
surface of the Eckhardt energy function described on Eq.
(\ref{eq:eckhardt}). A,B,M - stable equilibrium points and DP1,DP2
- two decomposition points. The dots correspond to the points on
the stability boundary during the trajectory adjustment
procedure.} \label{fig:eckhardt}
\end{figure}
\newpage
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/eckhardtgradientcurve.ps, width=3.5in}
} \caption{Gradient curve corresponding to the various points
along the stability boundary on the Eckhardt surface.}
\label{fig:eckhardtgradientcurve}
\end{figure}

\newpage
\begin{table}[htp]
\centering \caption{\protect\small Stable equilibrium points and
Decomposition points for the Muller-Brown Surface described in Eq.
(\ref {eq:mullerbrown}).}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Equilibrium Points &  Location & Energy value c(.) \\
\hline SEP A & (-0.558,1.442) & -146.7 \\
\hline DP 1 & (-0.822,0.624) & -40.67 \\
\hline SEP B & (-0.05,0.467) & -80.77 \\
\hline DP 2 & (0.212,0.293) & -72.25 \\
\hline SEP C & (0.623,0.028) & -108.7 \\ \hline
\end{tabular}
\end{center}
\label{TB:mullerbrownresults}
\end{table}
\newpage
\begin{table}[htp]
\centering \caption{\protect\small Stable equilibrium points and
Decomposition points for the three atom Lennard Jones Cluster
described in Eq. (\ref {eq:lennjones}).}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf \scriptsize Equilibrium Point} &  {\bf \scriptsize Location} & {\bf \scriptsize Energy value c(.)} \\
\hline

SEP A &$\begin{tabular}{c}(1.0,0.5,0.866) \\ \end{tabular}$&-3.000\\

\hline DP 1 & $\begin{tabular}{c} (2.0,1.0,0.0)  \\ \end{tabular}$ & -2.031\\
 \hline SEP B & $\begin{tabular}{c}
(1.0,0.5,-0.866)  \\ \end{tabular}$ &-3.000 \\

\hline
\end{tabular}
\end{center}
\label{TB:results}
\end{table}

\newpage




\begin{table}
\centering \caption{\protect\small Results of our algorithm on a
heptamer island over the FCC crystal. The number of force
evaluations made to compute the MGP is given in the last column. }
\begin{center}
\begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}|c|c|c|c|c|c|c|c|}
\hline
%{\bf \scriptsize Test Case} & {\bf \scriptsize }&{\bf \scriptsize Energy at } & {\bf \scriptsize Energy at} &{\bf \scriptsize } &  {\bf \scriptsize } & {\bf \scriptsize  No. of Force} \\
%{\bf \scriptsize Number} &  {\bf \scriptsize RMSD}& {\bf \scriptsize the MGP } & {\bf \scriptsize  the DP} &{\bf \scriptsize $\Delta$Energy} &  {\bf \scriptsize $\Delta $Force } & {\bf \scriptsize  evaluations} \\
Saddle No. & $E_{min}$ & $E_{saddle}$ & $E_{MGP}$ &$RMSD$& $\Delta$Energy & $\Delta$ Force & No. of evals \\
%Number & RMSD& the MGP & the DP & $\Delta$Energy & $\Delta$ Force & evaluations \\

\hline 1 & -1775.7787   & -1775.19 & -1775.2139 & 0.00917 &
0.02376 & 0.01833 & 49 \\
\hline 2 & -1775.7787  & -1775.1716
 & -1775.1906& 0.00802 &  0.01903 & 0.01671
& 43\\
\hline 3 & -1775.0079 &-1774.8055  & -1774.8213 & 0.0121 & 0.01578 & 0.01664& 97\\
\hline 4 & -1775.006  & -1774.8041  & -1774.9228
 & 0.03208 & 0.11868
& 0.02654& 67\\
\hline 5 & -1775.0058  & -1774.8024  & -1774.8149 & 0.01229 & 0.01256 & 0.01704 & 91\\
\hline 6 & -1775.0942  &-1774.5956  & -1774.3819 & 0.04285 &
-0.21362
 & 0.04343
& 37\\
\hline 7 & -1775.0931 &-1774.5841   & -1774.3916 &0.03296  &
-0.19252
 & 0.03905& 43\\
\hline 8 & -1775.01 &-1774.3106  & -1775.0789
 & 0.05287  & 0.76832
 & 0.04031& 97\\
\hline 9 & -1775.0097 &-1774.3082
  & -1775.0848
 & 0.05297 & 0.77662 & 0.04113
& 97\\
\hline 10 & -1774.3896
 &-1774.2979
 & -1774.9551 & 0.05623  & 0.65718
 & 0.03103& 79\\
\hline 11 & -1774.3928  &-1774.2997   & -1774.9541
 & 0.05615  & 0.65439
 & 0.03086
& 79\\
\hline 12 & -1774.3933 &-1774.2792   & -1774.2938
 & 0.02262 & 0.01450& 0.07092& 19\\
\hline
\end{tabular*}
\end{center}
\label{TB:highdimension}
\end{table}

\newpage
\pagebreak[4]

\begin{table}
\centering \caption{\protect\small Stable equilibrium points and
Decomposition points for the Eckhardt Surface described in Eq.
(\ref {eq:mullerbrown}).}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Equilibrium Points &  Location & Energy value c(.) \\
\hline SEP A & (-3.0,0.0) & 0.0 \\
\hline DP 1 & (0.0,1.4644) & 2.0409 \\
\hline SEP B & (3.0,0.0) & 0.0 \\
\hline DP 2 & (0.0,-1.4644) & 2.0409 \\
\hline SEP M & (0.0,0.0) & 4.7358 \\ \hline
\end{tabular}
\end{center}
\label{TB:Eckhardtresults}
\end{table}


==> orig/introduction-a.tex <==
\chapter {Introduction}
\label{ch:introduction} This chapter discusses the motivation for this thesis and introduces some terminology and theory needed to understand the following chapters.

\section {Motivation}
The problem of finding global optimal solution arises in many
disciplines ranging from science to engineering. The task of
finding such solutions is quite complicated and the complexity increases rapidly with
the dimensionality of the problem. Identifying some promising
regions in a solution space is relatively easier using certain
global methods available in the literature. However, the fine
tuning capability of these global methods is very poor and most of
these methods will end up with a relatively poor final solution even though the
surrounding region is promising. Hence, there is an absolute
necessity for exploring the surrounding region to get better solution.
In this thesis work, we develop a new method for finding such
solutions in a systematic manner. This method is more reliable
when compared to other stochastic approaches which merely use
random moves to find new solutions.

\begin{figure}
   \centering
   \subfigure[Entire Parameter Space]{\includegraphics[width = 4.05 in]{Figures/parfig.ps}}\qquad
   \subfigure[Promising Subspace]{\includegraphics[width = 4.05 in]{Figures/srfig.ps}}\qquad
   \caption{\label{fig:algo}Various stages of our algorithm in (a) Entire Parameter space - the dark regions indicate the promising solution subspaces. (b) The dots indicate the local optimal solutions and the regions surrounding are the stability regions of the corresponding local optimal solutions.
   }
   \label{fig:subspaces}
\end{figure}


Fig. \ref{fig:subspaces} clearly shows the problems with nonlinear surfaces. Global methods can be used to obtain promising subspaces in the parameter space. These are indicated by dark shaded regions in (a). However, these promising regions are not convex in nature. i.e. they will have multiple local optimal solutions. (b) gives the top view of the nonlinear surface in the promising region. The dots indicate the local optimal solutions. 'S' is the initial point obtained from the global methods. Applying local method at 'S' will converge to 'A'. There are other stochastic methods that can search the neighborhood regions e.g. mutations in genetic algorithms, low temperature annealing in simulated annealing method.

These stochastic methods randomly perturb the given point without much topological understanding of the nonlinear surface. Using stability regions, we have a deterministic approach to obtain
neighboring local maxima as opposed to widely used stochastic
methods. These stochastic methods never guarantee the
presence of a new stability region. Our approach not only
guarantees that a new local maximum obtained is different from the
original solution but also confirms that we will not miss a solution
in any particular direction. As shown in Fig. \ref{fig:subspaces}(b), the given local optimal solution 'A' is randomly perturbed to obtain new initial points ($s_1,s_2,s_3$). Applying local method using these initial points again, one can obtain the local optimal solutions $A,a_{14}$ and $a_{23}$ respectively. It can be observed that the solutions might appear again or might miss the neighborhood solutions. In this thesis, we present a new stability region based method for finding such neighborhood
solutions in a systematic manner. 

\input{background}

\section {Organization of this Thesis}
The remainder of this thesis is organized as follows.
Chapter~\ref{ch:saddlepointdetection} describes a new stability
boundary based method to find saddle points on potential energy
surfaces. Chapter~\ref{ch:lennardjones} demonstrates the use of a
new stability region method for finding the global minima that
corresponds to the stable structures of Lennard-Jones clusters.
Application of this method for efficient training of neural networks
is discussed in Chapter ~\ref{ch:training}. Finally,
Chapter~\ref{ch:future} discusses the future research directions
that I will be working on.


==> orig/lennardjones.tex <==
\chapter {Structure Prediction using Stability Region based Method}
\label{ch:lennardjones}

Finding global optimal solution is a challenging problem and appears
in many practical applications. Most of the traditional methods rely
on stochastic methods to find promising regions in the search space
and then apply deterministic local methods to fine tune the
solution. This may not be very effective solution for finding global
minima. This chapter describes a new method of searching the nearby
local minima in a systematic manner using the concepts of stability
regions. This method needs some initial points in the promising
subspaces and it will search many neighborhood regions as opposed to
single convergence region as in traditional methods. We applied this
new method for the problem of structure prediction of Lennard-Jones
clusters. We show that this method is very effective in searching
the neighborhood solutions and gives better solution that even the
traditional genetic algorithms fail to give.

\section{Introduction}
In the field of bioinformatics, the main interest of developing new
and efficient global optimization algorithms basically stem from the
problem of finding the lowest energy configuration of a
macromolecular system \cite {Horst00}. According to thermodynamic
hypothesis \cite{Anfinsen73}, the native structure of a protein is
structurally related to the global minimum of its potential energy
surface (PES). If this global minimum could be found reliably from
the primary amino acid sequence, this knowledge would provide us
with new insights into the nature of protein folding and save
biochemists many hours in the laboratory. Unfortunately, this goal
is far from being realized. Lack of a highly sophisticated
computational approach for global optimization of complex potential
energy functions is one of the primary limitations of structure
prediction for many years. Hence, any new global optimization
algorithm must be tested on much simpler systems. Lennard-Jones (LJ)
clusters represent one such test system which is well studied in the
literature. These clusters are aggregates of atoms, ions, or
molecules, that are very small and correspond to systems that are
neither single entities nor continua composed of an infinite number
of units, thus bridging the gap between single atoms or molecules
and bulk matter \cite {Hoare79}. These energy surfaces have huge
number of local minima. A cluster with 147 atoms is estimated to
have $10^{60}$ number of local minima \cite{Wales99}.

Usually global methods are good in getting promising regions in the
solution space, the fine tuning capability for getting a good local
minimum in that region is not really sophisticated. Since, the
nature of the algorithm is generally stochastic, even a hybrid local
search will behave stochastically (like mutations in genetic
algorithms or T=0K case in simulated annealing). Nevertheless, the
subspace surrounding the initial point will contain promising
solutions nearby. Hence, the challenge will be to explore all the
local minima inside the subspace surrounded around the initial
guess. The main problems of using stochastic based local searches is
that they might sometime miss the nearby local solution and
sometimes they don't even guarantee that you get always a new local
minima. After mutations, we might end up in the same convergence
region and it is not known until a local solver is applied at the
new initial point.

%Problems with most Optimization Algorithms - The convergence to an
%optimal solution depends on the chosen initial condition. The
%non-convergence to a local optimal solution may occur (i.e.
%divergence) Most algorithms tend to get stuck to a local optimal
%solution.
%
%Challenging Issues - How to effectively move (escape) from a local
%optimal solution and move on toward another local optimal solution;
%How to avoid revisiting local optimal solutions which are already
%found before; How to identify the regions that contain local optimal
%solutions; How to avoid searching the regions that contain no local
%optimal solutions.
%
%Most of the current optimization algorithms apply some global search
%techniques like genetic algorithms or simulated annealing to explore
%the entire search space to locate the regions of ``high-quality"
%solutions. Multiple points obtained from these methods are used as
%initial estimates for local optimizers to get the corresponding
%local minima. The best of all the local optimal solutions obtained
%is reported as the global optimal solution. Generally, the global
%search methods as stochastic in nature where as the local search
%techniques work deterministically. Several local solvers like the
%steepest descent method, Conjugate-gradient method, Newton-based
%methods have been used in literature and a thorough discussion about
%them is given in \cite{Press92}. Local-heuristic - Find a local
%optimal solution from an initial condition
%
%Our method systematically finds multiple local optimal solutions in
%a tier-by-tier manner.
%
%
%Enabling Technique (1) For systematically finding multiple local
%optimal solutions in a tier-by-tier manner. For finding another
%minimum-change local optimal solution (3) For finding another
%directional minimum-change local optimal solution
%
%Enhancing Technique (1) It enhances and ensures the convergence of a
%local search method. x1: initial condition diverges x2: new initial
%condition brought by the paradigm converges
%
%Find the set of local optimal solutions in a tier-by-tier manner.
%
%Avoid revisiting, missing to find local minima and visiting
%'nowhere' to find local optimal solutions.
%
%The most important advantage of the proposed method is that it can
%be used as an interface with any existing global optimization method
%to improve its performance in finding a better global optimal
%solution.
%
%Search procedure of our GOT Transformation : every local optimal
%solution becomes a stable equilibrium point. The search space is the
%union of the closure of quasi-stability region of every s.e.p. Find
%a local optimal solution (applying a local method). Apply our
%DT-based multi-tier search paradigm to search for the first-tier
%local optimal solutions. Find the first-tier local optimal solutions
%
%The main limitation of structure prediction algorithms is the lack
%of computational power in the present technology. Any problem that
%has exponential number of solutions will take years to solve using
%our present day computer power. Hence, there is an absolute need for
%an efficient global optimization algorithm  that can explore the
%entire search space in a very efficient way. The algorithm we are
%proposing is based on the ideas of genetic algorithms that had been
%extensively studied in the past.

 We test our algorithm for the strucute prediction of Lennard-Jones (LJ) clusters which the testbed
for many global optimization algorithms in the area of
bioinformatics. The Lennard-Jones potential has been used not only
for studying global optimization but also the effects of finite size
on phase transitions such as melting. The problem that is to be
solved in this paper is formally described as the following : {\it
Given N atoms interacting with two-body central forces, find the
three dimensional configuration that possess the global minimum
potential energy. } In general, this three dimensional configuration
will be in a simplified norm space and we take the Euclidean space
in further discussions. This energy minimization problem can be
described as a nonconvex nonlinear optimization problem.


%As described earlier, the main focus of this paper is to introduce a
%new global optimization technique and illustrate its capability of
%finding global optimal solution. Section~\ref{sec:background}
%briefly describes some relevant background. Section~\ref{sec:ga}
%describes the problem formulation and explains more about the
%Lennard-Jones clusters. Section~\ref{sec:lennardjones} analyzes the
%equations and properties of Lennard-Jones clusters and also gives
%details about their derivatives. The algorithm used for finding the
%global minima is clearly described in Section ~\ref {sec:algorithm}.
%Results are shown in Section ~\ref{sec:results} along with some
%discussion. Conclusions and future plans of our research are
%discussed in Section ~\ref{sec:conclusion}.


\section{Background}
\label{sec:background} Montecarlo methods have been used for the
structure prediction of microclusters in general based on the
Metropolis criterion. The simulated Annealing method \cite
{Kirkpatrick83} has been popularly used either as a stand alone
method or in combination with some other minimization methods. The
main motivation behind this method is the fact that each time a
compound is synthesized, nature somehow seems to solve an energy
minimization problem by what could be called an analog
computation.  The main problem of this method is that when the
catchment region of the global minimum is narrow, then this method
is very likely to miss it. The static method is based on a
minimization technique to find the configuration of a cluster
corresponding to the nearest energy local minimum. It is a
temperature independent approach and can be regarded as the $T=0K$
case. Diffusion equation method \cite {Kostrowicki91} has been
used to smoothly deform the potential energy hypersurface in such
a way that shallow potential wells disappear gradually, while the
deeper ones grow at their expense. The main advantage of this
method is that one need not explore several local minima. However,
this approach assumes that the shallow potential wells disappear
faster than the deeper ones which might not be true always.
Another problem of hypersurface deformation is that there is no
guarantee that the global minimum on the deformed PES will map
onto the global minimum of the original surface.

The basin-hopping method described in \cite {Wales97} is mainly
based on the variations of diffusion equation methods. However,
unlike other methods based upon hypersurface deformation, this
transformation in \cite {Wales97} does not change the global
minimum. This is the best known method for finding local minima.
Deformation procedures (like the distance scaling method) have
been used to reduce the number of local minima \cite{Pillardy99}.
Some successful global optimization results for LJ clusters using
Genetic algorithms are shown in \cite {Niesse96}.  The genetic
algorithms have also been used in combination with some other
algorithms for several problems. One such method is Conformational
Space Annealing \cite {Lee99a}. Some ideas that are described in
this paper basically originated from this method. The main success
of this algorithm is mainly because of its capability to search
over extremely broad ranges of conformational space, generating
numerous local minima before arriving at the global minimum free
energy conformation. Therefore, this searching method allows one
to calculate many different groups of low-energy potential
function values, one of which is presumably the global energy
minimum value. After applying a genetic algorithm one has to
minimize the conformation that is generated using any local
minimization algorithm. In this paper we used BFGS method for
local minimization. Advantages and disadvantages of using
different kinds of local minimization algorithms in the field of
computational chemistry \cite {Schlick02}.


\section{LJ Clusters}
\label{sec:lennardjones} The most common and most simplistic model
for interaction between atoms is the Lennard Jones pair potential.
Much of the initial interest in LJ clusters was motivated by a
desire to calculate nucleation rates for noble gases. The Lennard
Jones potential is given by the Equation ~\ref{eq:lennjones}. For
the sake of simplicity, we use reduced units, i.e. the values of
$\epsilon$ and $r_0$ are taken to be unity. Plot of Lennard-Jones
Potential of interaction between two atoms generated using
Equation~\ref{eq:lennjones} is shown in
Figure~\ref{fig:lennardjones}.

\begin{eqnarray}
V = \sum_{i=1}^{N-1} \sum_{j=i+1}^N v(r_{ij}) \\
v(r_{ij}) = \epsilon\left[\left(\frac{r_0}{r_{ij}}\right)^{12} -
2\left(\frac{r_0}{r_{ij}}\right)^6\right] \label{eq:lennjones}
\end{eqnarray}

where \\
\centerline {$ r_{ij} = \sqrt {  (x_i - x_j)^2 + (y_i - y_j)^2 +
(z_i - z_j)^2 }$} \\ $V$ is the total potential energy of the
microcluster is given as the summation of of all two-body
interaction terms, $v(r_{ij})$ is the potential energy term
corresponding to the interaction of atom $i$ with atom $j$, and
$r_{ij}$ is the Euclidean distance between $i$ and $j$. $\epsilon$
describes the strength of the interaction and $r_0$ is the
distance at which the potential is zero.

%\subsection*{Properties of LJ Potential}
%The constants $\epsilon$ and $r_0$ are important to determine the
%strength and shape of the interaction and hence the properties of
%the solid or liquid. $\epsilon$ is the minimum of the potential
%(energy scale) and $r_0$ is the distance at which the potential is
%zero (length scale). If $r_0~ = ~r_{ij}$, then the potential is
%zero. So by changing $r_0$ one can move the whole potential to the
%right or to the left. This can affect the overall structure of the
%solid state. The force between individual atoms is the negative of
%the gradient of the potential. The details of the generation of
%the force for this Lennard-Jones potential is shown in
%Section~\ref{sec:dynamicalsystem}.
%
When the separation $r$ is very small, the $\frac{1}{r^{12}}$ term
dominates, and the potential is strongly positive. Hence the
$\frac{1}{r^{12}}$ term describes the short range {\it repulsive
potential} due to the distortion of the electron clouds at small
separations. In contrast the $\frac{1}{r^6}$ predominates when the
separation $r$ increases in magnitude. Hence the $\frac{1}{r^6}$
term describes the {\it long-range attractive tail of the
potential} between two particles.

%\begin{figure}[htp]
%\centerline{ \epsfig{figure=Figures/lennardjones.ps, width=3.5in}}
% \caption{Plot of Lennard-Jones Potential
%of interaction between two atoms generated using Equation
%~\ref{eq:lennjones}.} \label{fig:lennardjones}
%\end{figure}

%The potential $v(r_{ij})$ has the following properties \cite
%{Hoare79}:
%\begin{itemize}
%\item {{\it No interaction at infinite separation} i.e.
%$v(r)\rightarrow 0$ as $r\rightarrow\infty$. The potential starts
%at $\infty$ at $r=0$ , falls to $0$ at r=$r_0$, reaches a minimum
%of -$\epsilon$ at $r=r_0$ and then rises to zero as
%$r\rightarrow\infty$.}
%
%\item {{\it Rigid core} i.e. $v(r)\rightarrow\infty$ for
%$r<r_{min}$ and $r_{min}\geq 0$.}
%
%\item {{\it Single stable state} i.e. $v'(r_0)$ = 0 and $v''(r_0)
%> 0 $.}
%
%\end{itemize}

In the cartesian coordinate system, for any local minimum point,
all the first order derivatives must be zero. Mathematically, it
can be written as follows \cite {Floudas00}:

\begin{eqnarray}
 \sum_{j=1}^N
~\frac{v'(r_{ij})}{r_{ij}} ~(x_i-x_j)~=~0 ~ ~\forall i=2, ...,N\\
\sum_{j=1}^N ~\frac{v'(r_{ij})}{r_{ij}} ~(y_i-y_j)~=~0 ~ ~ \forall
i=3, ...,N\\
\sum_{j=1}^N ~\frac{v'(r_{ij})}{r_{ij}} ~(z_i-z_j)~=~0 ~ ~\forall
i=4, ...,N
\end{eqnarray}


This is a necessary but not a sufficient condition for local
optimality. The system mentioned above can be transformed into a
dynamical system by taking the negative gradient of its potential
function derivatives. We explain the details about the derivatives
of the potential energy function. The \emph{Dynamical System} is a
$3 \times N$~matrix as shown below :

\[ \nabla V(x) = - \left[ \begin{array}{ccc} \frac{\partial
V}{\partial x_1} & \frac{\partial V}{\partial y_1} &
\frac{\partial V}{\partial z_1}\vspace{0.05in}
\\
\frac{\partial V}{\partial x_2} & \frac{\partial V}{\partial y_2} & \frac{\partial V}{\partial z_2} \\
. & . & . \\
. & . & . \\
 &  &  \\
. & . & . \\
. & . & . \vspace{0.05in}\\
\frac{\partial V}{\partial x_n} & \frac{\partial V}{\partial y_n}
& \frac{\partial V}{\partial z_n} \end{array} \right]\]

where \\
\begin{equation}
\frac{\partial V}{\partial x_i} =\sum_{j=1}^N ~\frac{\partial
V}{\partial r_{ij}}~ . ~\frac{\partial r_{ij}}{\partial x_i}
\label{eq:derivative}
\end{equation}
The partial derivative of the potential function $(V)$ w.r.t.
$r_{ij}$ is given by (\ref{eq:derivative1}).
\begin{equation}
\frac{\partial V}{\partial r_{ij}} = \ 12
\left[\left(\frac{1}{r_{ij}}\right)^{7} -
\left(\frac{1}{r_{ij}}\right)^{13}\right] \label{eq:derivative1}
\end{equation}
The partial derivative of the potential function $r_{ij}$ w.r.t.
individual cartesian coordinates is given by
(\ref{eq:derivative2}).

\begin{equation}
\frac{\partial r_{ij}}{\partial x_i} =  \frac{x_i-x_j }{r_{ij}}
\label{eq:derivative2}
\end{equation}

Substituting (\ref{eq:derivative1}) and (\ref{eq:derivative2}) in
(\ref{eq:derivative}), we have
\begin{equation}
\frac{\partial V}{\partial x_i} =\sum_{j=1}^N
~\frac{12}{(r_{ij})^8}
 ~ \left[ 1 - \left( \frac{1}{r_{ij}} \right)^6 \right] ~ (x_i-x_j)
\label{eq:finalderivative}
\end{equation}


\section{Exploring Multiple Local Minima}
\label{sec:algorithm} The method described in this section finds
multiple local minima present in the neighborhood of the existing
local minima. Our method is illustrated in the figure . \\Input :
Any random point or a promising location point obtained from a
stochastic global search method like genetic algorithm.\\ Output : Multiple local minima surrounding the initial guess.\\
%
%\begin{figure}[htp]
%\begin{center}
%\epsfig{figure=Figures/myleps1.ps, width=3.5in}
%% \hspace{0.3in} \epsfig{figure=Figures/energy.ps, width=1.3in}
%\caption {Contour plot of a 2-D LEPS potential (described in
%appendix). Each line represents the values of a constant potential.
%$A$ and $B$ are the two local minima. $D$ is the decomposition point
%to be computed.}
% \end{center}
%\label{fig:leps}
%\end{figure}

%\begin {enumerate}
%\itemsep +.1in

Step1: {\it Moving to a Local Minima} : Find a local minima using
some local solver. The initial guess can be obtained from any global
search method like genetic algorithms or it may be purely random
starts.
\\


Step2: {\it Initializing the Search direction} : Compute the
eigenvectors of the Hessian matrix at the local minimum 'A'. Taking
small step sizes along these eigenvector directions, evaluate the
objective function value. Because the small steps begin from a local
minimum, the objective function initially increases.

Step 3: {\it Identifying neighboring regions of convergence} :
Proceed with the evaluation along each of the directions till each
objective function value starts to decrease. This decrease indicates
crossing a stability boundary on the objective surface and entrance
into a neighboring region of convergence. These points are called
'X'. A heuristic can be applied to reduce the amount of computation
in this algorithm if desired. The points 'X' can be ranked according
to objective function value and objective function gradient measured
from 'A'. The top few ranking 'X', which may have a higher chance of
leading to promising regions, can be used to proceed to the next
step in the algorithm.
 \\



%\begin{figure}[htp]
%\centerline{ \epsfig{figure=Figures/myleps2.ps, width=3.5in}
%}\caption {Illustration of steps 1 and 2 of our method. The search
%direction is the direction of the vector AB. The exit point
%($X_{ex}$) is obtained by finding the peak of the energy function
%along this vector.} \label{fig:myleps2}
%\end{figure}

Step 4: {\it Finding Tier-1 local minima} :The points 'X' are used
as new initial guesses for the local solver. Each 'X' is guaranteed
to converge to a local minimum different from 'A'. These new Tier 1 local minima are usually unique because of the high dimensionality of the problem. \\

Step 5: {\it Exploring the entire subspace} : Steps 2 to 4 are
repeated to search for local minima beyond Tier 1. Here, the Tier 1
local minima take the place of the first local minimum 'A'. To avoid
the exponential growth of the number of local minima, the
above-mentioned heuristic can be applied to consider only the search
directions that yield promising results upon further exploration.
Depending on the complexity of the problem, local minima obtained
from Tier 2 or 3 already show significant improvement over the first local minimum 'A'. \\

Typically, the initial point 'A' can be replaced by the best of
neighborhood local minima where the MSE is the least.
\begin{figure*}[htp]
\centerline{ \hspace {0.1in}
  \epsfig{figure=Figures/fig1.ps, width=2.1in} \hspace {0.3in}
  \epsfig{figure=Figures/fig3.ps, width=2.3in}
} \caption{(a) Promising areas in the solution space obtained by
evolutionary stochastic approaches. (b) Multiple local minima are
explored around the local minimum in each promising location.
 (c) Exploring multiple minima from a single local minimum. `*' indicates the initial point obtained from the stochastic method.
`.' indicates the local minima. Dotted arrow indicates convergence
from a point to its local solution. Solid arrows indicate the
steepest ascent directions from a given local minimum. `X' indicates
initial points in other stability regions.
 }\label{fig:concept}
\end{figure*}


%\begin{figure}[htp]
%\epsfig{figure=Figures/myleps3.ps, width=3.5in}
%
%\caption {Illustration of the step 3 of our algorithm. $m_1$ is
%integrated till $m'_1$ is reached and traced back along the vector
%$m'_1B$ to get $m_2$, and so on... $m_n$ are the n points on the
%stability boundary. The $n^{th}$ point is the Minimum Vector-field
%Point where the magnitude of the gradient ($G_M$) is the minimum. D
%is the decomposition point.} \label{fig:energy}
%\end{figure}


\section {Results}
\label{sec:results}
%
%
%\begin{table}
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline Sl  &Name& No. of  & No. of  & Sample
%&No. of &No. of\\
%No. & &Features& Classes & size & Units & Variables \\
%
%\hline 1 & Splice   & 60 & 3 & 3190 & 10 & 621  \\
%\hline 2 & Image   & 19 & 7 & 2310 & 8 &  169\\
%\hline 3 & Ionosphere   & 34 & 2 & 351 & 9 &325  \\
%\hline 4 & Iris   & 4 & 3 & 150 & 3&19\\
%\hline 5 & Diabetes   & 8 & 2 & 768 & 8 & 81  \\
%\hline 6 & Vehicle  & 18 & 4 & 846 &12& 241\\
%\hline 7 & Wine   & 13 & 3 & 178 & 4 &61\\
%\hline 8 & Cancer   & 9 & 2 & 683 & 5  & 56\\
%\hline 9 & Sonar   & 19 & 39 & 208 & 8 &497\\
%\hline 10 & Vowel   &19 & 26 & 990 & 5 & 71\\
%\hline 3 & Ionosphere   & 34 & 2 & 351 & 9 &325  \\
%\hline 4 & Iris   & 4 & 3 & 150 & 3&19\\
%\hline 5 & Diabetes   & 8 & 2 & 768 & 8 & 81  \\
%\hline 6 & Vehicle  & 18 & 4 & 846 &12& 241\\
%\hline 7 & Wine   & 13 & 3 & 178 & 4 &61\\
%\hline 8 & Cancer   & 9 & 2 & 683 & 5  & 56\\
%\hline 9 & Sonar   & 19 & 39 & 208 & 8 &497\\
%\hline 10 & Vowel   &19 & 26 & 990 & 5 & 71\\
% \hline
%\end{tabular}
%\end{center}
%\label{TB:dataset}
%\end{table}
%In general, for any global optimization algorithm, one generates
%massive quantities of information. Rather than accumulating all the
%information for each new conformation and exponentially increasing
%the data size, one can apply more sensible approach to solve this
%problem by reviewing the following aspects at each newly generated
%energy-minimized conformation :
%\begin {enumerate} \item {Does the new conformation contain
%redundant i.e. is it significantly similar to one of the existing
%seeds? or does it represent a distinct class of local minima?}
%\item { If the conformation is judged to be significantly similar
%to an existing group, how do we determine which conformation in the
%bank of conformation is most likely to contain less information when
%compared to the new conformation?}
%\end {enumerate}

\subsection*{Distance Spectrum}
\label{sec:distance}

Estimating the distance between two different configurations is
not a trivial problem. Our assumption is that both the
configurations are of same scale , in other words, these
configurations are to be tested for the different permutations
between the atoms. The similarity between these two configurations
can be estimated using the distance spectrum. We for mthe distance
matrix of size N X N which gives s the distance between each atom
to every other atom. For a N atom system, the size of the distance
spectrum will be N*(N-1)/2. Once, the lower or upper triangle of
the distance matrix is obtained, it is sorted to obtain the
distance spectrum. The sorting algorithm we have used is the
bubble sort algorithm. To compare two similar configurations we
take the Root Mean Square Deviation (RMSD) of their corresponding
distance spectra.
%
%Theorem: Two similar atomic configurations will have the same
%distance spectrum. Corollary 1 : The distance spectrum can not be
%used for solving the problem of scale. Corollary 2 : The distance
%spectrum can solve the problem of any number of permutations.


==> orig/microclusters.tex <==
\section {Microclusters} \label{sec:microclusters}


==> orig/motiffinding.tex <==
\section {Motif Finding Problem - Probabilistic Setting} \label{sec:motif}

The goal of motif finding is to detect novel, overrepresented
unknown signals in a set of sequences (for eg. transcription factor
binding sites in a genome). Recently, many algorithms were proposed
to solve the problem and currently it is a very active area of
research. Most widely used algorithms for finding motifs obtain a
generative probabilistic representation of the overrepresented
signals and try to discover profiles that maximize information
content score. Though these profiles form a very powerful
representation of the signals, the major difficulty arises from the
fact that the best motif corresponds to the global maximum of a
non-convex continuous function. A DNA motif can be represented in
continuous space in terms of a position specific scoring matrix of
dimension LxJ, where L is the length of the motif and J = 4
representing A,T,C,G.  At each position, there will be a
probabilistic weight assigned to the likelihood of each nucleotide
alphabet being at that position.
%
%The position weight matrices is constructed from a single bucket of
%L-MERs The equations involved are the following: Qo,j = (Co,j + bj)
%/ ‡" Co,j + ‡" bj (1) Qi,j = (Ci,j + bj) / N + ‡" bj (2) Ax = ðQi,j
%/ ðQo,j (3) In (1) Qo,j represents the background distribution of
%each DNA nucleotide 'A', 'T', 'C', 'G'. Co,j is the count of each
%nucleotide where j = {A,T,C,G}. bj is a correction that are added to
%the nucleotide count. In (2) Qi,j represents the count of each
%nucleotide j = {A,T,C,G} where i represents the position of the
%nucleotide within the L-MER. In (3), the ratio is achieved between
%the product of all non-background positions to that of the
%background distribution of nucleotides. Equation (3) is employed
%when calculating the score of each L-MER in each of the given
%sequences.

Algorithms like Expectation Maximization (EM) and Gibbs sampling
tend to be very sensitive to the initial guesses and are known to
converge to the nearest local maxima very quickly. To improve the
quality of the results, EM is used with multiple starts or any other
global methods (like projection algorithms) that might yield
promising initial guesses. Random Projection is one such global
method that gives an initial guess in the convergence region of a
promising local maxima. The method involves hashing every possible
L-mer by those designated positions. Any hash code with more than a
threshold L-mers would be considered for further processing. The
initial predictions are then represented in a probabilistic method
known as position specific scoring matrix. However, these global
methods do not necessarily give initial guesses in the convergence
region of the best local maxima rather they suggest that a promising
solution is in the neighborhood region. I am planning to introduce a
novel optimization framework that searches the neighborhood regions
of the initial guess in a systematic manner. This framework also
allows flexibility in using different local solvers and global
methods that work well for some specific datasets. This idea of
allowing the users to choose between different local and global
methods is very helpful in such problems where many methods are
still in try out stage.


==> orig/multiobjective.tex <==
\section {Multi-objective Optimization} \label{sec:multi}
Real world engineering design problems are usually characterized by
the presence of many conflicting objectives. The methodology
described in earlier chapters can be extended to solve these
multi-objective problems. There are many architectures that can be
used to solve these problems.

I will focus my research on two such methods.  One of the simpler
yet efficient methods of solving these problems is the
$\epsilon$-constraint method. In this method, one objective function
is chosen to be the main one and others are reformulated as
constraints. By progressively, changing the constraint values, the
pareto-front could be sampled. The theory developed for constrained
optimization will be extended to solve these problems.

The other method that I will be working is the global criterion
method. In some problems, the users will have the knowledge of the
ideal vector that is to be attained. In these cases, we can use the
global criterion method which formulates the original problem as a
new optimization problem which minimizes the distance from the
current solution vector to the ideal solution vector. One special
case of this global criterion method is the min-max optimization.


==> orig/nonlineardynamics.tex <==
\section {Nonlinear Dynamics} \label{sec:nonlineardynamics}


==> orig/numerical.tex <==
\section {Numerical Improvements} \label{sec:motif}
The main goal of this work is to improve the efficiency of
numerical computations for faster convergence to the local minima.
This numerical improvements can also help during the tracing of
the decomposition point. If the original dynamical system is
multiplied by a positive definite matrix, then position of the
equilibrium points is unchanged and the type of the equilibrium
point is also preserved. The shape of the stability boundary
changes but still contains the same equilibrium points. One of the
main challenging problems is the choice of condition matrix. The
main idea is to study the local behavior from the Jacobian and
design a condition matrix that captures the local behavior of the
system.


==> orig/otherapplications.tex <==
\section {Other Application Areas} \label{sec:others}


==> orig/pattern.tex <==
\section{Pattern Discovery - Motif Finding Problem}
As a case study of the algorithm developed in the previous section, we describe its application to the motif finding problem in bioinformatics. In fact, we do not have to restrict the proposed algorithm to the case of mixture models. Here, we will demonstrate its capability in obtaining promising solutions on general likelihood surfaces. The main goal of the motif finding problem is to detect novel, over-represented unknown signals in a set of sequences (e.g.
transcription factor binding sites in a genome). The most widely
used algorithms for finding motifs obtain a generative probabilistic
representation of these over-represented signals and try to discover
profiles that maximize the information content score. Although these
profiles form a very powerful representation of the signals, the
major difficulty arises from the fact that the best motif
corresponds to the global maximum of a non-convex continuous
function. Popular algorithms like Expectation Maximization (EM) and
Gibbs sampling tend to be very sensitive to the initial guesses and
are known to converge to the nearest local maximum very quickly \cite{Reddy06a}. In
order to improve the quality of the results, EM is used with
multiple random starts or any other powerful stochastic global
methods that might yield promising initial guesses (like projection
algorithms). Global methods do not necessarily give initial guesses
in the convergence region of the best local maximum but rather
suggest that a promising solution is in the neighborhood region. In
this section, we apply the SREM algorithm proposed in the previous section to this motif finding problem. It has the capability to search the neighborhood regions of the initial alignment in a
systematic manner to explore the multiple local optimal solutions.
This effective search is achieved by transforming the original
optimization problem into its corresponding dynamical system and
estimating the practical stability boundary of the local maximum.


\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/sequences.ps, width=4.5in}
} \caption
{Synthetic DNA sequences containing some instance of the
pattern `CCGATTACCGA' with a maximum number of 2 mutations. The
motifs in each sequence are highlighted in the box. We have a (11,2)
motif where 11 is the length of the motif and 2 is the number of
mutations allowed.}
\label{fig:sequences}
\end{figure}

Recent developments in DNA sequencing have allowed biologists to
obtain complete genomes for several species. However, knowledge of
the sequence does not imply the understanding of how genes interact
and regulate one another within the genome. Many transcription
factor binding sites are highly conserved throughout the sequences
and the discovery of the location of such binding sites plays an
important role in understanding gene interaction and gene
regulation. Although there are several variations of the motif finding
algorithms, the problem discussed here is defined as
follows: without any previous knowledge of the consensus pattern,
discover all the occurrences of the motifs and then recover a pattern
for which all of these instances are within a given number of
mutations (or substitutions). Despite the significant amount of
literature available on the motif finding problem, many do not
exploit the probabilistic models used for motif refinement
\cite{Lawrence93,Bailey94}. In this section, we consider a precise version of the motif discovery problem in
computational biology as discussed in \cite{Buhler01,Pevzner00}. The
planted (l,d) motif problem \cite{Pevzner00} considered here is described as follows: Suppose there is a fixed but unknown
nucleotide sequence $M$( the {\it motif}) of length $l$. The problem
is to determine $M$, given $t$ sequences with $t_i$ being the length
of the $i^{th}$ sequence and each containing a planted variant of
$M$. More precisely, each such planted variant is a substring that
is $M$ with exactly $d$ point substitutions (see
fig.~\ref{fig:sequences}). More details about the complexity of the
motif finding problem is given in \cite{Pevzner00a}. A detailed
assessment of different motif finding algorithms was published
recently in \cite{Tompa05}.


%The length of the motif in each occurrence may not be the same as in
%all of the other occurrences, although in general the occurrences
%must have roughly the same length.


%More details on the estimates of the hardness of this problem
%without any complex information like overlapping motifs and
%background distribution is shown in \cite{Waterman84}.


\subsection{Motif Finding Literature}
\label{sec:background} Existing approaches used to solve the motif
finding problem can be classified into two main categories
\cite{Eskin04}. The first group of algorithms utilizes a generative
probabilistic representation of the nucleotide positions to discover
a consensus DNA pattern that maximizes the information content
score. In this approach, the original problem of finding the best
consensus pattern is formulated as finding the global maximum of a
continuous non-convex function. The main advantage of this approach
is that the generated profiles are highly representative of the
signals being determined \cite{Durbin99}. The disadvantage, however,
is that the determination of the ``best" motif cannot be guaranteed
and is often a very difficult problem since finding global maximum
of any continuous non-convex function is a challenging problem.
Current algorithms converge to the nearest local optimum instead of
the global solution. Gibbs sampling \cite{Lawrence93}, MEME
\cite{Bailey94}, greedy CONSENSUS algorithm \cite{Hertz99} and HMM
based methods \cite{Eddy98} belong to this category.

The second group uses patterns with `mismatch representation' which
define a signal to be a consensus pattern and allow up to a certain
number of mismatches to occur in each instance of the pattern. The
goal of these algorithms is to recover the consensus pattern with
the highest number of instances. These methods view the
representation of the signals as discrete and the main advantage of
these algorithms is that they can guarantee that the highest scoring
pattern will be the global optimum for any scoring function.  The
disadvantage, however, is that consensus patterns are not as
expressive of the DNA signal as profile representations. Recent
approaches within this framework include Projection methods
\cite{Buhler01,Raphael04}, string based methods \cite{Pevzner00},
Pattern-Branching \cite{Price03}, MULTIPROFILER \cite{Keich02} and
other branch and bound approaches \cite{Eskin02,Eskin04}.

A hybrid approach could potentially combine the expressiveness of
the profile representation with convergence guarantees of the
consensus pattern. An example of a hybrid approach is the Random
Projection \cite{Buhler01} algorithm followed by EM algorithm
\cite{Bailey94}. It uses a global solver to obtain promising
alignments in the discrete pattern space followed by further local
solver refinements in continuous space\cite{Barash01,Segal02}.
Currently, only few algorithms take advantage of a combined discrete
and continuous space search \cite{Buhler01,Eskin04,Raphael04}. We consider the profile representation of the motif
and a new hybrid algorithm is developed to escape out of the local
maxima of the likelihood surface.


Some motivations to develop the new SREM algorithm are :
\begin {itemize}
\item{A motif refinement stage is vital and popularly used by many
pattern based algorithms (like PROJECTION, MITRA etc) which try to
find optimal motifs. } \item{The traditional EM algorithm used in
the context of motif finding converges very quickly to the nearest
local optimal solution (within 5-8 iterations).} \item{There are
many other promising local optimal solutions in the close vicinity
of the profiles obtained from the global methods.}
\end{itemize}

In spite of the importance placed on obtaining a global optimal
solution in the context of motif finding, little work has been done
in the direction of finding such solutions \cite{Xing04}. There are
several proposed methods to escape out of the local optimal solution
to find better solutions in machine learning \cite{Elidan02} and
optimization \cite{Cetin93} related problems. Most of them are
stochastic in nature and usually rely on perturbing either the data
or the hypothesis. These stochastic perturbation algorithms are
inefficient because they will sometimes miss a neighborhood solution
or obtain an already existing solution. To avoid these problems, we
introduce a novel optimization framework that has a better chance of
avoiding sub-optimal solutions. It systematically escapes out of the
convergence region of a local maximum to explore the existence of
other nearby local maxima. Our method is primarily based on some
fundamental principles of finding exit points on the stability
boundary of a nonlinear continuous function. The underlying
theoretical details of our method are described in \cite{Chiang96,
Lee04}.

\subsection{Preliminaries}
\label{sec:problem} We will first describe our problem formulation
and the details of the EM algorithm in the context of motif finding
problem. We will then describe some details of the dynamical system
of the log-likelihood function which enables us to search for the
nearby local optimal solutions.

\subsubsection{Problem Formulation} Some promising initial alignments
are obtained by applying projection methods or random starts on the
entire dataset. Typically, random starts are used because they are
not expensive. Most promising set of alignments are considered for
further processing. These initial alignments are then converted into
profile representation.


\begin{table}[h]
\centering \caption{\protect\small A count of nucleotides
${A,T,G,C}$ at each position $K={1..l}$ in all the sequences of the
data set. $K=0$ denotes the background count.}

\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline $j$ &  $k=0$& $k=1$&$ k=2$&$ K=3$ &$k=4$& ~...~ &  $k=l$\\
\hline

${A}$ & $C_{0,1}$ & $C_{1,1}$ &$C_{2,1}$ &$C_{3,1}$ &$C_{4,1}$ &...
&$C_{l,1}$\\ \hline

${T} $& $C_{0,2}$ & $C_{1,2}$ &$C_{2,2}$ &$C_{3,2}$ &$C_{4,2}$ &...
&$C_{l,2}$\\ \hline

${G}$ & $C_{0,3}$ & $C_{1,3}$ &$C_{2,3} $&$C_{3,3}$ &$C_{4,3}$ &...
&$C_{l,3}$\\ \hline

${C}$ & $C_{0,4}$ & $C_{1,4}$ &$C_{2,4} $&$C_{3,4}$ &$C_{4,4}$ &...
&$C_{l,4}$\\ \hline

\end{tabular}
\end{center}
\label{TB:PSSM}
\end{table}



Let $t$ be the total number of sequences and $n$ be the average
length of the sequences. Let $S=\{S_1,S_2...S_t\}$ be the set of $t$
sequences. Let $P$ be a single alignment containing the set of
segments $\{P_1,P_2,...,P_t\}$. $l$ is the length of the consensus
pattern. For further discussion, we use
the following variables \\

 \begin{tabbing}
\hspace{0.5in}$i~=~1~...~t~~~~~~~~~~~~--$ for $t$ sequences \\
\hspace{0.5in}$k~=~1~...~l~~~~~~~~~~~~--$ for positions within an $l$-mer\\
\hspace{0.5in}$j~\in~\{A,T,G,C\}~~~~--$ for each nucleotide\\
 \end{tabbing}

The count matrix can be constructed from the given alignments as
shown in Table ~\ref{TB:PSSM}. We define $C_{0,j}$ to be the
non-position specific background count of each nucleotide in all of
the sequences where $j \in \{ A,T,C,G \}$ is the running total of
nucleotides occurring in each of the $l$ positions. Similarly,
$C_{k,j}$ is the count of each nucleotide in the $k^{th}$ position
(of the $l-mer$) in all the segments in $P$.


\begin{equation}\label{eq:backcount}
    Q_{0,j}=\frac{C_{0,j}}{\sum_{J\in \{A,T,G,C\}}{C_{0,J}}}
\end{equation}

\begin{equation}\label{eq:forecount}
    Q_{k,j}=\frac{C_{k,j}+b_j}{t+\sum_{J\in \{A,T,G,C\}}{b_J}}
\end{equation}

Eq. (\ref{eq:backcount}) shows the background frequency of each
nucleotide where $b_j$ is known as the Laplacian or Bayesian
correction and is equal to $d*Q_{0,j}$ where $d$ is some constant
usually set to unity.  Eq. (\ref{eq:forecount}) gives the weight
assigned to the type of nucleotide at the $k^{th}$ position of the
motif.

A Position Specific Scoring Matrix (PSSM) can be constructed from
one set of instances in a given set of $t$ sequences. From
(\ref{eq:backcount}) and (\ref{eq:forecount}), it is obvious that
the following relationship holds:

\begin{equation}\label{eq:sum}
    \sum_{j \in \{A,T,G,C\}}Q_{k,j}=1 ~~~~~~~~~~\forall k=0,1,2,...l
\end{equation}

For a given $k$ value in (\ref{eq:sum}), each $Q$ can be represented
in terms of the other three variables. Since the length of the motif
is $l$, the final objective function (i.e. the information content
score) would contain $3l$ independent variables\footnote {Although,
there are $4l$ variables in total, because of the constraints
obtained from (\ref{eq:sum}), the parameter space will contain only
$3l$ independent variables. Thus, the constraints help in reducing
the dimensionality of the search problem.}.

To obtain the score, every possible $l-mer$ in each of the $t$
sequences must be examined.  This is done so by multiplying the
respective $Q_{i,j} / Q_{0,j}$ dictated by the nucleotides and their
respective positions within the $l-mer$. Only the highest scoring
$l-mer$ in each sequence is noted and kept as part of the alignment.
The total score is the sum of all the best scores in each sequence.

\begin{equation}\label{eq:final}
\begin{split}
    A(Q) &=\sum_{i=1}^t log(A)_i=\sum_{i=1}^t
    log\left(\prod_{k=1}^{l}\frac{Q_{k,j}}{Q_b}\right)_i\\ & \quad
    =\sum_{i=1}^t \sum_{k=1}^l log(Q_{k,j}^{'})_i
\end{split}
\end{equation}


$Q_{k,j}^{'}$ is the ratio of the nucleotide probability to the
corresponding background probability, i.e. $Q_{k,j} / Q_b$.
$Log(A)_i$ is the score at each individual $i^{th}$ sequence where t
is the total number of sequences.  In equation (\ref{eq:final}), we
see that $A$ is composed of the product of the weights for each
individual position $k$. We consider this to be the Information
Content (IC) score which we would like to maximize. $A(Q)$ is the
non-convex $3l$ dimensional continuous function for which the global
maximum corresponds to the best possible motif in the dataset. EM
refinement performed at the end of a combinatorial approach has the
disadvantage of converging to a local optimal solution
\cite{Blekas03}. Our method improves the procedure for refining
motif by understanding the details of the stability boundaries and
by trying to escape out of the convergence region of the EM
algorithm.

%\subsection{EM algorithm for Motif Refinement}

\subsubsection{Hessian Computation and Dynamical System for the Scoring Function}
In order to present our algorithm, we have defined the dynamical
system corresponding to the log-likelihood function and the PSSM.
The key contribution here is the development of this
nonlinear dynamical system which will enable us to realize the
geometric and dynamic nature of the likelihood surface. We construct
the following {\it gradient system} in order to locate critical
points of the objective function (\ref{eq:final}):

\begin{equation}
 \dot{Q}(t)=-\nabla A(Q)\label{eq:gradientsystem}
\end{equation}

One can realize that this transformation preserves all of the
critical points \cite{Chiang96}. Now, we will describe the
construction of the gradient system and the Hessian in detail. In
order to reduce the dominance of one variable over the other, the
values of the each of the nucleotides that belong to the consensus
pattern at the position $k$ will be represented in terms of the
other three nucleotides in that particular column. Let $P_{ik}$
denote the $k^{th}$ position in the segment $P_i$. This will also
minimize the dominance of the eigenvector directions when the
Hessian is obtained. The variables in the scoring function are
transformed into new variables described in Table ~\ref{TB:hessian}.

\begin{equation}\label{eq:adsaq}
    A(Q)=\sum_{i=1}^t \sum_{k=1}^l log ~f_{ik}(w_{3k-2},w_{3k-1},w_{3k})_i
\end{equation}

where $f_{ik}$ can take the values \{$w_{3k-2}$, $w_{3k-1}$,
$w_{3k}$, $1-(w_{3k-2}+w_{3k-1}+w_{3k})$ \} depending on the $P_{ik}$ value.\\
%\begin{equation}
%\label{eq:scasereturn} f_{ik}=\begin{cases}
%~1-(w_{3k-2}+w_{3k-1}+w_{3k}) & \text{if $P_{ik}=C_k$} \\
%w_{3k-2}~ or~ w_{3k-1}~ or~ w_{3k} &\text{elsewhere}\\
%\end{cases}
%\end{equation}

\begin{table}[h]
\centering \caption{\protect\small A count of nucleotides $j \in
\{A,T,G,C\}$ at each position $k={1..l}$ in all the sequences of the
data set. $C_k$ is the $k^{th}$ nucleotide of the consensus pattern
which represents the nucleotide with the highest value in that
column. Let the consensus pattern be GACT...G and $b_j$ be the
background. }

\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline $j$ &  $k=b$& $k=1$&$ k=2$&$ K=3$ &$k=4$&~...~&  $k=l$\\
\hline

${A}$ & $b_A$ & $w_1$ &$C_2$ &$w_7$ &$w_{10}$ &... &$w_{3l-2}$\\
\hline

${T} $& $b_T$ & $w_2$ &$w_4$ &$w_8$ &$C_4$ &... &$w_{3l-1}$\\
\hline

${G}$ & $b_G$ & $C_1$ &$w_5 $&$w_9$ &$w_{11}$ &... &$C_l$\\
\hline

${C}$ & $b_C$ & $w_3$ &$w_6 $&$C_3$ &$w_{12}$ &... &$w_{3l}$\\
\hline

\end{tabular}
\end{center}
\label{TB:hessian}
\end{table}



The first derivative of the scoring function is a one dimensional
vector with $3l$ elements.
\begin{equation}\label{eq:beq}
    \nabla A= \left[~ \frac{\partial A}{\partial w_1} ~~ \frac{\partial A}{\partial w_2} ~~\frac{\partial A}{\partial w_3}
    ~~.~.~.~.~~~ \frac{\partial A}{\partial w_{3l}}
    ~\right]^T
\end{equation}

and each partial derivative is given by
\begin{equation}\label{eq:peq}
    \frac{\partial A}{\partial w_p}= \sum_{i=1}^t \frac{\frac{\partial f_{ip}}{\partial w_p}}{f_{ik}(w_{3k-2},w_{3k-1},w_{3k})}
\end{equation}
\begin{equation*}\label{eq:peq}
~~~~\forall p=1,2~...~3l~~and~~k=round(p/3)+1
\end{equation*}

The Hessian $\nabla^2 A$ is a block diagonal matrix of block size
3X3. For a given sequence, the entries of the 3X3 block will be the
same if that nucleotide belongs to the consensus pattern ($C_k$).
The gradient system is mainly obtained for enabling us to identify
the stability boundaries and stability regions on the likelihood
surface. The theoretical details of these concepts are published in
\cite{Chiang96}. The stability region of each local maximum is an
approximate convergence zone of the EM algorithm. If we can identify
all the saddle points on the stability boundary of a given local
maximum, then we will be able to find all the tier-1 local maxima.
However, finding all of the saddle points is computationally
intractable and hence we have adopted a heuristic by generating the
eigenvector directions of the PSSM at the local maximum. The next
section details our approach and explains the different phases of
our algorithm. In this problem, we will not trace the stability boundary for obtaining saddle points and hence, we call this as ``Exit-point" framework.

\subsection{Stability Region based Exit-point Framework}
\label{sec:algorithm}

Our framework consists of the following three phases:

\begin{itemize}

\item{{\it Global phase} in which the promising
solutions in the entire search space are obtained.} \item{{\it
Refinement phase} where a local method is applied to the solutions
obtained in the previous phase in order to refine the profiles.}
\item{{\it Exit phase} where the exit points are
computed and the Tier-1 and Tier-2 solutions are explored
systematically.}

\end{itemize}

In the global phase, a branch and bound search is performed on the
entire dataset. All of the profiles that do not meet a certain
threshold (in terms of a given scoring function) are eliminated in
this phase. The promising patterns obtained are transformed into
profiles and local improvements are made to these profiles in the
refinement phase. The consensus pattern is obtained from each
nucleotide that corresponds to the largest value in each column of
the PSSM.  The $3l$ variables chosen are the nucleotides that
correspond to those that are not present in the consensus pattern.
Because of the probability constraints discussed in the previous
section, the largest weight can be represented in terms of the other
three variables.




To solve (\ref{eq:final}), current algorithms begin at random
initial alignment positions and attempt to converge to an alignment
of $l-mer$s in all of the sequences that maximize the objective
function. In other words, the $l-mer$ whose $log(A)_i$ is the
highest (with a given PSSM) is noted in every sequence as part of
the current alignment. During the maximization of $A(Q)$ function,
the probability weight matrix and hence the corresponding alignments
of $l-mer$s are updated.  This occurs iteratively until the PSSM
converges to the local optimal solution. The consensus pattern is
obtained from the nucleotide with the largest weight in each
position (column) of the PSSM. This converged PSSM and the set of
alignments correspond to a local optimal solution. The exit phase
where the neighborhood of the original solution is explored in a
systematic manner is shown below:

%\begin{figure}
\textbf{Input:} Local Maximum (A).
\\\textbf{Output:} Best Local Maximum in the neighborhood region.
\\\textbf{Algorithm:}\\ {\it Step 1:} Construct the PSSM for the alignments corresponding to the local maximum (A) using Eqs.(\ref{eq:backcount}) and (\ref{eq:forecount}).
\\{\it Step 2:} Calculate the eigenvectors of the Hessian matrix for this PSSM.
\\{\it Step 3:} Find exit points ($e_{1i}$) on the practical stability boundary along each eigenvector direction.
\\{\it Step 4:} For each of the exit points, the corresponding Tier-1 local maxima ($a_{1i}$) are obtained by applying the EM algorithm after the ascent step.
\\{\it Step 5:} Repeat this process for promising Tier-1 solutions to obtain Tier-2 ($a_{2j}$) local maxima.
\\{\it Step 6:} Return the solution that gives the maximum information content score of $\{A,~a_{1i},~a_{2j}
\}$.\\
%\caption{The Exit phase where the neighborhood of the original
%solution is explored in a systematic manner.} \label{fig:alg1}
%\end{figure}


To escape out of this local optimal solution, our approach requires
the computation of a Hessian matrix (i.e. the matrix of second
derivatives) of dimension $(3l)^2$  and the $3l$ eigenvectors of the
Hessian. The main reasons for choosing the eigenvectors of the
Hessian as search directions are:
\begin{itemize}
\item{Computing the eigenvectors of the Hessian is related to finding
the directions with extreme values of the second derivatives, i.e.,
directions of extreme normal-to-isosurface change.}
\item{The eigenvectors of the Hessian will form the basis vectors for
the search directions. Any other search direction can be obtained by
a linear combination of these directions.} \item{This will make our
algorithm deterministic since the eigenvector directions are always
unique.}
\end{itemize}

The value of the objective function is evaluated along these
eigenvector directions with some small step size increments. Since
the starting position is a local optimal solution, one will see a
steady decline in the function value during the initial steps; we
call this the {\it descent stage}. Since the Hessian is obtained
only once during the entire procedure, it is more efficient compared
to Newton's method where an approximate Hessian is obtained for
every iteration. After a certain number of evaluations, there may be
an increase in the value indicating that the current point is out of
the convergence region of the local maximum. The point along this
direction where $A(Q)$ has the lowest value is called the {\it exit
point}. Once the exit point has been reached, few more evaluations
are made in the direction of the same eigenvector to ensure that one
has left the original region of convergence. This procedure is
clearly shown in Fig ~\ref{fig:summary}. Applying the local method
directly from the exit point may give the original local maximum.
The ascent stage is used to ensure that the new guess is in a
different convergence zone. Hence, given the best local maximum
obtained using any current local methods, this framework allows us
to systematically escape out of the local maximum to explore
surrounding local maxima. The complete algorithm is shown below :

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/summary.ps, width=3.5in}
} \caption {A summary of escaping out of the local optimum to the
neighborhood local optimum.  Observe the corresponding trend of
$A(Q)$ at each step.}

\label{fig:summary}
\end{figure}


%\begin{figure}[htp]
\textbf{Input:} The DNA sequences, length of the motif (l), Maximum
Number of Mutations (d) \\\textbf{Output:} Motif
(s)\\\textbf{Algorithm:}\\ {\it Step 1:} Given the sequences, apply
Random Projection algorithm to obtain different set of alignments.
\\{\it Step 2:} Choose the promising buckets and apply EM algorithm to
refine these alignments.
\\{\it Step 3:} Apply the exit point method to obtain nearby promising local optimal solutions. \\{\it Step 4:}
Report the consensus pattern that corresponds to the best alignments and their corresponding PSSM.\\
% \caption{The complete algorithm}
%\label{fig:alg2}
%\end{figure}


The new framework can be treated as a hybrid approach between global
and local methods. It differs from traditional local methods by
computing multiple local solutions in the neighborhood region in a
systematic manner. It differs from global methods by working
completely in the profile space and searching a subspace efficiently
in a deterministic manner. For a given non-convex function, there is
a massive number of convergence regions that are very close to each
other and are separated from one another in the form of different
basins of attraction. These basins are effectively modeled by the
concept of stability regions.

\subsection{Implementation Details}
\label{sec:implementation}

Our program was implemented on Red Hat Linux version 9 and runs on a
Pentium IV 2.8 GHz machine. The core algorithm that we have
implemented is $XP\_EM$ described in Algorithm ~\ref{complete}.
$XP\_EM$ obtains the initial alignments and the original data
sequences along with the length of the motif. It returns the best
motif that is obtained in the neighboring region of the sequences.
This procedure constructs the PSSM, performs EM refinement, and then
computes the Tier-1 and Tier-2 solutions by calling the procedure
$Next\_Tier$. The eigenvectors of the Hessian were computed using
the source code obtained from \cite{Press92}. $Next\_Tier$ takes a
PSSM as an input and computes an array of PSSMs corresponding to the
next tier local maxima using the exit point methodology.

\begin{algorithm}
\caption{Motif $XP\_EM$($init\_aligns,seqs,l$)} \label{complete}
\begin{algorithmic}
\STATE$PSSM = Construct\_PSSM(init\_aligns)$ \STATE $New\_PSSM=
Apply\_EM(PSSM, seqs)$\STATE $TIER1 = Next\_Tier (seqs, New\_PSSM,
l)$ \FOR{$i=1$ to $3l$} \IF{$TIER1[i]<>zeros(4l)$}
     \STATE $TIER2[i][~] = Next\_Tier (seqs,
TIER1[i], l)$   \ENDIF \ENDFOR \STATE Return $best(PSSM,TIER1,
TIER2)$
\end{algorithmic}
\end{algorithm}

Given a set of initial alignments, Algorithm \ref{complete} will
find the best possible motif in the neighborhood space of the
profiles. Initially, a PSSM is computed using $construct\_PSSM$ from
the given alignments. The procedure $Apply\_EM$ will return a new
PSSM that corresponds to the alignments obtained after the EM
algorithm has been applied to the initial PSSM. The details of the
procedure $Next\_Tier$ are given in Algorithm \ref{nexttier}. From a
given local solution (or PSSM), $Next\_Tier$ will compute all the
$3l$ new $PSSM$s in the neighborhood of the given local optimal
solution. The second tier patterns are obtained by calling the
$Next\_Tier$ from the first tier solutions \footnote {New PSSMs
might not be obtained for certain search directions. In those cases,
a zero vector of length $4l$ is returned. Only those new PSSMs which
do not have this value will be used for any further processing.}.
Finally, the pattern with the highest score amongst all the PSSMs is
returned.

\begin{algorithm}
\caption{PSSMs[~] $Next\_Tier$($seqs, PSSM,l$)} \label{nexttier}
\begin{algorithmic}
\STATE$Score=eval(PSSM)$ \STATE
$Hess=Construct\_Hessian(PSSM)$\STATE $Eig[~]=Compute\_EigVec
(Hess)$ \STATE $MAX\_Iter=100$

\FOR{$k=1$ to $3l$} \STATE $PSSMs[k]= PSSM~~~~~~Count=0$ \STATE
$Old\_Score=Score~~~~~~~~~ep\_reached=FALSE$

\WHILE{$(!~ep\_reached)~ \&\& ~(Count<MAX\_Iter)$} \STATE
$PSSMs[k]=update(PSSMs[k],Eig[k],step)$ \STATE $Count~=~Count~+~1$
\STATE $New\_Score~=~eval(PSSMs[k])$

\IF{$(New\_Score~>~Old\_Score)$} \STATE $ep\_reached=TRUE$ \ENDIF

\STATE $Old\_Score=New\_Score$
    \ENDWHILE
\IF{$count<MAX\_Iter$}
    \STATE $PSSMs[k]=update(PSSMs[k],Eig[k],ASC)$
\STATE $PSSMs[k]=Apply\_EM(PSSMs[k],Seqs)$ \ELSE \STATE
$PSSMs[k]=zeros(4l)$ \ENDIF \ENDFOR \STATE \bf Return $PSSMs[~]$
\end{algorithmic}
\end{algorithm}

The procedure $Next\_Tier$ takes a PSSM, applies the Exit-point
method and computes an array of PSSMs that corresponds to the next
tier local optimal solutions. The procedure $eval$ evaluates the
scoring function for the PSSM using (\ref{eq:final}). The procedures
$Construct\_Hessian$ and $Compute\_EigVec$ compute the Hessian
matrix and the eigenvectors respectively. $MAX\_iter$ indicates the
maximum number of uphill evaluations that are required along each of
the eigenvector directions. The neighborhood PSSMs will be stored in
an array variable $PSSMs[~]$. The original PSSM is updated with a
small step until an exit point is reached or the number of
iterations exceeds the $MAX\_Iter$ value. If the exit point is
reached along a particular direction, some more iterations are run
to guarantee that the PSSM has exited the original stability region
and has entered a new one. The EM algorithm is then used during this
ascent stage to obtain a new PSSM \footnote{ For completeness, the
entire algorithm has been shown in this section. However, during the
implementation, several heuristics have been applied to reduce the
running time of the algorithm. For example, if the first tier
solution is not very promising, it will not be considered for
obtaining the corresponding second tier solutions.}.

\begin{figure}
\centerline{
  \epsfig{figure=Figures/diagram3.ps, width=2.5in}
} \caption {Diagram illustrates the exit point method of escaping
from the original solution ($A$) to the neighborhood local optimal
solutions ($a_{1i}$) through the corresponding exit points
($e_{1i}$). The dotted lines indicate the local convergence of the
EM algorithm.}

\label{fig:diagram}
\end{figure}


The initial alignments are converted into the profile space and a
PSSM is constructed. The PSSM is updated (using the EM algorithm)
until the alignments converge to a local optimal solution. The
Exit-point methodology is then employed to escape out of this local
optimal solution to compute nearby first tier local optimal
solutions.  This process is then repeated on promising first tier
solutions to obtain second tier solutions. As shown in Fig.
\ref{fig:resultstier}, from the original local optimal solution,
various exit points and their corresponding new local optimal
solutions are computed along each eigenvector direction. Sometimes
two directions may yield the same local optimal solution. This can
be avoided by computing the saddle point corresponding to the exit
point on the stability boundary \cite{Reddy06}. There can be many
exit points, but there will only be a unique saddle point
corresponding to the new local minimum. However, in high dimensional
problems, this is not very efficient. Hence, we have chosen to
compute the exit points. For computational efficiency, the
Exit-point approach is only applied to promising initial alignments
(i.e. random starts with higher Information Content score).
Therefore, a threshold $A(Q)$ score is determined by the average of
the three best first tier scores after 10-15 random starts; any
current and future first tier solution with scores greater than the
threshold is considered for further analysis. Additional random
starts are carried out in order to aggregate at least ten first tier
solutions. The Exit-point method is repeated on all first tier
solutions above a certain threshold to obtain second tier solutions.


\begin{figure}
\centerline{
  \epsfig{figure=Figures/results2.ps, width=3.5in}
} \caption {2-D illustration of first tier improvements in a $3l$
dimensional objective function. The original local maximum has a
score of 163.375. The various Tier-1 solutions are plotted and the
one with highest score (167.81) is chosen.}

\label{fig:resultstier}
\end{figure}

\subsection{Experimental Results}
\label{sec:results} Experiments were performed on both synthetic
data and real data. Two different methods were used in the global
phase: random start and random projection. The main purpose of our work is not to demonstrate that our algorithm can outperform the
existing motif finding algorithms. Rather, the main work here
focuses on improving the results that are obtained from other
efficient algorithms. We have chosen to demonstrate the performance
of our algorithm on the results obtained from the random projection
method which is a powerful global method that has outperformed other
traditional motif finding approaches like MEME, Gibbs sampling,
WINNOWER, SP-STAR, etc. \cite{Buhler01}. Since the comparison was
already published, we mainly focus on the performance improvements
of our algorithm as compared to the random projection algorithm. For
the random start experiment, a total of $N$ random numbers between
$1$ and ($t-l+1$) corresponding to initial set of alignments are
generated. We then proceeded to evaluate our Exit-point methodology
from these alignments.




%\begin{table*}[htp]
%\centering \caption{\protect\small The consensus patterns and their
%corresponding scores of the original local optimal solution obtained
%by applying random projection method on the synthetics data. The
%best first tier and the second tier optimal solution are also
%reported. }
%
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%
%(l,d) &  Initial Pattern &Score&   First Tier Pattern&  Score&
%Second Tier Pattern &Score \\ \hline
%
%(11,2)&  TATCGCTGGGC& 147.5 &TAACGCTGGTC& 148.2 &  TCTCGCTGGGC&
%151.1 \\ \hline (13,3) & CACCTTGGTAATT& 168.4  & GACCTTGGGTATT&
%170.6& GACCATGGGTATT &171.5 \\ \hline(15,4) &ATGGCGTCCGCAATG &174.7
%&ATGGCGTCCGGAATA& 175.8& ATGGCGTCCGAAAGA& 178.5\\ \hline (17,5)&
%CGACACTTTCTCAATGT &  178.8& CGACACTTTCTCAATAT &182.8&
%CGACACTATCTTAAGAT  & 183.2\\ \hline (20,6) &TCAAATAGACTAGAGGCGAC&
%189.0 &TCTAATATAATGGAGGCTGC &   190.0& TCTACTAGACTGGAGGCGGC &191.1\\
%\hline
%
%\end{tabular}
%\end{center}
%\label{TB:real_res}
%\end{table*}

\subsubsection {Synthetic Datasets}
The synthetic datasets were generated by implanting some motif
instances into $t=20$ sequences each of length 600. Let $m$
correspond to one full random projection + EM cycle. We have set
$m=1$ to demonstrate the efficiency of our approach. We compared the
performance coefficient (PC) which gives a measure of the average
performance of our implementation compared to that of Random
Projection. The PC is given by :

\begin{equation}\label{eq:pc}
    PC=\frac{|K \cap P|}{|K \cup P|}
\end{equation}

where K is the set of the residue positions of the planted motif
instances, and P is the corresponding set of positions predicted by
the algorithm. Table \ref {TB:syn_das} gives an overview of the
performance of our method compared to the random projection
algorithm on the ({\it l,d}) motif problem for different {\it l} and
{\it d} values.


Our results show that by branching out and discovering multiple
local optimal solutions, higher $m$ values are not needed. A higher
$m$ value corresponds to more computational time because projecting
the $l$-mers into $k$-sized buckets is a time consuming task. Using
our approach, we can replace the need for randomly projecting {\it
l}-mers repeatedly in an effort to converge to a global optimum by
deterministically and systematically searching the solution space
modeled by our dynamical system and improving the quality of the
existing solutions. The improvements of our algorithm are clearly
shown in Table \ref{TB:syn_das}. We can see that for higher length
motifs, the improvements are more significant.



Fig. \ref{fig:resultstier} shows the Tier-1 solutions obtained from
a given consensus pattern. Since the exit points are being used
instead of saddle points, our method might sometimes find the same
local optimal solution obtained before. As seen from the figure, the
Tier-1 solutions can differ from the original pattern by more than
just one nucleotide position. Also, the function value at the exit
points is much higher than the original value.


\begin{table*}[htp]
\centering \caption{\protect\small  The consensus patterns and their
corresponding scores of the original local optimal solution obtained
from multiple random starts on the synthetic data. The best first
tier and second tier optimal patterns and their corresponding scores
are also reported. }
\begin{tiny}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline

(l,d) &  Initial Pattern &Score&   First Tier Pattern&  Score&
Second Tier Pattern &Score \\ \hline

(11,2)&  AACGGTCGCAG &125.1& CCCGGTCGCTG& 147.1& CCCGGGAGCTG
&153.3\\ \hline (11,2)&
ATACCAGTTAC &145.7 &ATACCAGTTTC &151.3 &ATACCAGGGTC& 153.6 \\
\hline(13,3)& CTACGGTCGTCTT &  142.6 &CCACGGTTGTCTC &157.8&
CCTCGGGTTTGTC &  158.7\\ \hline (13,3)&  GACGCTAGGGGGT& 158.3&
GAGGCTGGGCAGT &161.7 &  GACCTTGGGTATT& 165.8\\ \hline (15,4)&
CCGAAAAGAGTCCGA& 147.5& CCGCAATGACTGGGT& 169.1& CCGAAAGGACTGCGT&
176.2\\ \hline (15,4)& TGGGTGATGCCTATG& 164.6& TGGGTGATGCCTATG&
166.7& TGAGAGATGCCTATG& 170.4\\ \hline (17,5) &TTGTAGCAAAGGCTAAA&
143.3 &CAGTAGCAAAGACTACC &  173.3& CAGTAGCAAAGACTTCC &  175.8\\
\hline (17,5)& ATCGCGAAAGGTTGTGG  & 174.1& ATCGCGAAAGGATGTGG &176.7
&ATTGCGAAAGAATGTGG &  178.3\\ \hline (20,6)& CTGGTGATTGAGATCATCAT&
165.9& CAGATGGTTGAGATCACCTT &   186.9& CATTTAGCTGAGTTCACCTT  & 194.9
\\ \hline(20,6)& GGTCACTTAGTGGCGCCATG &216.3& GGTCACTTAGTGGCGCCATG&
218.8& CGTCACTTAGTCGCGCCATG &   219.7\\ \hline

\end{tabular}
\end{center}
\end{tiny} \label{TB:syn_res}
\end{table*}


As opposed to stochastic processes like mutations in genetic
algorithms, our approach reduces the stochastic nature and obtains
the nearby local optimal solutions systematically. Fig.
\ref{fig:syn_rs} shows the performance of the Exit-point approach on
synthetic data for different ({\it l,d}) motifs. The average scores
of the ten best solutions obtained from random starts and their
corresponding improvements in Tier-1 and Tier-2 are reported. One
can see that the improvements become more prominent as the length of
the motif is increased. Table \ref{TB:syn_res} shows the best and
worst of these top ten random starts along with the consensus
pattern and the alignment scores.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/syn_rs.ps, width=3.2in}
} \caption {The average scores with the corresponding first tier and
second tier improvements on synthetic data using the random starts
with Exit-point approach with different ({\it l,d}) motifs.}
\label{fig:syn_rs}
\end{figure}

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/syn_rp.ps, width=3.2in}
} \caption {The average scores with the corresponding first tier and
second tier improvements on synthetic data using the Random
Projection with Exit-point approach with different ({\it l,d})
motifs.} \label{fig:syn_rp}
\end{figure}

\begin{table}[htp]
\centering \caption{\protect\small The results of performance
coefficient with $m=1$ on synthetically generated sequences. The IC
scores are not normalized and the perfect score is 20 since there
are 20 sequences. }
\begin{center}
\begin{tabular}{|c|c|c|}
\hline

Motif  &  PC obtained using &PC obtained using\\
(l,d) &  Random Projection &Exit-point method \\ \hline

(11,2)&  20& 20 \\  \hline(15,4) &14.875 &17\\  \hline (20,6)
&12.667&18\\ \hline
\end{tabular}
\end{center}
\label{TB:syn_das}
\end{table}


With a few modifications, more experiments were conducted using the
Random Projection method.  The Random Projection method will
eliminate non-promising regions in the search space and gives a
number of promising sets of initial patterns. EM refinement is
applied to only the promising initial patterns. Due to the
robustness of the results, the Exit-point method is employed only on
the top five local optima. The Exit-point method is again repeated
on the top scoring first tier solutions to arrive at the second tier
solutions. Fig. \ref{fig:syn_rp} shows the average alignment scores
of the best random projection alignments and their corresponding
improvements in tier-1 and tier-2 are reported. In general, the
improvement in the first tier solution is more significant than the
improvements in the second tier solutions.
%Table ~\ref{TB:real_res} reports the best
%initial alignment and tier-1 and tier-2 improvements using random
%projection along with the consensus pattern and their corresponding
%scores.

\subsubsection{Real Datasets}

Table~\ref{TB:realdata} shows the results of the Exit-point
methodology on real biological sequences. We have chosen $l=20$ and
$d=2$. `{\it t}' indicates the number of sequences in the real data.
For the biological samples taken from \cite {Buhler01,Price03}, the
value $m$ once again is the average number of random projection + EM
cycles required to discover the motif. All other parameter values
(like projection size $k=7$ and threshold $s$=4) are chosen to be
the same as those used in the Random projection paper
\cite{Buhler01}. All of the motifs were recovered with $m=1$ using
the Exit-point strategy. Without the exit point strategy, the Random
Projection algorithm needed {\it multiple cycles} (m=8 in some cases
and m=15 in others) in order to retrieve the correct motif. This
elucidates the fact that global methods can only be used to a
certain extent and should be combined with refined local heuristics
in order to obtain better efficiency. Since the random projection
algorithm has outperformed other prominent motif finding algorithms
like SP-STAR, WINNOWER, Gibbs sampling etc., we did not repeat the
same experiments that were conducted in \cite{Buhler01}. Running one
cycle of random projection + EM is much more expensive
computationally. The main advantage of our strategy comes from the
deterministic nature of our algorithm in refining motifs.

\begin{table*}[htp]
\centering \caption{\protect\small Results of Exit-point method on
biological samples. The real motifs were obtained in all the six
cases using the Exit-point framework.}
\begin{tiny}
\begin{center}
%\begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}|c|c|c|c|c|c|}
\begin{tabular}{|c|c|c|c|c|}
\hline

\textbf{Sequence} &\textbf{Sample Size}&\textbf{t}& \textbf{ Best
(20,2) Motif }&\textbf{ Reference Motif} \\\hline
E. coli CRP & 1890 & 18 &\underline {TGTGAAATAGATCACA}TTTT &TGTGANNNNGNTCACA \\
preproinsulin& 7689 &4 & GGAAATTGCAG\underline{CCTCAGCCC}& CCTCAGCCC \\
DHFR &800& 4&  CTGCA\underline{ATTTCGCGCCA}AACT& ATTTCNNGCCA \\
metallothionein &6823& 4 & CCCTC\underline{TGCGCCCGG}ACCGGT& TGCRCYCGG \\
c-fos &3695& 5&  \underline{CCATATTAGGACATCT}GCGT &CCATATTAGAGACTCT \\
yeast ECB& 5000 &5 &GTA\underline{TTTCCCGTTTAGGAAA}A
&TTTCCCNNTNAGGAAA \\ \hline
\end{tabular}
\end{center}
\end{tiny}
\label{TB:realdata}
\end{table*}



%This Exit Point framework has also been tested on real human
%sequences. Usually the real data sets contain a lot more overly
%expressed patterns which are often meaningless and the background
%frequencies are not evenly distributed. The length of the motif is
%usually not known in the real data. We tried to obtain the various
%motifs from real human DNA sequences using the Exit-point approach.
%Fig 7 summarizes our results on the real data. Motifs with different
%(l,d) values are retrieved and the bar charts indicate the alignment
%scores of the original and the best tier-1 and tier-2 solutions. As
%seen from the figure, there is a significant improvement in the
%scores for different motifs. Only the best solution is analyzed
%further due to computational time constraints while using the real
%data.
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/real_rs.ps, width=3.5in}
%} \caption{The average scores with the corresponding first tier and
%second tier improvements on real sequences using the random starts
%with exit point approach with different (l,d) motifs.}
%\label{fig:real_rs}
%\end{figure}

The Exit-point framework broadens the search region in order to obtain an improved
solution which may potentially correspond to a better motif. In most
of the profile based algorithms, EM is used to obtain the nearest
local optimum from a given starting point. In our approach, we
consider the boundaries of these convergence regions and find the
surrounding local optimal solutions based on the theory of stability
regions. We have shown on both real and synthetic data sets that
beginning from the EM converged solution, the Exit-point approach is
capable of searching in the neighborhood regions for another
solution with an improved information content score. This will often
translate into finding a pattern with less hamming distance from the
resulting alignments in each sequence. Our approach has demonstrated
an improvement in the score on all datasets that it was tested on.
One of the primary advantages of the Exit-point methodology is that
it can be used with different global and local methods. The main
contribution of our work is to demonstrate the capability of this
hybrid EM algorithm in the context of the motif finding problem. Our
algorithm can potentially use any global method and improve its
results efficiently. From our results, we see that motif refinement stage plays a vital
role and can yield accurate results deterministically. We would like
to continue our work by combining other global methods available in
the literature with existing local solvers like EM or GibbsDNA that
work in continuous space. By following the example of
\cite{Tompa05}, we may improve the chances of finding more promising
patterns by combining our algorithm with different global and local
methods.




==> orig/problem.tex <==
\chapter {Problem Formulation}
\label{ch:problem}

This chapter discusses the details of our framework that has been designed for solving various problems in global optimization.

Any global optimization method will consist of a global method which primarily explores the entire search space.
Its main duty is select some promising areas in the search space which has a very high potential of containing the global minima.

It is usually followed by a local method which will converge to the local minima in that area. In this dissertation, we combine them along with a new hybrid method
which guarantees a better local minima than the existing one. This is done by the concept of {\it escaping from the existing local minima}/
This chapter contains the details about these methods. The algorithms used as global method is described in section ~\ref{sec:global}.

\section {Transformation of the solution space}
\label{sec:transform}

\subsection{Selection}
\label{sec:selection}

High-fitness individuals have a better chance of reproducing,
while low-fitness ones are more likely to disappear. Selection
alone cannot introduce any new individuals into the population,
i.e., it cannot find new points in the search space. Crossovers
and mutations are used to explore the solution space. Selection is
mainly responsible for determining the convergence characteristics
of Genetic algorithms. {\it Selection pressure} is the degree to
which the best individuals are favoured. The higher the selection
pressure, the more the best individuals are favoured. The
convergence rate of a GA is largely determined by the magnitude of
the selection pressure.

\subsection{Crossover}
\label{sec:crossover}

crossover is nothing but a recombination (mating) of two
individuals. This can be performed by exchanging parts of the
strings to form new individuals (children). Crossover is a
controversial operator due to its disruptive nature(i.e., it can
split important information). No definite answer about the
necessity of using the crossover has been reached so far.  Besides
GAs, other evolutionary algorithms do not rely on crossovers.

\subsection{Mutation}
\label{sec:mutation} There is a growing recognition of the
importance of mutation in contrast with viewing it as responsible
for re-introducing inadvertently lost gene values. A mutation
operator is more important at the final generations when the
majority of the individuals present similar quality. A variable
mutation rate is very important for search efficiency. Its setting
is much more critical than that of crossover rate. For real-valued
encoding, the mutation operator can be implemented by random
replacement, i.e. replace the value with a random one. Mutation
can also be used as hill climbing mechanism.

The details of how these concepts of genetic algorithms are used
in our algorithm to determine the structure is clearly illustrated
in subsection.

Before we proceed further with the discussion about the algorithm,
we need to define some terms and initialize certain threshold
values that we will be using in further sections. Let $r_{ij}$ be
the Euclidean distance between the two conformations $i$ and $j$.
Let $r_{t}$ be the threshold distance. Basically, these two
variables will make sure that the two conformations $i$ and $j$
will not give any repetitive information. In this way, a pool of m
solutions are generated randomly. Each solution consists of a
string of 3N coordinates \footnote {Even though the problem is
originally of 3N dimensions (where N is the cluster size), the
optimization for the global minimum structure is done in (3N-6)
dimensional space. However, it is not a consideration for our
discussion here because we are only trying to estimate the minimum
energy. The remaining 6 degrees of freedom are due to the
rotational and translational variants of the original structure}.
This pool of solutions is called the {\it Bank}. Based on the
values of $r_{ij} $ between the two conformations, the new
conformations are either accepted or rejected. This is the {\it
selection step} of the GA which necessarily says that only the fit
species will survive. If $r_{ij}>r_t$, then $i$ constitutes a new
group. The lowest-energy representatives from each group within
the bank, including the new $i$ group, are then compared and the
worst conformation (i.e. the highest-energy conformation) is
discarded. Therefore, the size of the bank always remains
constant.

\subsection{Estimating Promising Locations}
\label{sec:aspects}

As described earlier, the selection operator will increase the
average fitness of the solution pool but does not introduce any
new features of variations to the bank. The flowchart of the
algorithm that is used here is shown in Figure
\ref{fig:flowchart}. Select a few number of dissimilar solutions
from the bank ({\it seeds}). Extensive changes should take place
in this trial of solutions if we want to achieve the global
solution. To do this, we invoke the {\it crossover} operator. With
certain cross over probability ($p_c$), a pair of trial solutions
$S_1$ and $S_2$ are transformed into a new pair of solutions
$S_1'$ and $S_2'$. This is done by shuffling each of the
coordinates in the original pair based on the crossover
probability variable. Once, the cross over is performed in the
solution space, it will undergo {\it mutation}. Let $p_m$ be the
mutation probability variable and $p_r$ be a random number
generated between 0 and 1. If $p_m>p_r$, then that particular
coordinate will be mutated. These three phases complete the
generation of the genetic algorithm and the process is usually
repeated for a pre-specified number of times.


\section {Properties of Nonlinear Manifolds}
\label{sec:properties}


==> orig/protein.tex <==
\section {Protein Folding Problem} \label{sec:proteinfolding}


==> orig/results.tex <==
\chapter {Experimental Results} \label{ch:results} This chapter
shows some results obtained from our system. Section ~\ref
{sec:rescalib} gives the results of the calibration process.
Frames from synthesized virtual videos are shown in Section ~\ref
{sec:resvirt}. Some preliminary results of the face modeling are
shown in Section ~\ref {sec:res3d}

\section {Calibration}
\label {sec:rescalib}

Section ~\ref {sec:vvs} describes the results obtained during the
calibration of the virtual video synthesis. The calibration
results for the 3D face modeling are described in Section ~\ref
{sec:face}

\subsection {Virtual Video Synthesis}
\label {sec:vvs}

During the calibration, a rectangular grid of dimension 400 x 400
is projected onto the face. The grid is made by repeating three
colored lines. Colored lines were used because it is easy to
distinguish the lines (see Figure ~\ref{fig:grid})on the captured
side views. We used white, green and cyan colors for this purpose.
These colors were chosen because of their bright appearance over
the skin color. The first few frames will have the grid projected
onto the face and then the grid is turned off. One of the frames
with the grid is taken and the transformation tables are
generated. We calculate the transform functions represented by
Equations ~\ref{eq:st} and ~\ref {eq:uv} from the grid coordinates
in both side views and the original grid coordinates. Each pixel
in the frontal virtual grid is then obtained from the
corresponding inverse transform functions.

The size of the grid pattern that is projected in the calibration
stage plays a significant role in the quality of the video. This
size is decided based on the trade-off between the quality of the
video and the time taken. An appropriate grid size has be chosen
based on trial and error. We started by projecting a sparse grid
pattern onto the face and then increasing the density of the grid
pattern. At one point, the increase in the density does not
significantly improve the quality of the face image but starts
consuming more time. At that point, the grid is finalized. Also,
this grid is decided based upon the average face size. In our
experiments, we settled on a grid cell size of row-width of 24
pixels and column-width of 18 pixels.

\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/grid.ps, width=3.5in} }
\caption{A square grid with alternating three colors is projected
onto the face. Each grid cell has a row-width =24 pixels,
col-width=18 pixels.} \label{fig:grid}
\end{figure}

Figure ~\ref {fig:calibrationfaces} shows the frames that are
captured during the calibration stage of the experiment.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/left_calib_face.ps, width=2.5in}
  \hspace{0.3in} \epsfig{figure=Figures/right_calib_face.ps, width=2.5in}
}
 \caption{Face images captured during the calibration stage using environment-static FCS}
 \label{fig:calibrationfaces}
\end{figure}

\subsection {Face Modeling}
\label {sec:face} As discussed earlier (Section
~\ref{sec:calib3df}), to apply the structure from stereo method,
we need to calibrate both cameras and the projector with respect
to WCS. We shall now discuss the results of the cameras and
projector calibration.

\subsubsection {Camera Calibration}
This section shows some of the sample results of the camera and
projector calibration procedures that were discussed in Section
~\ref{sec:calib3df}. Figure ~\ref {fig:cameracalib} shows some of
the images of the calibration sphere that were captured from the
left camera and the right camera during the calibration stage.

\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/leftcalibsphere.ps,
width=2.5in}
  \hspace{0.8in} \epsfig{figure=Figures/rightcalibsphere.ps, width=2.5in}}
 \caption{
The images that are captured from the left camera and the right
camera during the camera calibration.} \label{fig:cameracalib}
\end{figure}

Equations ~\ref {eq:leftcameramatrix} and ~\ref {eq:rightcameramatrix} shows the camera matrices obtained from the 12 calibration points shown in Figure ~\ref {fig:cameracalib}.\\

\begin{equation}
\centerline {$\displaystyle
\left[ \begin{matrix}  32.150  &  0.921  &  8.699 & 135.927\\    2.809 & -32.033 &  -4.347 & 124.153  \\    0.015 &   0.003 &  -0.023 & 1.000\\
\end{matrix}\right]$} \label{eq:leftcameramatrix}
\end{equation}

\begin{equation}
\centerline {$\displaystyle
\left[ \begin{matrix} 28.197  &  1.474  &-16.748 & 164.733\\   -0.509 & -32.143 &  -4.232 & 118.646   \\         -0.011  &  0.002 &  -0.023  &  1.000\\
\end{matrix}\right]$} \label{eq:rightcameramatrix}
\end{equation}

After obtaining the calibration matrices using the methods
described in the previous chapter, one can evaluate the accuracy
of these matrices using the calibration points as test points.
Estimation of these calibration points in the 2D image can be done
using the given 3D coordinates of the calibration points and the
calibration matrix. The difference in the actual 2D image
coordinates of these calibration points and the estimated values
of the 2D image coordinates is termed the ``residual". Table ~\ref
{TB:leftcalib} shows the residuals obtained while calibrating the
left camera.
\begin{table}[htp]
  \centering \caption{\protect\small Results of left camera
  calibration for points on the calibration sphere.}
   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{6}{|c|}{INPUT DATA} & \multicolumn{5}{c|}{OUTPUT
DATA} \\\hline

Point & \multicolumn{2}{c|}{2D Image} & \multicolumn{3}{c|}{3D
Coordinates}& \multicolumn{2}{c|}{2D Fit Data} &
\multicolumn{3}{c|}{Residuals} \\ \cline{2-11}

 & u & v & x & y & z &  $u^1$ & $v^1$ & $u_{error}$ &
$v_{error}$  & $Total_{error}$ \\ \hline

A & 198 & 116 & 0.00 & 0.00 & 4.65 &  198.0 & 116.7 & 0.0 & -0.7 &
0.7 \\ \hline

B & 190 & 36 &  0.00 & 2.33 & 4.03 & 189.8 & 35.3 & 0.2 & 0.7 &
0.9  \\ \hline

C & 135 & 56 & -1.64 & 1.64 & 4.03 & 135.0 & 55.7 & -0.0 & 0.3 &
0.3 \\ \hline

D & 109 & 115 & -2.33  & 0.00 & 4.03 & 110.4 & 114.9  & -1.4 & 0.1
& 1.5 \\ \hline

E & 134 & 176 & -1.64 & -1.64 & 4.03 & 132.9 & 176.4 & 1.1 & -0.4
& 1.5 \\ \hline

F & 187  & 202 & 0.00 & -2.33  & 4.03 & 187.7 &  201.4 & -0.7 &
0.6 & 1.3  \\ \hline

G & 240 & 177 & 1.64 & -1.64 & 4.03 & 240.3 & 177.2 & -0.3 & -0.2
& 0.5
\\ \hline
H & 262 & 121 & 2.33 & 0.00 & 4.03 & 261.6 & 120.5  & 0.4 & 0.5 &
0.9  \\ \hline

I & 241 & 62 & 1.64 & 1.64 & 4.03 & 241.3 & 62.7 & -0.3 & -0.7 &
1.0\\ \hline

K & 74 &16 & -2.85 &2.85 & 2.33 & 73.8 & 16.3 &  0.2 & -0.3 & 0.5
\\ \hline

L & 30 & 116 & -4.03 & 0.00 & 2.33 & 30.1 & 115.9  & -0.1 & 0.1 &
0.2 \\\hline

M & 69 & 220 & -2.85 & -2.85 & 2.33 & 69.2 & 220.1 & -0.2 & -0.1 &
0.3 \\ \hline
  \end{tabular}
\label{TB:leftcalib}
\end{table}

%
%
%\begin{table}[htp]
%  \centering   \caption{\protect\small Results of Right Camera Calibration}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
%\multicolumn{6}{|c|}{INPUT DATA} & \multicolumn{5}{c|}{OUTPUT
%DATA} \\\hline
%
%Point & \multicolumn{2}{c|}{2D Image} & \multicolumn{3}{c|}{3D
%Coordinates}& \multicolumn{2}{c|}{2D Fit Data} &
%\multicolumn{3}{c|}{Residuals} \\ \cline{2-11}
%
% & u & v & x & y & z &  $u^1$ & $v^1$ & $u_{error}$ &
%$v_{error}$  & $Total_{error}$ \\ \hline
%
%A & 97 & 110 & 0.00 & 0.00 & 4.65 &   97.3 & 110.9 &-0.3 & -0.9 &
%1.2 \\ \hline
%
%B & 111 & 29 & 0.00 & 2.33 & 4.03 &  110.5 & 29.5  & 0.5& -0.5 &
%1.0 \\ \hline
%
%C & 58 & 54 & -1.64 & 1.64 & 4.03 &   57.5 & 53.4& 0.5 & 0.6 & 1.1
%\\ \hline
%
%D &  33 & 111 & -2.33 & 0.00 & 4.03 & 34.0 & 110.2 & -1.0& 0.8&
%1.8\\ \hline
%
%E & 53 & 167 & -1.64 & -1.64 & 4.03 & 52.6 & 168.3 & 0.4 & -1.3 &
%1.7 \\ \hline
%
%F & 104 & 196 & 0.00 & -2.33 & 4.03 & 104.0 & 195.3 & 0.0 & 0.7 &
%0.7 \\ \hline
%
%G & 160 & 173 & 1.64 & -1.64 & 4.03  & 159.4 & 173.4 & 0.6 & -0.4
%& 1.0 \\ \hline
%
%H & 185  & 115 &  2.33 & 0.00 & 4.03  & 184.8 &  114.0 & 0.2 & 1.0
%& 1.2 \\ \hline
%
%I &163  & 54 & 1.64 & 1.64 & 4.03 &  163.8 & 53.7 & -0.8 & 0.3 &
%1.1 \\ \hline
%
%O & 222 & 219 & 2.85 & -2.85 & 2.33 &  222.0 & 218.7 &0.0& 0.3
%&0.3 \\ \hline
%
%P &265 &118&  4.03& 0.00 &2.33 & 265.5&  118.4 &    -0.5 &-0.4
%&0.9 \\ \hline
%
%Q &229 &17 &2.85 & 2.85&  2.33 & 228.6 & 17.2 & 0.4 &-0.2 &0.6\\
%\hline
%\end{tabular}
%
%\label{TB:rightcalib}
%\end{table}
%
\subsubsection {Calibration of the Projector}
The Table ~\ref {TB:projcalib} shows the errors in the calibration
of the projector. The errors are slightly higher when compared to
both cameras. Perhaps, these errors might have been due to the
radial distortion of the projector. Also in the case of the
projector, all the 17 calibration points (shown in Figure ~\ref
{fig:label_sphere}) are chosen for calibration.  The main
difference in the case of the projector when compared with the
previously discussed camera calibration method is that the (u,v)
coordinates are obtained by projecting an image with known image
points onto the 3D calibration points. The mouse was used to click
on the 2D image that is projected onto the 3D world points.
Equation
~\ref {eq:projectorcalibmatrix} shows the projector calibration matrix.\\

\begin{equation}
\centerline {$\displaystyle
\left[ \begin{matrix}    35.434 &   0.613   &-9.550 & 512.584\\      0.256  &-35.130 & -11.145&  449.176  \\   0.000  &  0.000 &  -0.018  &  1.000\\
\end{matrix}\right]$} \label{eq:projectorcalibmatrix}
\end{equation}

\begin{table}[htp]
  \centering \caption{\protect\small Results of projector calibration for points on the calibration sphere.}
   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{6}{|c|}{INPUT DATA} & \multicolumn{5}{c|}{OUTPUT
DATA} \\\hline

Point & \multicolumn{2}{c|}{2D Image} & \multicolumn{3}{c|}{3D
Coordinates}& \multicolumn{2}{c|}{2D Fit Data} &
\multicolumn{3}{c|}{Residuals} \\ \cline{2-11}

 & u & v & x & y & z &  $u^1$ & $v^1$ & $u_{error}$ &
$v_{error}$  & $Total_{error}$ \\ \hline

A & 511 & 432 & 0.00 & 0.00 & 4.65  & 510.3 & 433.1 &     0.7   &  -1.1& 1.8\\
\hline

B & 512 & 348 & 0.00 &2.33 &4.03 & 511.9 &  347.3 & 0.1 &0.7 &0.8
\\ \hline

C & 449 & 373 &-1.64& 1.64& 4.03 &448.9 & 372.7 & 0.1& 0.3 & 0.4
\\ \hline

D & 420 &435 & -2.33 & 0.00 & 4.03 & 422.0 & 434.8 & -2.0 & 0.2 &
2.2 \\ \hline

E & 448 &496 &-1.64 & -1.64 &4.03&  447.0 &  497.4 &1.0
&-1.4 &2.4 \\
\hline

F &509 &524& 0.00& -2.33& 4.03  &509.4  &523.7 &    -0.4 & 0.3 &
0.7\\ \hline


G & 573 & 498 & 1.64 &-1.64 & 4.03 &  572.4 & 498.2 & 0.6& -0.2&    0.8\\
\hline

H & 600& 437 & 2.33 &-0.00& 4.03&  599.3 & 436.0  & 0.7&
1.0 &   1.7 \\
\hline

I&573 & 374 & 1.64& 1.64 & 4.03&   574.2& 373.5  & -1.2 &0.5 & 1.7
\\ \hline

J & 513 & 292 &0.00& 4.03& 2.33  & 513.6  &293.7  & -0.6& -1.7
&2.3\\ \hline

K&409 & 336& -2.85 &2.85& 2.33  & 407.9 & 336.2  & 1.1& -0.2
&1.3\\ \hline

L&363 & 441 &-4.03 &0.00 &2.33  & 362.7  &440.5  & 0.3& 0.5& 0.8
\\ \hline

M&405 & 547& -2.85 &-2.85& 2.33 &  404.8  &545.5 &     0.2 &1.5 &1.7 \\
\hline

N&508 & 588 &0.00& -4.03 &2.33  &  509.4&  589.6&     -1.4 &-1.6 &3.0\\
\hline

O&616 & 548& 2.85& -2.85& 2.33  & 615.2 & 546.8  & 0.8& 1.2 &2.0\\
\hline

P&660 & 441 & 4.03 & 0.00 & 2.33  &660.2 & 442.4 &    -0.2  &   -1.4 &1.6\\
\hline


Q&618 & 339 &2.85 &2.85 &2.33 &  618.1&  337.6  &   -0.1   &   1.4  &  1.5\\
\hline

  \end{tabular}
\label{TB:projcalib}
\end{table}


\section {Virtual Video Synthesis}
\label {sec:resvirt} This section discusses the results of the
virtual video synthesis algorithm that is described in Section
~\ref {sec:virtualview}. It also discusses the synchronization
issues that might affect the quality of the novel virtual views.

\subsection {Face Warping}
The results \footnote {If this thesis work was accessed through
the University Microfilm (UMI) database, the images will not be in
color. Even though the color information is lost, the author feels
that the concept is well explained using gray scale images.} of
the warping during the calibration and the operation stage is
shown in Figure ~\ref {fig:warpingresults}.

\begin{figure}[htp]
\centerline{
 \epsfig{figure=Figures/warping.ps, width=5.0in}
} \hspace{0.9in} (a) \hspace{1.1in} (b) \hspace{1.0in} (c)
\hspace{1.0in} (d)\\
\caption{Frontal view generation during the calibration stage and
reconstruction of the frontal image from the side view using the
grid: (a) left image captured during the calibration stage. (b)
virtual image constructed using the transformation tables and the
right image during the calibration stage. (c) right image captured
during the operational stage. (d) result of the reconstructed
frontal view from the transformation tables and the right image
during the operational stage} \label{fig:warpingresults}
\end{figure}

\subsection {Virtual View Synthesis}
Figure ~\ref{fig:originalvirtual} shows the output image of the
frontal view that is generated by our algorithm. This output is
obtained by applying our warping and mosaicking algorithms to the
left and right views shown in Figure ~\ref {fig:priresult}.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/demo/leftframe2.ps, width=2.0in}
 \hspace{1.0in} \epsfig{figure=Figures/demo/rightframe2.ps, width=2.0in}
} \caption{Face images captured during the operational phase using
the ESFCS } \label{fig:priresult}
\end{figure}

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/demo/realframe2.ps, width=2.0in,height=2.2in}
 \hspace{1.0in} \epsfig{figure=Figures/demo/virtualframe2.ps, width=2.0in,height=2.2in}
}

\caption{(a) Frontal view that is obtained from the camcorder and
(b) virtual frontal view generated from our algorithm }
\label{fig:originalvirtual}
\end{figure}

Figure ~\ref {fig:hmdpriresult} shows the side views of the human
face captured using the HMFCS. The main problems of capturing the
faces using HMFCS are:
\begin {enumerate}
\item Lighting variations
\item Distortion caused by the mirrors
\item Vibrations of the cameras and the mirrors
\end{enumerate}

\begin{figure}[htp] \centerline{
  \epsfig{figure=Figures/left_face_hmd.ps, width=2.5in}
  \hspace{0.3in} \epsfig{figure=Figures/right_face_hmd.ps, width=2.5in}
}

\caption{Face images captured using the HMFCS (a) left image and
(b) right image } \label{fig:hmdpriresult}
\end{figure}

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/real_face_hmd.ps, width=2.0in}
} \caption{Virtual frontal view generated from the side views
captured through HMFCS} \label{fig:hmdoriginalvirtual}
\end{figure}

Figure ~\ref{fig:hmdoriginalvirtual} shows the output of the
virtual view generated from the images captured using HMFCS.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/demo/leftframe1.ps, width=1.0in, height=0.9in}
 \hspace{0.08in} \epsfig{figure=Figures/demo/leftframe6.ps, width=1.0in, height=0.9in}
 \hspace{0.08in}   \epsfig{figure=Figures/demo/leftframe3.ps, width=1.0in, height=0.9in}
 \hspace{0.08in} \epsfig{figure=Figures/demo/leftframe4.ps, width=1.0in, height=0.9in}
 \hspace{0.08in}   \epsfig{figure=Figures/demo/leftframe5.ps, width=1.0in, height=0.9in}
   } \vspace{0.2in} \centerline{
  \epsfig{figure=Figures/demo/rightframe1.ps, width=1.0in, height=0.9in}
 \hspace{0.081in} \epsfig{figure=Figures/demo/rightframe6.ps, width=1.0in, height=0.9in}
 \hspace{0.08in}   \epsfig{figure=Figures/demo/rightframe3.ps, width=1.0in, height=0.9in}
 \hspace{0.08in} \epsfig{figure=Figures/demo/rightframe4.ps, width=1.0in, height=0.9in}
 \hspace{0.08in}   \epsfig{figure=Figures/demo/rightframe5.ps, width=1.0in, height=0.9in}
 }
\vspace{0.2in} \centerline{
     \epsfig{figure=Figures/demo/realframe1.ps, width=1.0in, height=1.1in}
 \hspace{0.1in} \epsfig{figure=Figures/demo/realframe6.ps, width=1.0in,height=1.1in}
\hspace{0.1in}\epsfig{figure=Figures/demo/realframe3.ps,width=1.0in,height=1.1in}
 \hspace{0.1in} \epsfig{figure=Figures/demo/realframe4.ps, width=1.0in,height=1.1in}
\hspace{0.1in}\epsfig{figure=Figures/demo/realframe5.ps, width=1.0in,height=1.1in} \\
   } \vspace{0.2in} \centerline{
     \epsfig{figure=Figures/demo/virtualframe1.ps, width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/demo/virtualframe6.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/demo/virtualframe3.ps,width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/demo/virtualframe4.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/demo/virtualframe5.ps, width=1.0in} \\
}

\caption{(a) Top row: images captured from the left camera. (b)
Second row: images captured using the right camera. (c) Third row:
images captured using camcorder that is placed in front of the
face. (d) Final row: virtual frontal views generated from the
images in the first two rows} \label{fig:demo}
\end{figure}

\subsection {Video Synchronization}
Synchronization in the two videos is crucial in our application.
Since, two views of a face with lip movements are merged together,
any small changes in the synchronization will have high impact on
the misalignment of the lips. This synchronization can be
evaluated based on sensitive movements such as eyeball movements
(see Figure ~\ref {fig:eyeball}) and blinking eyelids (see Figure
~\ref{fig:eyeblink}). Similarly, mouth movements can be analyzed
from the virtual videos.

%\begin{figure}[htp]
%%\centerline{\epsfig{figure=Figures\figure.ps, width=2.5in} }
%\caption{Synchronization of the eyeball movements.}
%\label{fig:eyeballs}
%\end{figure}
%
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/eyeball/realframe1.ps, width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeball/realframe2.ps,
 width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeball/realframe3.ps,width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeball/realframe4.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeball/realframe5.ps, width=1.0in} \\
   } \vspace{0.2in} \centerline{
     \epsfig{figure=Figures/eyeball/virtualframe1.ps, width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeball/virtualframe2.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeball/virtualframe3.ps,width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeball/virtualframe4.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeball/virtualframe5.ps, width=1.0in} \\
}\caption{Synchronization of the eyeball movements: real video is
in the top row and the virtual video is in the bottom row.}
\label{fig:eyeball}
\end{figure}


\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/eyeblink/realframe1.ps, width=1.0in, height=1.1in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeblink/realframe2.ps, width=1.0in,height=1.1in}
\hspace{0.1in}\epsfig{figure=Figures/eyeblink/realframe3.ps,width=1.0in,height=1.1in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeblink/realframe4.ps, width=1.0in,height=1.1in}
\hspace{0.1in}\epsfig{figure=Figures/eyeblink/realframe5.ps, width=1.0in,height=1.1in} \\
   } \vspace{0.2in} \centerline{
     \epsfig{figure=Figures/eyeblink/virtualframe1.ps, width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeblink/virtualframe2.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeblink/virtualframe3.ps,width=1.0in}
 \hspace{0.1in} \epsfig{figure=Figures/eyeblink/virtualframe4.ps, width=1.0in}
\hspace{0.1in}\epsfig{figure=Figures/eyeblink/virtualframe5.ps, width=1.0in} \\
} \caption{Synchronization of the eyelids during blinking: real
video is in the top row and the virtual video is in the bottom
row.} \label{fig:eyeblink}
\end{figure}

\section {3D Face Model Construction}
\label {sec:res3d} A 3D individualized head model can be
constructed by adjusting a generic mesh model to fit the 3D
feature points of an individual face. Depth information at the eye
corners, mouth corners and nose tip is estimated using the stereo
method. Section ~\ref{sec:stereo} deals with the results of the
stereovision computations.

\subsection {Stereovision Computations}
\label {sec:stereo} Table ~\ref {TB:time} shows the error obtained
during the estimation of 3D world coordinates on the calibration
sphere. On average, the error in coordinates was less than 0.1
inches. The maximum total error was not more than 0.2 inches. For
estimating the depth information of the facial feature points this
accuracy might be sufficient.

\begin{table}[htp]
  \centering   \caption{\protect\small Depth estimation from left camera and projector for points on the calibration sphere. 3D coordinate dimensions are in inches.}
   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
\multicolumn{8}{|c|}{INPUT DATA} & \multicolumn{4}{c|}{OUTPUT
DATA} \\\hline

Point &\multicolumn{3}{c|}{3D Coordinates}&
\multicolumn{2}{c|}{Left Camera}& \multicolumn{2}{c|}{Projector} &
\multicolumn{3}{c|}{Computed points} & \multicolumn{1}{c|}{Error}
\\ \cline{2-11}

&x &y&z& u & v & x & y &   $x^1$ & $y^1$ &  $z^1$ & \\
\hline

A &  0.00 &  0.00 &  4.65  &  198 &116& 511& 432& 0.00 &0.02 &
4.69&
0.06  \\
\hline

B &  0.00  & 2.33 &  4.03  & 190& 36 & 512 &348 &-0.02  &2.30 &4.12& 0.14  \\
\hline

 C  & -1.64 & 1.64  & 4.03  & 135 &56  &449 &373& -1.65 &
 1.64&
4.07& 0.05  \\\hline

 D  & -2.33 & 0.00& 4.03&   109 &115& 420& 435& -2.38&  -0.01&
4.09 &0.12  \\\hline

E &  -1.64&  -1.64& 4.03 &  135& 176& 448& 496& -1.62& -1.62&
4.14& 0.15  \\\hline

F &  0.00 &-2.33  &4.03 &  187 &202 &509 &524 &-0.02& -2.34 &4.04&
0.04
\\\hline

G &1.64 &  -1.64 & 4.03 & 240 &177& 573& 498 &1.65 &-1.64& 4.04&
0.02  \\\hline

 H &  2.33 &  0.00 &4.03 &  262 &121& 600 &437 &2.32 &  -0.03&
 4.11&
0.12  \\\hline

I  & 1.64& 1.64 &4.03& 241& 62&  573 &374& 1.59& 1.64 &4.17 &0.19
\\\hline

K& -2.85 &2.85 &2.32&   74 & 16 & 409 &336 &-2.83& 2.86& 2.30&
0.05
\\\hline

L &-4.03& 0.00 &2.33 &  30 & 116& 363 &441 &-4.03& 0.00& 2.31
&0.02
\\\hline

M& -2.85& -2.85& 2.33 &  69 & 220 &405 &547& -2.84& -2.86& 2.26
&0.09

 \\\hline

\end{tabular}
\label{TB:time}
\end{table}

%
%\begin{table}[tb]
%  \centering   \caption{\protect\small Depth Estimation from Right Camera and Projector}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
%\multicolumn{8}{|c|}{INPUT DATA} & \multicolumn{4}{c|}{OUTPUT
%DATA} \\\hline
%
%Point &\multicolumn{3}{c|}{3D Coordinates}&
%\multicolumn{2}{c|}{Right Camera}& \multicolumn{2}{c|}{Projector}
%& \multicolumn{4}{c|}{Residuals}
%\\ \cline{2-12}
%
%&x &y&z& s & t & x & y &   $x^1$ & $y^1$ &  $z^1$ & $Total_{error}$ \\
%\hline
%
%A &  0.000 &  0.000& 4.650 & 97 & 110& 511& 432& 0.002 &  0.031&
%4.675&
%-0.058 \\
%\hline
%
%B &  0.000 &  2.325 &  4.027 &  111 &29 & 512& 348 &-0.020&  2.339 &3.949 &0.084\\
%\hline
%
% C&   -1.644 & 1.644 &  4.027 &  58 & 54 & 449 &373& -1.658&
% 1.644&
%3.970& 0.071 \\\hline
%
%D  & -2.325 & 0.000 & 4.027 &  33 & 111& 420 &435 &-2.388 & -0.006 &3.977& 0.119 \\
%\hline
%
%E& -1.644&  -1.644& 4.027 &53 & 167& 448 &496 &-1.625& -1.602& 4.043& -0.077\\
%\hline
%
% F& 0.000 &-2.325 & 4.027 &104 &196& 509& 524& -0.015& -2.335 &3.996 &0.056\\
%\hline
%
%G &1.644 &  -1.644 &4.027 &  160& 173& 573& 498 &1.648 &-1.630 &3.996& 0.013 \\
%\hline
%
% H& 2.325&   0.000& 4.027 &  185& 115& 600& 437& 2.327 &  -0.020&
% 4.010&
%0.036 \\
%\hline
%
%I& 1.644 &  1.644 &4.027 &  163& 54& 573 &374& 1.592 &  1.649& 3.952& 0.122 \\
%\hline
%
%O& 2.848& -2.848 & 2.325 &  222& 219& 616 &548 &2.864 &-2.867& 2.359& -0.031 \\
%\hline
%
% P& 4.027 &  0.000 &  2.325 &  265 &118 &660& 441& 4.010& 0.030
% &2.310&
%0.002 \\
%\hline
%
%Q& 2.848& 2.848& 2.325 &  229 &17 &618& 339 &2.827 &  2.853&
%2.215& 0.125
%\\
%\hline
%
%\end{tabular}
%
%\label{TB:time}
%\end{table}
%



%
%
%\begin{table}[tb]
%  \centering   \caption{\protect\small Depth Estimation from Left Camera and Right Camera}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} \hline
%\multicolumn{8}{|c|}{INPUT DATA} & \multicolumn{4}{c|}{OUTPUT
%DATA} \\\hline
%
%Point &\multicolumn{3}{c|}{3D Coordinates}&
%\multicolumn{2}{c|}{Left Camera}& \multicolumn{2}{c|}{Right
%Camera} & \multicolumn{4}{c|}{Residuals}
%\\ \cline{2-12}
%
%&x &y&z& u & v & s & t &   $x^1$ & $y^1$ &  $z^1$ &
%$Total_{error}$ \\\hline
%
%A &  0.000 &   0.000 &   4.650&    198 &116 &97 & 110& 0.004
%&0.015& 4.675& -0.044
%\\\hline
%
%B &  0.000&   2.325 &  4.027 &  190 &36 & 111& 29 & 0.020& 2.320&
%4.031& -0.019
%\\\hline
%
%C &  -1.644 & 1.644 &  4.027 &  135 &56 & 58& 54 & -1.632 & 1.632&
%4.015& 0.012 \\\hline
%
%D &  -2.325 & 0.000& 4.027& 109& 115 &33 & 111& -2.360&  -0.016&
%4.023& 0.055
%\\\hline
%
%E &-1.644 & -1.644 & 4.027 &135 &176 &53 & 167& -1.603 & -1.621&
%4.083& -0.120 \\\hline
%
%F &  0.000 &   -2.325&  4.027 &187& 202& 104& 196 &-0.007& -2.346&
%4.009& 0.046
%\\\hline
%
%G& 1.644& -1.644&  4.027 &  240& 177& 160& 173& 1.657& -1.641&
%4.016 &-0.004\\\hline
%
% H &2.325 &  0.000 & 4.027& 262 &121 &185& 115& 2.349& -0.029&
%4.060& -0.028 \\\hline
%
%I& 1.644 &1.644 &  4.027 &  241& 62 & 163 &54 &1.641 &1.644&
%4.066& -0.036\\\hline
%
%\end{tabular}
%
%\label{TB:time}
%\end{table}
%
%
\subsection {Customization of the 3D Face Model}
\label {sec:res3d} The generic model used to generate the
customized texture mapped face model was described in Figure ~\ref
{fig:meshmodel}. This model is made up of 395 vertices and a total
of 2454 edges forming 818 triangles. Each triangle is defined by
three vertices. This model is a complete head model that contains
the ears and the back head portion. It also includes the eye
balls, which are not common in some other face models. The
customization of the generic head model is done by distorting the
generic model as described in \cite {Ip96}. As discussed earlier,
the 3D information of some of the prominent facial feature points
are estimated and the 3D model is distorted to obtain the
customized head model. The frontal view texture used for texture
mapping the 3D model is shown in Figure ~\ref {fig:front_texture}.
This texture map was obtained by extending the grid lines during
the calibration stage. Figure ~\ref {fig:3dmodel} shows different
rendered views of the 3D face model that was constructed from the
two side views.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/output.ps, width=3.5in}
}
 \caption{Frontal texture used for 3D face model construction}
\label{fig:front_texture}
\end{figure}
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/3dmodels.ps, width=5.0in}
}
\caption{Different views rendered from the texture mapped 3D
face model} \label{fig:3dmodel}
\end{figure}


==> orig/saddlepoint.tex <==
\section {Saddle Point Detection} \label{sec:saddlepoint}


==> orig/saddlepointdetection.tex <==
\chapter {Finding Saddle Points using Stability Boundary based Method}
\label{ch:saddlepointdetection}


The task of finding saddle points on potential energy surfaces play
a crucial role in understanding the dynamics of a micro-molecule as
well as in studying the folding pathways of macro-molecules like
proteins. The problem of finding the saddle points on a high
dimensional potential energy surface is transformed into the problem
of finding decomposition points of its corresponding nonlinear
dynamical system. This chapter introduces a new method to compute
saddle points on potential energy surfaces using stability
boundaries. Our method explores the dynamic and geometric
characteristics of stability boundaries of a nonlinear dynamical
system. A novel trajectory adjustment procedure is used to trace the
stability boundary. Our method was successful in finding the saddle
points on different potential energy surfaces of various dimensions.
A simplified version of the algorithm has also been used to find the
saddle points of symmetric systems with the help of some analytical
knowledge. The main advantages and effectiveness of the method are
clearly illustrated with some examples. Promising results of our
method are shown on various problems with varied degrees of freedom.

\section{Introduction and Background}

Recently, there had been a lot of interest across various
disciplines to understand a wide variety of problems related to
bioinformatics. One of the most challenging problems in the field
of bioinformatics is de-novo protein structure prediction where
the structure of protein is estimated from some complex energy
functions. Scientists have related the native structure of a
protein structurally to the global minimum of the potential energy
surface of its energy function. If the global minimum could be
found reliably from the primary amino acid sequence, it would
provide us with new insights into the nature of protein folding.
However, understanding the process of protein folding involves
more than just predicting the folded structures of foldable
sequences. The folding pathways in which the proteins attain their
native structure can deliver some important information about the
properties of the protein structure.

Proteins usually have multiple stable macrostates. The
conformations associated with one macrostate correspond to a
certain biological function. Understanding the transition between
these macrostates is important to comprehend the interplay between
that protein and its environment. Hence, to understand the
kinetics of the folding process we need the structure of the
transition state. Since, it is difficult to characterize these
structures by experiments, simulations are ideal tools for
characterization of the transition structures. Recently,
biophysicists started exploring the computational methods that can
be used to analyze conformational changes and identify possible
reaction pathways. In particular, the analysis of complex
transitions in macromolecules has been thoroughly studied.


\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/figure1a.ps, width=3.5in}
} \caption{The surface and contour plots of a two-dimensional
energy function.A saddle point ($x_d$) is located between two
local minima ($x_s^1$ and $x_s^2$). $x_m^1$ and $x_m^2$ are two
local minima located in the orthogonal direction.}
\label{fig:saddlepoint}
\end{figure}


Transition state conformations are saddle points. {\it Saddle
points} are the points on the potential energy surface where the
gradient is zero and the Hessian matrix of the second derivatives
of the potential energy has only one negative eigenvalue \cite
{Heidrich91}. Intuitively, this means that a saddle point is a
maximum along one direction but a minimum along all other
orthogonal directions. Fig. 1 shows a saddle point ($x_d$) located
between two local minima ($x_s^1$ and $x_s^2$) and two local
maxima ($x_m^1$ and $x_m^2$). As shown in the figure, the saddle
point is a maximum along the direction of the vector joining the
two local minima and a minimum along its orthogonal direction (or
the direction of the vector joining the two local maxima). The
direction in which the saddle point is the maximum is usually
unknown in most of the practical problems and is the direction of
interest. This makes the problem of finding the saddle points more
challenging than the problem of finding local minima on a
potential energy surface. In terms of transition states, saddle
points are local maxima with respect to the reaction coordinates
for folding and local minima with respect to all other
coordinates. The search for the optimal transition state becomes a
search for the saddle points at the edge of the potential energy
basin corresponding to the initial state. Hence, finding the
saddle points on the potential energy surfaces is a challenging
problem and will give new insight into the folding mechanism of
proteins.
%
%The primary focus of this chapter is to find the saddle points on
%different potential energy surfaces with varied degrees of freedom.
%The saddle point to be found is between two known neighborhood local
%minima. Section~\ref{sec:background} briefly describes some related
%methods that were developed for finding saddle points.
%Section~\ref{sec:overview} gives the necessary theoretical
%background of our approach and describes the problem formulation.
%Section~\ref{sec:algorithm} explains the various steps involved in
%our approach. The implementation details along with the pseudocode
%of different procedures are provided in Section
%\ref{sec:implementation}. Results of our method on different systems
%are clearly illustrated in Section \ref{sec:results} with some
%relevant discussion.

\section*{Relevant Background}
\label{sec:background}

In the field of computational chemistry, finding saddle points had
been a topic of active research for almost two decades. Recently,
there has also been some interest in finding the saddle points of
the lennard jones clusters since it will give some idea about the
dynamics of the system \cite {Doye02}. The properties of
higher-index saddle points have been invoked in recent theories of
the dynamics of supercooled liquids. Since the saddle points are
related to the eigenvalues of the Hessian matrix, several methods
have been proposed in the literature that are based on the idea of
diagonalization of the Hessian matrix \cite {Helgaker91}. Some
improved methods dealing with the updates of Hessian matrix have
also been proposed \cite {Quapp98}. Even though these methods appear
to find saddle points accurately, they work mainly for low
dimensional systems. These methods are not practical for more higher
dimensional problems because the computational cost increases
tremendously as the the number of dimensions increase.\\

However, some methods have been developed that work without the
necessity for computing the second derivatives. Because of the
scalability issues, much more importance is given to the algorithms
that use only the first derivatives to compute the saddle points. A
detailed description of the methods that work only based on first
derivatives along with their advantages and disadvantages is given
in a recent review paper \cite{Henkelman00b}. The various methods
that are used to find saddle points are drag method, dimer method,
self penalty walk, activation relaxation technique, ridge method ,
conjugate peak refinement, DHS method, Nudged elastic band, Step and
slide. Almost all these methods except the dimer method are used to
identify the saddle point between two given neighboring local
minima. Though the dimer method successfully finds the saddle points
in those cases where only one minimum is given, it does not
have a good control over which saddle point it tries to find.\\

Most of the methods above are some variations of the existing
approaches. Also, these methods start searching for the saddle
points from the local minimum itself and hence needs to compute the
first derivative. However, our approach doesn't need the gradient
information at all from the local minima. It will find the stability
boundary in some direction and then traces the stability boundary
till it reaches the saddle point. This tracing of the stability
boundary is much more efficient than looking for saddle points in
the entire search space. This chapter introduces a completely novel
{\it stability boundary} based approach to compute the saddle points
between two given local minima. Our method crops from some of the
fundamental results on stability regions of nonlinear dynamical
systems \cite{Chiang88,Chiang96a}.

\section{System Overview}
\label {sec:overview}

This section introduces some of the terminology needed to
understand our approach. Most importantly, this section deals with
the transformation of the potential energy function into a
nonlinear dynamical system. It also gives the correspondence
between all the critical points of a $n$-dimensional potential
energy surface and its nonlinear dynamical system.



\subsection*{Problem Formulation and Transformations}
\label{sec:problem}


%\cite{Chiang96,Lee04} describes some of the theoretical concepts
%required to understand our methodology. In this paper, we
%transform the problem of finding the saddle points on high
%dimensional potential energy surfaces into the problem of
%computing the decomposition points of the corresponding nonlinear
%dynamical system. The decomposition point exists between two
%nearby stable equilibrium points and can be computed using our
%{\it stability boundary based method}.
%

%
%\begin{thm}\label{th:epos}{\it (Equilibrium points and optimal
%solutions):}
%     Suppose that the optimization problem (1) satisfies Assumptions 1. If     is a non-degenerate critical point of the optimization problem (1), then    is a hyperbolic equilibrium point of (3). Moreover,
%     is a stable equilibrium point of (3) if and only if  is an isolated local minimum of (1).
%     is a source of (3) if and only if      is an isolated local maximum of (1).
%
%\end{thm}
%
%Theorem ~\ref{th:epos} shows the transformation between the
%equilibrium points and the optimal solutions. Theorem
%~\ref{th:dpse} gives the one-to-one correspondence between the
%search problem and the dynamical system constructed.
%
%\begin{thm}\label{th:dpse}{\it (Decomposition Points and Stable Equilibrium
%Points):}
%
%    Suppose that the optimization problem (1) satisfies Assumptions 1-2. Let a stable equilibrium point    of (3) be given. If xd is a decomposition point on ?Ap(   ), then there exists another stable equilibrium point    to which the 1-D unstable manifold of xd converges. Conversely, if
%                                       , then there exists a decomposition point xd on ?Ap(   )
%
%\end{thm}




We used a new {\it trajectory adjustment procedure} to move along
the practical stability boundary. Once the exit point is
identified, the consecutive points on the stability boundary can
be identified by the ray-adjustment procedure. During this
traversal, the value of the gradient along the boundary is noted
and the process of moving along the boundary is terminated when
the Minimum vector-field point(MVP) is obtained. The MVP is
guaranteed to be in the local neighborhood of the decomposition
point and any robust nonlinear system solver can be applied to
reach the decomposition point.

\section{A Stability Boundary based Method}
\label{sec:algorithm} The method described in this section finds
the decomposition point when the two neighborhood minima are
given. Our method is illustrated on a two-dimensional LEPS
potential energy surface. The equations corresponding to the LEPS
potential are given in appendix. The two local minima are $A$ and
$B$ and the decomposition point is $D$.\\

%\begin{figure}[htp]
%\begin{center}
%\epsfig{figure=Figures/myleps1.ps, width=3.5in}
%% \hspace{0.3in} \epsfig{figure=Figures/energy.ps, width=1.3in}
%\caption {Contour plot of a 2-D LEPS potential (described in
%appendix). Each line represents the values of a constant
%potential. $A$ and $B$ are the two local minima. $D$ is the
%decomposition point to be computed.}
% \end{center}
%\label{fig:leps}
%\end{figure}

%\begin {enumerate}
%\itemsep +.1in

Step1: {\it Initializing the Search direction} : Choose the
direction vector that joins the two given local minima ($A$ and
$B$). If only one local minimum is available then search direction
will be made based on eigen vectors of the Hessian matrix computed
at that local minimum. However, in our case, the location of the
neighborhood local minima is given, hence the initialization of the search direction becomes more explicit. \\

Step 2: {\it Locating the exit point ($X_{ex}$)} : (see fig.
\ref{fig:myleps2}a) Along the direction $AB$, starting from $A$, the
function value is evaluated at different step intervals. Since the
vector is between two neighborhood local minima, the value of the
energy function will monotonically increase and decrease till it
reaches the other local minimum ($B$). The
point where the energy value attains its peak is called the {\it exit point}.\\
\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/myleps2.ps, width=2.5in}
\hspace{0.5in} \epsfig{figure=Figures/myleps3.ps, width=2.5in}
}\caption {(a) Illustration of steps 1 and 2 of our method. The
search direction is the direction of the vector AB. The exit point
($X_{ex}$) is obtained by finding the peak of the energy function
along this vector. (b) Illustration of the step 3 of our algorithm.
$m_1$ is integrated till $m'_1$ is reached and traced back along the
vector $m'_1B$ to get $m_2$, and so on... $m_n$ are the n points on
the stability boundary. The $n^{th}$ point is the Minimum
Vector-field Point where the magnitude of the gradient ($G_M$) is
the minimum. D is the decomposition point.} \label{fig:myleps2}
\end{figure}

Step 3: {\it Moving along the stability boundary to locate the
Minimum Vector-field Point} : The exit point ($X_{ex}$) is
integrated for a predefined number of times. Let $m'_1$ be the new
point obtained after integration. The value of the energy function
between $m'_1$ and one of the local minima (say $B$) is evaluated
If the value is immediately decreasing then it means that there is
no peak in that search direction and hence the stability boundary
will not be encountered in this direction. In this case, the
search direction has to be modified. The simplest way to find the
peak is to search in the exact opposite direction. Let the new
boundary point that is obtained along the vector $m'_1B$ starting
from the point $m'_1$ and where the value attains the peak is
$m_2$. This process is repeated and the value of the gradient is
noted at each of the boundary points. This process of moving along
the boundary is terminated when the minimum vector-field point is
reached. In summary, the trajectory of integration is being
modified so that it move towards the MVP and will not converge to
one of the local minima. Hence, this step is named as the
trajectory-adjustment procedure.

Step 4: { \it Locating the Decomposition point} : The Minimum
Vector-field Point ($m_n$) obtained from the previous step will be
present in the neighborhood of the decomposition point. A local
minimizer to solve the system of nonlinear equations is applied
with $m_n$ as initial guess and this will yield the decomposition
point.  A detailed survey about different Local minimizations
applied to various energy
functions is given in \cite{Schlick02}. \\

%\end {enumerate}
%%\subsection {Theoretical Background}
%
%%The following theorems will try to convince he reader that the
%%algorithm described above should find the saddle points.
%%
%%\newtheorem{thm}{Theorem}
%%%[section]
%%%\newtheorem{cor}[thm]{Corollary}
%%%\newtheorem{lem}[thm]{Lemma}
%%
%%\begin{thm}\label{th:mono} Between two consecutive minima the value of the energy function will monotonically increase till
%%the exit point and reduce monotonically gradually till it reaches
%%the other minima
%%\end{thm}
%%
%%\begin{proof}
%%
%%\end{proof}
%%
%%
%%%
%%%End of proof symbol. The \end{proof} command generates a "qed
%%%symbol" (by default, a hollow square) at the end of the proof. The
%%%symbol can be redefined with \qedsymbol; in particular, if you
%%%don't want qed symbols, just redefine \qedsymbol to an empty
%%%command as follows: \renewcommand{\qedsymbol}{}. If this
%%%definition is placed in the preamble, its effect is global.
%%%However, one can also place the definition inside a \begin{proof}
%%%... \end{proof} pair. In this case, it only affects the current
%%%proof and eliminates the qed symbol in that proof, but has no
%%%effect on other proofs. (There are situations where one might want
%%%to do that.)
%%

%%\begin{thm}\label{th:exitpoint} Integrating the analytical exit point
%%will eventually move towards the saddle point
%%\end{thm}
%%
%
%%
%%Before we proceed further with the discussion about the algorithm,
%%we need to define some terms and initialize certain threshold
%%values that we will be using in further sections. Let $r_{ij}$ be
%%the Euclidean distance between the two conformations $i$ and $j$.
%%Let $r_{t}$ be the threshold distance. Basically, these two
%%variables will make sure that the two conformations $i$ and $j$
%%will not give any repetitive information. In this way, a pool of m
%%solutions are generated randomly. Each solution consists of a
%%string of 3N coordinates \footnote {Even though the problem is
%%originally of 3N dimensions (where N is the cluster size), the
%%optimization for the global minimum structure is done in (3N-6)
%%dimensional space. However, it is not a consideration for our
%%discussion here because we are only trying to estimate the minimum
%%energy. The remaining 6 degrees of freedom are due to the
%%rotational and translational variants of the original structure}.
%%This pool of solutions is called the {\it Bank}. Based on the
%%values of $r_{ij} $ between the two conformations, the new
%%conformations are either accepted or rejected. This is the {\it
%%selection step} of the GA which necessarily says that only the fit
%%species will survive. If $r_{ij}>r_t$, then $i$ constitutes a new
%%group. The lowest-energy representatives from each group within
%%the bank, including the new $i$ group, are then compared and the
%%worst conformation (i.e. the highest-energy conformation) is
%%discarded. Therefore, the size of the bank always remains
%%constant.

%%Here are the main parameters to keep in mind.
%%    \begin{itemize}
%%     \item {Computational complexity}
%%     \item {Scalability}
%%     \item {reproducibility}
%%     \item {Reliable}
%%    \end{itemize}
%%

%\section{Implementation Details}
%\label{sec:implementation}
%
%
%For our illustration, lets consider a N dimensional energy
%function $F$ with variables $X_i$, where $i=1...N$. From the
%algorithmic viewpoint, our method consists of three stages.
%The psuedocode for finding the decomposition point. Let $A$ and $B$ are the local minima.\\
%
%$point${\bf
%\hspace{0.1in}procedure\hspace{0.1in}}$locate\_DP(A,B)$
%\begin{algorithmic}
%\STATE Initialize $stepsize=10~$  // initial evaluation step size
%\STATE $EP~\leftarrow ~ find\_boundary(A,B, stepsize)~$ // Exit
%point \STATE $MVP~\leftarrow ~ compute\_MVP(EP)~$ // Trace the
%boundary\STATE $DP~\leftarrow ~ local\_minimizer(MVP)$ \STATE \bf
%return $DP$
%\end{algorithmic}
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/myleps2aa.ps, width=2.5in} } \caption{The plot of the energy function value along
%the vector $AB$. The curve monotonically increases starting from
%$A$ and then decreases till it reaches $B$. $X_{ex}$ is the exit
%point where the function attains its peak value. $a_1$, $a_2$, ...
%$a_9$ are the interval points. The marked circles indicate that
%the function has been evaluated at these points. The empty circles
%indicate the points where the function is yet to be evaluated.}
%\label{fig:energycurve}
%\end{figure}
%
%$point${\bf
%\hspace{0.05in}procedure\hspace{0.05in}}$find\_boundaryPt(A,B,steps
%)$
%\begin{algorithmic}[1]
%\STATE Initialize $eps$  // accuracy \STATE
%$interval~=~(B-A)/steps$ \STATE $cur~=~eval(A)$ \STATE
%$tmp~=~A~+~interval$
%    \IF{$eval(tmp)~<~cur$}
%    \STATE $B~=~2*A~-~B$
%    \ENDIF
%\FOR{$i=1~to~steps$} \STATE  $tmp~=~A~+~i*interval$ \STATE
%$prev~=~cur$ \STATE $cur~=~eval(tmp)$
%    \IF{$prev~>~cur$}
%    \STATE $newPt~=~A~+~(i-2)*interval$
%    \STATE $BdPt~=~GoldenSectionSearch(tmp,newPt,eps)$
%    \STATE \bf return $BdPt$
%    \ENDIF
%\ENDFOR \STATE \bf return $NULL$
%\end{algorithmic}
%
%The procedure $find\_boundaryPt$ will find the point on the
%stability boundary between two given points $A$ and $B$ starting
%from $A$. If the function value is monotonically decreasing from
%the first step, then it indicates that there will not be any
%boundary in that direction, and the search is changed to a new
%direction. The new direction can be obtained by making $B=2A-B$.
%Finding the exit point can be done more efficiently by first
%evaluating the function at comparatively large step intervals. The
%function evaluation is started from $a_1$ , $a_2$ and so on. Once
%$a_6$ is reached the energy value start to reduce indicating that
%the peak value was reached. Golden section search algorithm (see
%appendix) is used to efficiently find the exit point within a
%small interval range where the peak value is present. The golden
%section search is applied to obtain the exit point $X_{ex}$ within
%the intervals $a_4$ and $a_6$.
%
%Fig. \ref{fig:energycurve} shows the other two possibilities of
%having the interval points. It should be noted that the golden
%section search procedure should not be invoked with two
%consecutive intervals between which the value starts to reduce. It
%should be applied to two intervals $a_4$ and $a_6$. The two
%possibilities are that $a_5$ can be present either to the left of
%the peak or to the right of the peak. From Fig.
%\ref{fig:energycurve}b, we can see that the value at $a_5$ is
%greater than $a_4$ and less than $a_6$ but still the peak is not
%present between $a_5$ and $a_6$. This is the reason why the golden
%section search method should have $a_4$ and $a_6$ as its
%arguments.
%
%\begin{figure}
% \epsfig{figure=Figures/peak2.ps, width=3.5in}\\
% \hspace{1.0in} (a) \hspace{1.8in} (b)\\
%\caption {The interval point $a_5$ can be present either to the
%left or to the right of the peak. When $a_6$ is reached, the
%golden section search method is invoked with $a_6$ and $a_4$ as
%the interval.} \label{fig:energycurve}
%\end{figure}
%
%In an ideal case, integration from the exit point will lead to the
%decomposition point. However, due to the numerical approximations
%made, the integration at the exit point will eventually converge
%to its corresponding local minima. Hence, we need to adjust the
%path of integration so that it can effectively trace the boundary.
%
%$point${\bf \hspace{0.1in}procedure\hspace{0.1in}}$compute\_MVPt(
%ExPt)$
%
%\begin{algorithmic}[1]
%\STATE Initialize $dt$  // Integral step size
%
%\STATE Initialize $intsteps$  // No. of integration steps
%
%\STATE Initialize $smallstep$  //small step size
%
%\STATE $reduce\_flag~=~OFF$  // To check if gradient reduced
%
%\STATE $BdPt~=~ExPt$
%
%\STATE $GM\_next~=~GM(BdPt)$
%
%\WHILE{(1)}
%
%\STATE $NewPt~=~integrate(BdPt,intsteps,dt)$ \STATE
%$prevPt~=~BdPt$
%
%\STATE $BdPt~=~find\_boundaryPt(NewPt,~A,~smallstep)$
%
%\STATE $GM\_prev~=~GM\_next$
%
%\STATE $GM\_next~=~GM(BdPt)$
%
%    \IF{$GM\_next~<~GM\_prev$}
%    \STATE $reduce\_flag~=~ON$
%    \ENDIF
%
%\IF{$GM\_next>GM\_prev$ \& $reduce\_flag=ON$}
%    \STATE $MVPt=prevPt$
%    \ENDIF
%
%\STATE \bf return $MVPt$
%
%\ENDWHILE
%
%\end{algorithmic}
%
%The procedure $compute\_MVPt$ takes in the exit point as the
%argument and returns the computed MVP obtained by tracing the
%stability boundary starting from the exit point. The point on the
%stability boundary is integrated for a predefined number of times
%(say 5). From the exit point, it is integrated using the equation
%shown below.
%
%\begin{equation}
%X_i = X_i - \left(\frac{\partial F}{\partial X_i}\right)~.~ \Delta
%t ~ ~~~~~~~~~\forall i=1,...,N
% \label{th:integrate}
%\end{equation}
%
%The procedure $integrate$ computes a point ($newPt$) by
%integrating a certain number of integral steps ($intstep$) with a
%predefined integration step size ($\Delta t$) from  the boundary
%point ($bdPt$). Once again a new boundary point is obtained from
%$newPt$ and local minima in the other stability region using the
%procedure $find\_boundaryPt$ and this process is repeated. Another
%important issue to be dealt is that when should we stop this
%process. For this, we need to compute the magnitude of the
%gradient at all points obtained on the stability boundary. The
%magnitude of the gradient ($G_M$) is calculated using Eq.
%(\ref{th:GM}).
%\begin{equation}
%G_M =  \sqrt {\sum_{i=1}^{N}\left(\frac{\partial F}{\partial
%X_i}\right)^2 } \label{th:GM}
%\end{equation}
%
%where $\Delta t$ is the integral step size. The $G_M$ value can
%either start increasing and then reduce or it might start reducing
%from the exit point. The $reduce\_flag$ indicates that the $G_M$
%value started to reduce before. $GM\_next$ and $GM\_prev$ are the
%two variables used to store the values of the current and previous
%$G_M$ values respectively. The $MVP$ is obtained when $GM\_next
%> GM\_prev$ and $reduce\_flag=ON$.
%
%
%%The exit point ($X_{ex}$) is integrated for a predefined number of
%%times (say 5). Let $m'_1$ be the new point obtained after
%%integration. The value of the energy function between $m'_1$ and
%%one of the local minima (say $B$) is evaluated If the value is
%%immediately decreasing then move in the opposite direction. This
%%indicates that the next point on the boundary will be reached in
%%the opposite direction. Let the new boundary point that is
%%obtained along the vector $m'_1B$ starting from the point $m'_1$
%%and where the value attains the peak is $m_2$. This process is
%%repeated and the value of the gradient is noted at each of the
%%boundary points. This process of moving along the boundary is
%%terminated when the minimum vector-field point is reached. Let the
%%point $m_n$ be the point on the boundary corresponding to the minimum vector-field point. \\
%
%%A subspace trust region method based on the interior-reflective
%%Newton algorithm described in \cite{Coleman96} has been used for
%%local minimization. A detailed description of different local
%%search methods along with their implementation is given in \cite
%%{press92}.

\section{Results and Discussion}
\label{sec:results}

\subsection*{Test Case 1: Two-dimensional Potential Energy Surfaces}
\subsubsection{Muller-Brown surface}

The Muller-Brown surface forms a standard two-dimensional example of
a potential energy function in theoretical chemistry \cite
{Muller79}. This surface was designed for testing the algorithms
that find saddle points. Eq. (\ref {eq:mullerbrown}) gives the
Muller-Brown energy function. Fig. \ref{fig:mullerbrownresult}a
represents the two-dimensional contour plot of the potential energy
surface of the muller-brown function.
\begin{equation} \label{eq:mullerbrown}
%\begin{split}
C(x,y) = \sum_{i=1}^4 A_i~ exp\Bigl[a_i(x-x_i^o)^2+b_i(x-x_i^o)(y-y_i^o) + c_i(y-y_i^o)^2\Bigr].\\
%\end{split}
\end{equation}
where \\
\begin{table}[h]
\begin{center}
\begin{tabular}{l l}
 A  = (-200.0, -100.0, -170.0, -15.0) &   a = ( -1.0, -1.0, -6.5, -0.7) \\
 $x^o$ = (1.0, 0.0, -0.5, -1.0)& b = (0.0, 0.0, 11.0, 0.6)\\
$y^o$ = ( 0.0, 0.5, 1.5, 1.0)   & c = (-10.0, -10.0, -6.5, 0.7)
\end{tabular}
\end{center}
\label{TB:values}
\end{table}
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/mullerbrown.ps, width=3.5in}
%} \caption{Two dimensional contour plot of the potential energy
%surface corresponding to the muller-brown function described on
%Eq. (\ref{eq:mullerbrown}). A,B,C - three local minima and 1,2 -
%two decomposition points.} \label{fig:mullerbrown}
%\end{figure}

As shown in Fig. \ref {fig:mullerbrownresult}a, there are three
local minima (A,B,C) and two decomposition points (1,2) on the
muller-brown potential energy surface. Decomposition point 1 is
present between two local minima A and B and is more challenging to
find, compared to decomposition point 2 which is present between
local minima B and C. Table~\ref {TB:mullerbrownresults} shows the
exact locations and energy values of the local minima and the
decomposition points.

\begin{table}[htp]
\centering \caption{\protect\small Local Minima and Decomposition
Points for the Muller-Brown Surface described in Eq. (\ref
{eq:mullerbrown}).     (LM - Local Minimum, DP - Decomposition
Point)}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Equilibrium Points &  Location & Energy value c(.) \\
\hline LM A & (-0.558,1.442) & -146.7 \\
\hline DP 1 & (-0.822,0.624) & -40.67 \\
\hline LM B & (-0.05,0.467) & -80.77 \\
\hline DP 2 & (0.212,0.293) & -72.25 \\
\hline LM C & (0.623,0.028) & -108.7 \\ \hline
\end{tabular}
\end{center}
\label{TB:mullerbrownresults}
\end{table}

The dynamical system corresponding to (\ref{eq:mullerbrown}) is
given by
\begin{center}
\begin{equation}
\nabla C(x) = ~-~\left[ \begin{array}{c} \frac{\partial
C}{\partial x} \vspace{0.05in}\\
\frac{\partial C}{\partial y} \\
\end{array} \right]
\end{equation}

\begin{eqnarray*}
\frac{\partial C}{\partial x} = \sum_{i=1}^4
A_i~.~P~.~[~2a_i(x-x_i^o)+
 b_i(y-y_i^o)~]\\
\frac{\partial C}{\partial y}= \sum_{i=1}^4
A_i~.~P~.~[~b_i(x-x_i^o)+2c_i(y-y_i^o)~] \label{eq:dcdxy}
\end{eqnarray*}
\end{center}
where \\
\begin{equation*}
P=exp~[~a_i(x-x_i^o)^2+ b_i(x-x_i^o)(y-y_i^o) +
c_i(y-y_i^o)^2~]\label{eq:derivative}
\end{equation*}


The exit point obtained between the local minima A and B is (-0.313,
0.971). Fig. \ref{fig:mullerbrownresult}a shows the results of our
algorithm on Muller-Brown surface. The dashed lines indicate the
initial search vector which is used to compute the exit point. The
dots indicate the points along the stability boundary obtained
during the trajectory adjustment procedure These dots move from the
exit point towards the MVP. The gradient curve corresponding to the
points along this stability boundary is shown in Fig.
\ref{fig:mullerbrownresult}b. From the MVP, the local minimizer is
applied to obtain decomposition point (DP 1). The exit point
obtained between the local minima B and C is (0.218, 0.292). It
converges to the decomposition point (DP 2) directly when the local
minimizer is obtained.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/mullerbrown_results.ps, width=2.5in}
\hspace{0.5in}\epsfig{figure=Figures/gradientcurve.ps, width=2.5in}
} \caption{(a) Results of our algorithm  to find the decomposition
points on Muller-Brown surface. The dashed lines indicate the
initial search direction. The dots indicate the results of the
trajectory adjustment procedure. These points are the points on the
stability boundary and they eventually reach the MVP. (b) The
gradient curve corresponding to the various points obtained from the
trajectory adjustment procedure. The graph shows that the magnitude
of the gradient slowly increases in the initial phases and then
starts to reduce. The highlighted point corresponds to the gradient
at the MVP.} \label{fig:mullerbrownresult}
\end{figure}

%\subsubsection*{Minyaev-Quapp surface}
%
%The Minyaev-Quapp surface forms a standard two-dimensional example
%of a potential energy function in theoretical chemistry \cite
%{Minyaev97}. Eq. (\ref {eq:minyaevquapp}) gives the Minyaev-Quapp
%energy function. Fig. \ref{fig:minyaevquapp} represents the
%two-dimensional contour plot of the potential energy surface of
%the Minyaev-Quapp function.
%\begin{equation} \label{eq:minyaevquapp}
%C(x,y) = cos(2x)+0.57cos(2(x-y)) + cos(2y)% & \quad
%\end{equation}
%
%As shown in Fig. \ref {fig:mullerbrown}, there are three local
%minima (A,B,C) and two decomposition points (1,2) on the
%muller-brown potential energy surface. Decomposition point 1 is
%present between two local minima A and B and it is more
%challenging to find it when compared to the decomposition point 2
%which is present between local minima B and C. Table~\ref
%{TB:mullerbrownresults} shows the energy values at the local
%minima and the decomposition points.
%
%\begin{table}[htp]
%\centering \caption{\protect\small Local Minima and Decomposition
%Points for the Muller-Brown Surface described in Eq. (\ref
%{eq:mullerbrown}).     (LM - Local Minimum, DP - Decomposition
%Point)}
%\begin{center}
%\begin{tabular}{|c|c|c|}
%\hline
%Equilibrium Points &  Location & Energy value c(.) \\
%\hline LM A & (-0.558,1.442) & -146.7 \\
%\hline DP 1 & (-0.822,0.624) & -40.67 \\
%\hline LM B & (-0.05,0.467) & -80.77 \\
%\hline DP 2 & (0.212,0.293) & -72.25 \\
%\hline LM C & (0.623,0.028) & -108.7 \\ \hline
%\end{tabular}
%\end{center}
%\label{TB:minyaevquappresults}
%\end{table}
%
%The dynamical system corresponding to (\ref{eq:minyaevquapp}) is
%given by
%
%\begin{equation}
%\nabla C(x) = ~-~\left[ \begin{array}{c} \frac{\partial
%C}{\partial x} \vspace{0.05in}\\
%\frac{\partial C}{\partial y} \\
%\end{array} \right]
%\end{equation}
%
%\begin{eqnarray*}
%\frac{\partial C}{\partial x} = -2~sin(2x)-1.14~sin(2(x-y))\\
%\frac{\partial C}{\partial y}= -2~sin(2y)+1.14~sin(2(x-y))
%\label{eq:dcdxy}
%\end{eqnarray*}
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/mullerbrown_results.ps, width=3.5in}
%} \caption{Results of our method used to find the decomposition
%point. The dotted lines indicate the position corresponding to the
%point on the gradient curve.} \label{fig:minyaevquapp}
%\end{figure}
%The exit point obtained between the local minima A and B is
%(-0.313, 0.971). From this exit point, it took 14 steps to move
%towards the minimum vector-field point(MVP). The gradient curve is
%shown in Fig. \ref{fig:minyaevquappgradientcurve}. From this MVP,
%the local minimizer is applied to obtain decomposition point (DP
%1). The exit point obtained between the two local minima B and C
%is (0.218, 0.292). It converged to the decomposition point (DP 2)
%directly when the local minimizer is obtained.
%
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/gradientcurve.ps, width=3.5in}
%} \caption{Results of our method used to find the decomposition
%point. The dotted lines indicate the position corresponding to the
%point on the gradient curve.}
%\label{fig:minyaevquappgradientcurve}
%\end{figure}
%

\subsection*{Test Case 2: Three-dimensional symmetric systems}
\label{sec:lennardjones} {\it Three atom Lennard Jones clusters :}
This system is mainly used to demonstrate a simplified version of
our algorithm. Our method has some advantages when applied to
energy surfaces that are symmetric in nature. To demonstrate thi,
we used the Lennard Jones pair potential which is the most common
and simplistic model for interaction between atoms. The Lennard
Jones potential is given by the Eq. (\ref{eq:lennjones}). For
simplicity, we applied reduced units, i.e. the values of
$\epsilon$ and $r_0$ are taken to be unity. Plot of Lennard-Jones
Potential of interaction between two atoms generated using Eq.
(\ref{eq:lennjones}) is shown in Fig. \ref{fig:lennardjones}. The
original problem is to find the global minima of the potential
energy surface obtained from the interaction between N atoms with
two-body central forces. In this example, we consider the
potential energy surface corresponding to the three-atom cluster
which exhibits symmetric behaviour along the x-axis.

\begin{center}
\begin{eqnarray}
V = \sum_{i=1}^{N-1} \sum_{j=i+1}^N v(r_{ij}) \nonumber \\
v(r_{ij}) = \epsilon\left[\left(\frac{r_0}{r_{ij}}\right)^{12} -
2\left(\frac{r_0}{r_{ij}}\right)^6\right] \label{eq:lennjones}
\end{eqnarray}
\end{center}
where \\
\centerline {$ r_{ij} = \sqrt {  (x_i - x_j)^2 + (y_i - y_j)^2 +
(z_i - z_j)^2 }$}
\\
$V$ is the total potential energy of the microcluster is given as
the summation of of all two-body interaction terms, $v(r_{ij})$ is
the potential energy term corresponding to the interaction of atom
$i$ with atom $j$, and $r_{ij}$ is the Euclidean distance between
$i$ and $j$. $\epsilon$ describes the strength of the interaction
and $r_0$ is the distance at which the potential is zero.

%%The constants $\epsilon$ and $r_0$ are important to determine the
%%strength and shape of the interaction. $\epsilon$ is the minimum
%%of the potential (energy scale) and $r_0$ is the distance at which
%%the potential is zero (length scale). If $r_0 = r_{ij}$, then the
%%potential is zero. So by changing $r_0$ one can move the whole
%%potential to the right or to the left. When the separation $r$ is
%%very small, the $\frac{1}{r^{12}}$ term dominates, and the
%%potential is strongly positive. Hence the $\frac{1}{r^{12}}$ term
%%describes the short range {\it repulsive potential} due to the
%%distortion of the electron clouds at small separations. In
%%contrast the $\frac{1}{r^6}$ predominates when the separation $r$
%%increases in magnitude. Hence the $\frac{1}{r^6}$ term describes
%%the {\it long-range attractive tail of the potential} between two
%%particles. The force between individual atoms is the negative of
%%the gradient of the potential.

\begin{figure}[htp]
\centerline{ \epsfig{figure=Figures/ljmorse.ps, width=3.5in}}
 \caption{Characteristic curves of Lennard-Jones potential and the Morse potential with all parameters set to unity.
 Solid line represents Lennard-Jones potential (\ref{eq:lennjones}) and the dashed line represents the Morse potential (\ref{eq:morsepotential}).} \label{fig:lennardjones}
\end{figure}

\begin{table}[htp]
\centering \caption{\protect\small Local minima and decomposition
points for the three atom Lennard Jones Cluster described in Eq.
(\ref {eq:lennjones}).     (LM - Local Minimum , DP -
Decomposition Point)}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
{\bf \scriptsize Equilibrium Point} &  {\bf \scriptsize Location} & {\bf \scriptsize Energy value c(.)} \\
\hline

LM A &$\left(\begin{tabular}{ccc}
0.0 & 0.0 & 0.0 \\
1.0 & 0.0 & 0.0 \\
0.5 & 0.866 & 0.0  \\ \end{tabular}\right)$&-3.000\\

\hline DP 1 & $\left(\begin{tabular}{ccc}
0.0 & 0.0 & 0.0 \\
2.0 & 0.0 & 0.0 \\
1.0 & 0.0 & 0.0  \\ \end{tabular}\right)$ & -2.031\\
 \hline LM B & $\left(\begin{tabular}{ccc}
0.0 & 0.0 & 0.0 \\
1.0 & 0.0 & 0.0 \\
0.5 & -0.866 & 0.0  \\ \end{tabular}\right)$ &-3.000 \\

\hline
\end{tabular}
\end{center}
\label{TB:results}
\end{table}

The dynamical system corresponding to (\ref{eq:lennjones}) is
given by
\begin{equation}
 \nabla V(x) = ~-~\left[ \begin{array}{ccc} \frac{\partial
V}{\partial x_1} & \frac{\partial V}{\partial y_1} &
\frac{\partial V}{\partial z_1}\vspace{0.05in} \\
\frac{\partial V}{\partial x_2} & \frac{\partial V}{\partial y_2}
& \frac{\partial V}{\partial z_2} \vspace{0.05in}\\
\frac{\partial V}{\partial x_3} & \frac{\partial V}{\partial y_3}
& \frac{\partial V}{\partial z_3} \end{array} \right]
\label{eq:finalderivative} \end{equation} where
%\begin{equation*}
%\frac{\partial V}{\partial x_i} =\sum_{j=1}^3 ~\frac{\partial
%V}{\partial r_{ij}}~ . ~\frac{\partial r_{ij}}{\partial x_i}
%\label{eq:derivative}
%\end{equation*}

%The partial derivative of the potential function w.r.t. $r_{ij}$
%is.
%\begin{equation}
%\frac{\partial V}{\partial r_{ij}} = \ 12
%\left[\left(\frac{1}{r_{ij}}\right)^{7} -
%\left(\frac{1}{r_{ij}}\right)^{13}\right] \label{eq:derivative1}
%\end{equation}
%The partial derivative of $r_{ij}$ w.r.t. individual cartesian
%coordinates is given by
%
%\begin{equation}
%\frac{\partial r_{ij}}{\partial x_i} =  \frac{x_i-x_j }{r_{ij}}
%\label{eq:derivative2}
%\end{equation}
%
%Substituting (\ref{eq:derivative1}) and (\ref{eq:derivative2}) in
%(\ref{eq:derivative}), we have
%\begin{equation*}
\[ \frac{\partial V}{\partial x_i} =\sum_{\substack{j=1\\j\neq i}}^3
~\frac{12}{(r_{ij})^8}
 ~ \left[ 1 - \left( \frac{1}{r_{ij}} \right)^6 \right]~ . ~
 (x_i-x_j)\]
%\label{eq:finalderivative}
%\end{equation*}

Based on the two given local minima, one can compute the exit
point analytically (not numerically) since the system is
symmetric. Since the exit point is an exact (not an approximate)
value, one can eventually reach the decomposition
point by integrating the exit point. The exit point is \\
\begin{center}
$\left(\begin{tabular}{ccc}
0.0 & 0.0 & 0.0 \\
1.0 & 0.0 & 0.0 \\
0.5 & 0.0 & 0.0  \\ \end{tabular}\right)$ \end{center}In this
case, there is no need to use the trajectory-adjustment procedure.
Integrating from the exit point will eventually find the
decomposition point. The last two steps of our method,
trajectory-adjustment procedure and the local minimizer are not
required to obtain the decomposition point. It is clear from the
above example that in all cases where we compute the exit point
numerically, we get an approximate of the exit point and hence it
will eventually converge to one of the two local minima after
integration. In such cases, the trajectory-adjustment procedure
will help us to maintain the path along the stability boundary and
prevents from being trapped in one of the local minima.

\subsection*{Test Case 3: Higher Dimensional Systems}
\label{sec:pes} {\it Heptamer island on a crystal:} To test our
method on a higher dimensional system, we have chosen a heptamer
island on the surface of an Face-Centered Cubic (FCC) crystal.
This system will not only illustrate the atomic scale mechanism of
island diffusion on surfaces but also will help us in
understanding the kinetics of a process. The atoms interact via a
pairwise additive Morse potential described by Eq. (\ref
{eq:morsepotential}).

\begin{equation}
V(r)\ = \ A~\left( e^{-2\alpha (r-r_0)}-2 e^{-\alpha
(r-r_0)}\right) \label{eq:morsepotential}
\end{equation}

where $A=0.71$~eV, $\alpha=1.61$~\AA$^{-1}$,\
$r_0=2.9$~\AA. \\

These parameters were chosen in such a way that it will reproduce
diffusion barriers on real surfaces. The potential was cut and
shifted at $9.5$~\AA. The surface is simulated with a 6 layer
slab, each layer containing 56 atoms. The minimum energy lattice
constant for the FCC solid is  $2.74$~\AA. The bottom three layers
in the slab are held fixed.  A total of 7 + 168 = 175 atoms are
allowed to move during the search for decomposition points. Hence,
this is an example of 525 (175 X 3) dimensional search problem.
This is the same system used in the review paper by Henkelman et
al \cite{Henkelman00b}. Fig. \ref{fig:minimum1} shows the top view
of the initial configuration of the island with a compact heptamer
sitting on top of the surface. The shading indicates the height of
the atoms. The white ones are the heptamer island on the surface
of the crystal and the black ones are at the bottom most part of
the crystal.
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/min01a.eps, width=2.5in}
} \caption{Top view of the surface and the seven atom island on
the surface of an FCC crystal. The shading indicates the height of
the atoms.} \label{fig:minimum1}
\end{figure}


%%We have focused on the
%%initial stage of such a configurational transition, i.e. saddle
%%points that are at the boundary of the potential basin
%%corresponding to the compact heptamer state. % A total of 13 processes were found with saddle
%%point energy less than or equal to $1.513$~eV. The lowest energy
%%processes correspond to uniform translation of the island from FCC
%%sites to HCP sites.  There are two slightly different directions
%%for the island to hop, and thus two slightly different saddle
%%points, of energy $0.601$~eV and $0.620$~eV (see figure 8).  The
%%next three low energy saddle points, processes 3 to 5, correspond
%%to a pair of edge atoms shifting to adjacent FCC sites. The three
%%processes are quite similar, just three slightly inequivalent
%%directions. Process 6 and 7 are quite interesting.  Here, a pair
%%of atoms is again shifted, but now only to the nearby HCP sites.
%%The other 5 atoms in the cluster are also shifted to adjacent HCP
%%sites but in the opposite direction.  The final state has all
%%island atoms sitting at HCP sites. Processes 8 and 9 involve a
%%concerted move of three edge atoms.  Process 10 and 11 involve an
%%edge dimer where one of the atoms moves in a direction away from
%%the island while the other one takes its place.  This is a
%%significantly higher energy final state, because of the low
%%coordination of one of the displaced atoms.  Finally, processes 12
%%and 13 involve the displacement of just one atom away from the
%%island, again resulting in low coordination in the final state.
%
%%One common feature of processes 3 to 13 is that the final state is
%%higher in energy than the initial state.  The saddle point is
%%typically late, i.e. close to the final state.
%
%%The potential shift at the cutoff distance is to ensure that the
%%energy is continuous.  So if the energy at the cutoff, E(Rc)=-Ec,
%%the energy will be zero if two atoms are separated by more than
%%Rc, but will jump to -Ec as soon as they get within the distance
%%Rc. To avoid that discontinuity (in the energy), the potential is
%%shifted by Ec so that the interaction energy is zero on either
%%side of the cutoff.
%
%%Its important to have a potential which is typical of interacting
%%atoms to show that your method is applicable to chemistry.  There
%%are some aspects of the problems we are interested in, such as a
%%very strong repulsion when atoms approach each other, a bonding
%%distance where atoms prefer to sit, and zero interaction when
%%atoms move apart.  However, this can be considered as an object
%%function, but it has this (qualitative) special form.

Let $N$ be the number of atoms that can move (175) and $N'$ be the
total number of atoms (343).
\begin{equation}
V(r)\ = \sum_{i=1}^N ~\sum_{j=1}^{N'} ~\ A~\left( e^{-2\alpha
(r_{ij}-r_0)}-2 e^{-\alpha (r_{ij}-r_0)}\right) \label{eq:energy}
\end{equation}

where $r_{ij}$ is the Euclidean distance between $i$ and $j$. The
\emph{Dynamical System} is a $3 \times N$~matrix
\[ \nabla V(X) =~-~ \left[ \begin{array}{ccc}
\frac{\partial V}{\partial x_1} & \frac{\partial V}{\partial y_1} & \frac{\partial V}{\partial z_1} \vspace{0.05in}\\
\frac{\partial V}{\partial x_2} & \frac{\partial V}{\partial y_2} & \frac{\partial V}{\partial z_2} \vspace{0.05in}\\
. & . & . \\
. & . & . \\
 &  &  \\
. & . & . \\
. & . & . \vspace{0.03in}\\
\frac{\partial V}{\partial x_n} & \frac{\partial V}{\partial y_n}
& \frac{\partial V}{\partial z_n} \end{array} \right]\]

where \\
\begin{equation}
\frac{\partial V}{\partial x_i} =\sum_{\substack{j=1\\j\neq i}}^n
\ 2\alpha A~\left( e^{-\alpha (r-r_0)}- e^{-2\alpha
(r-r_0)}\right)  . \frac{(x_i-x_j)}{r_{ij}} \label{eq:derivative}
\end{equation}
%
%%\begin{equation}
%%\frac{\delta F}{\delta r_{ij}} = \label{eq:derivative1}
%%\end{equation}
%%
%%\begin{equation}
%%\frac{\delta r_{ij}}{\delta x_i} = \label{eq:derivative2}
%%\end{equation}
%
%%\begin{figure}[htp]
%%\centerline{ \epsfig{figure=Figures/lennardjones.ps, width=3.5in}}
%% \caption{The average number of iterations required to get to the
%% best value achieved. This is an average of 100 trials.
%%~\ref{eq:lennjones}.} \label{fig:graph3}
%%\end{figure}
%


\begin{figure}[htp]
\begin{center}
\epsfig{figure=Figures/sp03.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/sp05.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/sp07.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/sp10.eps, width=0.6in} \hspace{0.15in}

\epsfig{figure=Figures/min03b.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/min05b.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/min07b.eps, width=0.6in} \hspace{0.15in}
\epsfig{figure=Figures/min10a.eps, width=0.6in} \hspace{0.15in}

\end{center}
\caption{Some sample configurations of the heptamer island on the
surface of the FCC crystal. First row- saddle points
configurations. Second row- corresponding other minimum energy
configurations.} \label{fig:atoms}
\end{figure}

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/gradientcurve2.ps, width=3.5in}
} \caption{The gradient curve obtained in one of the higher
dimensional test cases.} \label{fig:gradientcurve2}
\end{figure}
\begin{table}[htp]
\centering \caption{\protect\small Results of our algorithm on a
higher dimensional test system. Energy value at one of the minimum
is -1775.7911. $E_{min}$ is the energy value at the other minimum.
$E_{saddle}$ is the energy value at the saddle point.  $E_{MVP}$
is the energy value at the Minimum Vector Field Point. $RMSD$ is
the root mean square distance of all the atoms at the MVP and the
saddle point. $\Delta$Energy is the energy difference between
$E_{MVP}$ and $E_{saddle}$. $\Delta$ Force is the magnitude of the
gradient at the MVP. No. of evals is the number of force
evaluations made to compute the MVP. }
\begin{center}
\begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}|c|c|c|c|c|c|c|}
\hline
%{\bf \scriptsize Test Case} & {\bf \scriptsize }&{\bf \scriptsize Energy at } & {\bf \scriptsize Energy at} &{\bf \scriptsize } &  {\bf \scriptsize } & {\bf \scriptsize  No. of Force} \\
%{\bf \scriptsize Number} &  {\bf \scriptsize RMSD}& {\bf \scriptsize the MGP } & {\bf \scriptsize  the DP} &{\bf \scriptsize $\Delta$Energy} &  {\bf \scriptsize $\Delta $Force } & {\bf \scriptsize  evaluations} \\
Sl & $E_{min}$ & $E_{saddle}$ & $E_{MVP}$ &$RMSD$ & $\Delta$ Force & evals\\
No. & &  &  &&   &  \\
%Number & RMSD& the MGP & the DP & $\Delta$Energy & $\Delta$ Force & evaluations \\

%\hline 1 & -1775.7787   & -1775.19 & -1775.2139 & 0.00917 &
%0.02376 & 0.01833 & 49 \\
%\hline 2 & -1775.7787  & -1775.1716
% & -1775.1906& 0.00802 &  0.01903 & 0.01671
%& 43\\
%\hline 3 & -1775.0079 &-1774.8055  & -1774.8213 & 0.0121 & 0.01578 & 0.01664& 97\\
%\hline 4 & -1775.006  & -1774.8041  & -1774.9228
% & 0.03208 & 0.11868
%& 0.02654& 67\\
%\hline 5 & -1775.0058  & -1774.8024  & -1774.8149 & 0.01229 & 0.01256 & 0.01704 & 91\\
%\hline 6 & -1775.0942  &-1774.5956  & -1774.3819 & 0.04285 &
%-0.21362
% & 0.04343
%& 37\\
%\hline 7 & -1775.0931 &-1774.5841   & -1774.3916 &0.03296  &
%-0.19252
% & 0.03905& 43\\
%\hline 8 & -1775.01 &-1774.3106  & -1775.0789
% & 0.05287  & 0.76832
% & 0.04031& 97\\
%\hline 9 & -1775.0097 &-1774.3082
%  & -1775.0848
% & 0.05297 & 0.77662 & 0.04113
%& 97\\
%\hline 10 & -1774.3896
% &-1774.2979
% & -1774.9551 & 0.05623  & 0.65718
% & 0.03103& 79\\
%\hline 11 & -1774.3928  &-1774.2997   & -1774.9541
% & 0.05615  & 0.65439
% & 0.03086
%& 79\\
%\hline 12 & -1774.3933 &-1774.2792   & -1774.2938
% & 0.02262 & 0.01450& 0.07092& 19\\
%\hline
\hline 1 & -1775.7787   & -1775.19 & -1775.2139 & 0.00917 &
 0.01833 & 49 \\
\hline 2 & -1775.7787  & -1775.1716
 & -1775.1906& 0.00802  & 0.01671
& 43\\
\hline 3 & -1775.0079 &-1774.8055  & -1774.8213 & 0.0121  & 0.01664& 97\\
\hline 4 & -1775.006  & -1774.8041  & -1774.9228
 & 0.03208
& 0.02654& 67\\
\hline 5 & -1775.0058  & -1774.8024  & -1774.8149 & 0.01229 & 0.01704 & 91\\
\hline 6 & -1775.0942  &-1774.5956  & -1774.3819 & 0.04285
 & 0.04343
& 37\\
\hline 7 & -1775.0931 &-1774.5841   & -1774.3916 &0.03296
 & 0.03905& 43\\
\hline 8 & -1775.01 &-1774.3106  & -1775.0789
 & 0.05287
 & 0.04031& 97\\
\hline 9 & -1775.0097 &-1774.3082
  & -1775.0848
 & 0.05297  & 0.04113
& 97\\
\hline 10 & -1774.3896
 &-1774.2979
 & -1774.9551 & 0.05623  & 0.03103& 79\\
\hline 11 & -1774.3928  &-1774.2997   & -1774.9541
 & 0.05615
 & 0.03086
& 79\\
\hline 12 & -1774.3933 &-1774.2792   & -1774.2938
 & 0.02262 & 0.07092& 19\\
\hline
\end{tabular*}
\end{center}
\label{TB:highdimension}
\end{table}

To illustrate the importance of the minimum vector-field point and
the effectiveness of the boundary tracing, we compared our results
with that of the other methods reported in the review paper by
Henkelman et al. The results of our method is shown in Table
\ref{TB:highdimension}. The last column indicates the number of
gradient computations that were made to reach the minimum
vector-field point. As seen from the table, our method finds the
saddle points with less number of gradient computations when
compared to other methods. Typically, even the best available
method takes at least 200-300 evaluations of the gradient. For
detailed results about the performance of other methods refer to
\cite{Henkelman00b}. The performance of our method is not compared
directly with the results from the existing methods because the
results that were reported are for a gradient value of 0.01 and
the minimum vector field point that was computed in our case
varied from 0.01-0.05. However, the minimum vector field point can
be treated as a saddle point for most of the practical
applications. The RMSD (root mean square distance) value between
the MVP and the saddle point is very low. As discussed earlier, we
need to use a robust, efficient nonlinear system solver to reach
the saddle point from the minimum vector field point.

\subsection*{Special Cases}
\subsubsection{Eckhardt surface}

The Eckhardt surface is one more potential energy function in
theoretical chemistry \cite {Eckhardt88}. This example is shown as
an exceptional case where we need to perturb the exit point in order
to follow the stability boundary. Such cases almost never occur in
practice and hence dealing with such surfaces will not be given much
importance. Eq. (\ref {eq:eckhardt}) gives the Eckhardt energy
function. Fig. \ref{fig:eckhardt}a represents the two-dimensional
contour plot of the potential energy surface of the muller-brown
function.
\begin{equation} \label{eq:eckhardt}
%\begin{split}
C(x,y) = e^{ -[x^2 +(y+1)^2]} + e^{-[x^2+(y-1)^2]}+
4~e^{-[3(x^2+y^2)/2]}+y^2/2
%\end{split}
\end{equation}

As shown in Fig. \ref {fig:eckhardt}, there are two local minima
(A,B), two decomposition points (1,2) on the Eckhardt potential
energy surface. A local maximum is present exactly at the center
between the two local minima. The two decomposition points are on
either side of the maximum. Table~\ref{TB:Eckhardtresults} shows
the energy values at the local minima and the decomposition
points.


The dynamical system corresponding to (\ref{eq:eckhardt}) is given
by
\begin{center}
\begin{equation} \label{eq:mqdynamicalsystem}
\nabla C(x) = ~-~\left[ \begin{array}{c} \frac{\partial
C}{\partial x} \vspace{0.05in}\\
\frac{\partial C}{\partial y} \\
\end{array} \right]
\end{equation}
\end{center}
\begin{equation*}
%\begin{split}
\frac{\partial C}{\partial x} %&=
-2x~e^{-[x^2+(y+1)^2]}-2x~e^{-[x^2+(y-1)^2]}-12x~e^{-[3(x^2+y^2)/2]}
\label{eq:dcdx}%\end{split}
\end{equation*}
\begin{equation*}
%\begin{split}
\frac{\partial C}{\partial y} =
-2(y+1)~e^{-[x^2+(y+1)^2]}-2(y-1)~e^{-[x^2+(y-1)^2]}-12y~e^{-[3(x^2+y^2)/2]}+y
\label{eq:dcdy}
%\end{split}
\end{equation*}



This surface can be treated as a special case where there are
different critical points lying on the vector joining the two local
minimum. As seen from the figure, there is a local maximum at (0,0),
which is the exit point obtained. It should be noted that this
system is also symmetric and hence one can obtain the exit point
analytically. Since, the exit point is also a critical point, the
exit point is first perturbed and then the trajectory adjustment
procedure is used to compute the MVP. The two decomposition points
are at (0.0,1.4644) and (0.0,-1.4644). The gradient curve is shown
in Fig. \ref{fig:eckhardt}b. From this MVP, the local minimizer is
applied to obtain decomposition point (DP 1). The other
decomposition point (DP 2) is similarly obtained.

\begin{table}[htp]
\centering \caption{\protect\small Local Minima and Decomposition
Points for the Muller-Brown Surface described in Eq. (\ref
{eq:mullerbrown}). (MIN - Minimum, MAX - Maximum, DP -
Decomposition Point)}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Equilibrium Points &  Location & Energy value c(.) \\
\hline MIN A & (-3.0,0.0) & 0.0 \\
\hline DP 1 & (0.0,1.4644) & 2.0409 \\
\hline MIN B & (3.0,0.0) & 0.0 \\
\hline DP 2 & (0.0,-1.4644) & 2.0409 \\
\hline MAX M & (0.0,0.0) & 4.7358 \\ \hline
\end{tabular}
\end{center}
\label{TB:Eckhardtresults}
\end{table}

\begin{figure}[htp]
\centerline{
   \epsfig{figure=Figures/eckhardt1.ps, width=2.5in}
  \hspace{0.8in}\epsfig{figure=Figures/eckhardtgradientcurve.ps,
  width=2.5in}\\
} \caption{(a) Two dimensional contour plot of the potential energy
surface of the Eckhardt energy function described on Eq.
(\ref{eq:eckhardt}). A,B - two minima , M - maximum and 1,2 - two
decomposition points. (b)Results of our method used to find the
decomposition point. The dotted lines indicate the position
corresponding to the point on the gradient curve.}
\label{fig:eckhardt}
\end{figure}

%\begin{center}
%\begin{equation} \label{eq:edynamicalsystem}
%\nabla C(x) = ~-~\left[ \begin{array}{c} \frac{\partial
%C}{\partial x} \vspace{0.05in}\\
%\frac{\partial C}{\partial y} \\
%\end{array} \right]
%\end{equation}
%\end{center}
%where
%\begin{equation*}
%\frac{\partial C}{\partial x} = \sum_{i=1}^4
%A_i~.~P~.~[~2a_i(x-x_i^o)+
% b_i(y-y_i^o)~]
%\label{eq:dcdx}
%\end{equation*}
%
%\begin{equation*}
%\frac{\partial C}{\partial y}= \sum_{i=1}^4
%A_i~.~P~.~[~b_i(x-x_i^o)+2c_i(y-y_i^o)~] \label{eq:dcdx}
%\end{equation*}
%where \\
%\begin{equation*}
%P=exp~[~a_i(x-x_i^o)^2+ b_i(x-x_i^o)(y-y_i^o) +
%c_i(y-y_i^o)^2~]\label{eq:derivative}
%\end{equation*}


%\section{Conclusions and Future Research}
%\label{sec:conclusion}
%
%Saddle points play a vital role in realizing the folding pathways
%of a protein as well as in understanding the transition state
%structures during chemical reactions. This paper primarily focuses
%on a new method for finding saddle points on potential energy
%surfaces using stability boundaries. Our approach is based on some
%fundamental results of nonlinear dynamical systems. A new {\it
%trajectory adjustment procedure} has been used to move along the
%stability boundary. Our method was successful in finding the
%saddle points on different potential energy surfaces of varying
%dimensions. We have also explored the symmetric behaviour of some
%energy surfaces to obtain the exit point analytically and
%developed a simplified version of our algorithm to compute the
%saddle points. The algorithm has also been tested successfully on
%a heptamer island over the surface of an FCC crystal.
%
%As a continuation of this work, we are planning to implement a
%hierarchial approach for finding the global minimum on a potential
%energy surface. Combining our approach with any stochastic
%algorithm will enable us to search the entire solution space more
%effectively. This can be done by using the method presented in
%this paper as a tool for {\it escaping from a given local minimum
%to another local minimum in the neighborhood}. Though the current
%work assumes that the two local minima between which the saddle
%point is computed are given, it can be easily extended to find
%saddle points from a single local minimum. We would also like to
%exploit some other application areas where the energy surfaces are
%more complicated.
%
%
%\section*{APPENDIX-A:  LEPS Potential} \label{sec:appendix-A}
%The model of LEPS potential simulates a reaction involving three
%atoms confined to motion along a line. Only one bond can be formed
%either between atoms A and B or between atoms B and C.
%
%\begin{equation} \label{eq:lepspotential}
%%\begin{split}
% C(x,y)=
%\frac{Q_{AB}}{1+a}+\frac{Q_{BC}}{1+b}+\frac{Q_{AC}}{1+c}-\Bigl[\frac{J_{AB}^2}{(1+a)^2}
%+\frac{J_{BC}^2}{(1+b)^2}+\frac{J_{AC}^2}{(1+c)^2}+
%\frac{J_{AB}J_{BC}}{(1+a)(1+b)}
%+\frac{J_{BC}J_{AC}}{(1+b)(1+c)}+\frac{J_{AB}J_{AC}}{(1+a)(1+c)}\Bigr]^{\frac{1}{2}}
%%\end{split}
%\end{equation}
%
%where the $Q$ functions represent the Coulomb interactions between
%electron clouds and the nuclei and the $J$ functions represent the
%quantum mechanical exchange interactions. The form of the Q and J
%functions is given below:
%\begin{equation*}
%Q(r)\ =  \frac{d}{2}~\left( \frac{3}{2}e^{-2\alpha (r-r_0)}-
%e^{-\alpha (r-r_0)}\right) \label{eq:lepspotential1}
%\end{equation*}
%
%\begin{equation*}
%J(r)\ = \ \frac{d}{4}~\left( e^{-2\alpha (r-r_0)}-6 e^{-\alpha
%(r-r_0)}\right) \label{eq:lepspotential2}
%\end{equation*}
%
%The parameters were chosen to be $a=b=c=0.05$, $d_{AB} = d_{AC} =
%d_{BC} = 4.746$, $\alpha=1.942$ and $r_0=0.742$. The details about
%the LEPS potential are given in \cite{Polanyi69}.
%
%\section*{APPENDIX-B: Golden section search}\label{sec:appendix-B}
%The following procedure describes the golden section search
%method. Let $a$ and $b$ be the two intervals between which the
%{\it exit point} is located. Golden section search method computes
%the exit point with an accuracy of $\pm \epsilon$.
%$r$ is the {\it golden mean} ($\frac {3- \sqrt{5}}{2}$) \cite {Press92}. $f(x)$ returns the function value at point $x$. \\
%
%{\bf procedure\hspace{0.1in}}$GoldenSectionSearch(a,b,\epsilon)$
%\begin{algorithmic}[1]
%\STATE Initialize $r=0.38197$   (golden mean) \STATE $c=a+r(b-a)$
%\STATE $d=b-r(b-a)$
% \WHILE{$|b-a|>\epsilon$}
%    \IF{$f(c)>f(d)$}
%    \STATE $b=d,~d=c,~c=a+r(b-a)$
%    \ELSE
%    \STATE $a=c,~c=d,~d=b-r(b-a)$
%\ENDIF \ENDWHILE \STATE \bf return $b$
%\end{algorithmic}
%
%
%
%% optional entry into table of contents (if used)
%%%\addcontentsline{toc}{section}{Acknowledgment}
%%%This research was supported in part by the following grants: NSF
%%%IIS-0222831 and the MSU Foundation Strategic Partnership grant.
%%% trigger a \newpage just before the given reference
%%% number - used to balance the columns on the last page
%%% adjust value as needed - may need to be readjusted if
%%% the document is modified later
%%%\IEEEtriggeratref{8}
%%% The "triggered" command can be changed if desired:
%%%\IEEEtriggercmd{\enlargethispage{-5in}}
%%%
%%% references section
%%% NOTE: BibTeX documentation can be easily obtained at:
%%% http://www.ctan.org/tex-archive/biblio/bibtex/contrib/doc/
%%%
%%% can use a bibliography generated by BibTeX as a .bbl file
%%% standard IEEE bibliography style from:
%%% http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/bibtex
%%%\bibliographystyle{IEEEtran.bst}
%%% argument is your BibTeX string definitions and bibliography database(s)
%%%\bibliography{IEEEabrv,../bib/paper}
%%%
%%% <OR> manually copy in the resultant .bbl file
%%% set second argument of \begin to the number of references
%%% (used to reserve space for the reference number labels box)
%%%\begin{thebibliography}{1}
%%%
%%%\bibitem{IEEEhowto:kopka}
%%%H.~Kopka and P.~W. Daly, \emph{A Guide to {\LaTeX}}, 3rd~ed.\hskip 1em plus
%%%  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
%%%
%%%\end{thebibliography}
%%%


==> orig/supervised-global.tex <==
\section{Supervised Learning - Training ANNs}
\label{sec:training} Artificial neural networks (ANN) are powerful
statistical machine learning tools that are widely used in several
domains of science and engineering for problems like function
approximation, timeseries prediction, medical diagnosis, character
recognition, load forecasting, speaker identification, risk
management etc. They were developed in analogy to the human brain
for the purpose of improving conventional learning capabilities.
These networks serve as excellent approximators of nonlinear
continuous functions \cite{Leung03}. However, using an artificial
neural network to model a system involves in dealing with certain
difficulties in achieving the best representation of the
classification problem. Hence, it is vital to develop algorithms
that can exploit the power of a given network architecture and this
can be achieved by obtaining the global minimum of the error on the
training data along with the cross validation procedure. The main
focus of this section is to develop a robust training algorithm for
obtaining the optimal set of weights of an artificial neural network
by searching the parameter subspace in a systematic manner using
TRUST-TECH methodology.

\subsection{Network Description} \label{sec:background}

The main goal of optimal training of the network is to find a set of
weights that achieves the global minimum of the mean square error
(MSE) \cite{Haykin99}. We will consider a simple one hidden layer
neural network with $n$ (number of features) input nodes, $k$ hidden
nodes and $1$ output node. Thus, each network has $nk$ weights and
$k$ biases to the hidden layer, and $k$ weights and one bias to the
output node. Hence, training a neural network effectively is
necessarily a search problem of dimension $s=(n+2)k + 1$. The
network is trained to deliver the output value ($Y_i$) of the the
$i^{th}$ sample at the output node which will be compared to the
actual target value ($t_i$). The local minima problem is one of the
thoroughly studied aspects of neural networks \cite{Haykin99}.

The performance of a network is usually gauged by measuring the mean
square error (MSE) of its outputs from the expected targets. The
goal of optimal training is to find a set of parameters that
achieves the global minimum of the MSE
\cite{Haykin99,Shang96,Leung03}. For a $n$-dimensional dataset, the
MSE over $Q$ samples in the training set is given by:

\begin{equation}\label{eq:MSE}
    C(W) =\frac{1}{Q}\sum_{i=1}^Q \left[t(i)-y(W,X)\right]^2\\
\end{equation}

where $t$ is the target output, $X$ is the input vector and $W$ is
the weight vector. The MSE as a function of the parameters will
adopt a complex topology with several local optimal solutions. The
network's weights and thresholds must be set so as to minimize the
prediction error made by the network. Since it is not possible to
analytically determine the global minimum of the error surface, the
neural network training is essentially an exploration of the error
surface for an optimal set of parameters that attain this global
minimum.

Training algorithms can be broadly classified into `{\it local}' and
`{\it global}' methods. Local methods begin at some initial guesses
and deterministically lead to a nearby local minimum. From an
initial random configuration of weights and thresholds, the local
training methods incrementally seek for improved solution until they
reach local minima. Typically, some form of the gradient information
at the current point on the error surface is calculated and used to
make a downhill move. Advanced techniques like Genetic algorithms
and simulated annealing are applied in combination with standard
Backpropagation (BP) in order to allow for more promising solutions
and avoid being stuck at local minima. These methods can explore the
entire solution space effectively and obtain promising local optimal
solutions, but they lack fine-tuning capability to obtain a precise
final solution and require a local methods to be employed. From both
of the methods mentioned above, one can realize that there is a
clear gap between these methods and our approach tries to
communicate with both local and global methods.


\subsection{Problem Statement} \label{sec:training}

\begin{table}[h]
\centering \caption{\protect\small Description of the notations
used}
\begin{center}
\begin{tabular}{cl}
\hline  Notation &   Description \\
 \hline

 $Q$ & Number of training samples\\
 $X$ & Input vector\\
 $W$ & Weight vector\\
 $n$ & Number of features\\
 $k$ & Number of hidden nodes\\
 $w_{0j}$ & weight for $j^{th}$ hidden and the output node\\
 $w_{ij}$ & weight for $i^{th}$ input and $j^{th}$ hidden node \\
 $b_0$ & bias of the output node \\
 $b_j$ & bias of the $j^{th}$ hidden node \\
 $t_i$ & target value of the $i^{th}$ input sample\\
 $y$ & output of the network\\
 $e_i$ & Error for the $i^{th}$ input sample\\

 \hline

\end{tabular}
\end{center}
\label{TB:nota}
\end{table}
Table \ref{TB:nota} gives the important notations used in the rest
of this section. The final nonlinear mapping of the network model is
given by:
\begin{equation*}\label{eq:finalresult}
    y(W,X) =\phi_2\left( \sum_{j=1}^k w_{0j} \phi_1\left(\sum_{i=1}^n w_{ij}x_i+b_{j}\right)+b_{0}\right)
\end{equation*}
where $\phi_1$ and $\phi_2$ are the activation functions of the
hidden nodes and the output nodes respectively. $\phi_1$ and
$\phi_2$ can be same functions or can be different functions. We
have chosen to use $\phi_2$ to be sigmoidal and $\phi_1$ to be
linear. Results in the literature \cite{Gorse97}, suggest that this
set of activation functions yield the best results for feedforward
neural networks. The task of the network is to learn associations
between the input-output pairs
{$(X_1,t_1),(X_2,t_2),...,(X_Q,t_Q)$}. Without loss of generality,
lets construct the following weight vector :
\begin{equation*}\label{eq:Wvec}
{\scriptstyle
W=}(w_{01},w_{02},..,w_{0k},..,w_{n1},w_{n2},..,w_{nk},b_0,b_1,b_2..,b_k)^T
\end{equation*}
which includes all the weights and biases that are to be computed.
Hence, the problem of training neural networks is $s$-dimensional
unconstrained minimization problem where $s=(n+2)k+1$. The mean
squared error which is to be minimized can be written as
\begin{equation}\label{eq:JW}
    C({\scriptstyle W}) = \frac{1}{Q} \sum_{i=1}^{Q} e_i^2({\scriptstyle
  W})
\end{equation}
where the error $ e_i({\scriptstyle W}) = t_i-y({\scriptstyle
W},{\scriptstyle X_i})$. The error cost function $C(\cdot)$ averaged
over all training data is a highly nonlinear function of the
synaptic vector ${\scriptstyle W}$ Ignoring the constant for
simplicity, it can be shown that
\begin{eqnarray}
    \nabla C({\scriptstyle W}) = J^T({\scriptstyle W})e({\scriptstyle
    W})\\
\nabla^2 C({\scriptstyle W}) = J^T({\scriptstyle W})J({\scriptstyle
W})+S({\scriptstyle W}) \label{eq:firstderivative}
\end{eqnarray}
where $J({\scriptstyle W})$ is the Jacobian matrix
\[ J({\scriptstyle W}) = ~ \left[ \begin{array}{ccccc} \frac{\partial
e_1}{\partial {\scriptstyle W_1}} & \frac{\partial e_1}{\partial
{\scriptstyle W_2}} &.&.& \frac{\partial e_1}{\partial {\scriptstyle
W_s}}\vspace{0.05in}
\\\frac{\partial
e_2}{\partial {\scriptstyle W_1}} & \frac{\partial e_2}{\partial
{\scriptstyle W_2}} &.&.& \frac{\partial e_2}{\partial {\scriptstyle
W_s}}\vspace{0.05in}
\\ .&.&. &    &.\\
.&.& & .   &.\vspace{0.05in}\\
\frac{\partial e_Q}{\partial {\scriptstyle W_1}} & \frac{\partial
e_Q}{\partial {\scriptstyle W_2}} &.&.& \frac{\partial e_Q}{\partial
{\scriptstyle W_s}}\vspace{0.05in}
\end{array} \right]\]
and
\begin{equation}\label{eq:secondderivative}
    S({\scriptstyle W}) = \sum_{i=1}^{Q} e_i({\scriptstyle
  W}) \nabla^2 e_i({\scriptstyle W})\end{equation}
Generally, if we would like to minimize $J({\scriptstyle W})$ with
respect to the parameter vector ${\scriptstyle W}$, any variation of
Newton's method can be written as
\begin{equation}\label{eq:firstderivative}
\begin{split}
    \Delta {\scriptstyle W} &= -\left[\nabla^2 C({\scriptstyle W})\right]^{-1}~\nabla C({\scriptstyle W}) \\
    &=-\left[J^T({\scriptstyle W})J({\scriptstyle W})+S({\scriptstyle W})\right]^{-1} J^T({\scriptstyle W})e({\scriptstyle W}) \\
\end{split}
\end{equation}


\subsection{Problem Transformation}
This section mainly deals with the transformation of the original
likelihood function into its corresponding nonlinear dynamical
system and introduces some terminology pertinent to comprehend our
algorithm. This transformation gives the correspondence between all
the critical points of the error surface and that of its
corresponding gradient system as described earlier. To analyze the
geometric structure of the error surface, we build a {\it
generalized gradient system} described by
\begin{equation}\label{eq:dwdt}
    \frac{d{\scriptstyle W}}{dt} = -grad_R ~C({\scriptstyle W})= -R({\scriptstyle W})^{-1}\nabla C({\scriptstyle W})
\end{equation}
where the error function $C$ is assumed to be twice differentiable
to guarantee unique solution for each initial condition
${\scriptstyle W}(0)$ and $R({\scriptstyle W})$ is a positive
definite symmetric matrix (also known as {\it Reimannian metric})
for all ${\scriptstyle W} \in \Re^s$. The state vector $\scriptstyle
W$ belongs to the Euclidean space $\Re^s$, and the vector field $C :
\Re^s \rightarrow \Re^s$ satisfies the sufficient condition for the
existence and uniqueness of the solutions. A state vector
$\scriptstyle W$ is called an {\it equilibrium point} of Eq.
(\ref{eq:dwdt}) if $C({\scriptstyle W} )=0$. An equilibrium point is
said to be {\it hyperbolic} if the Jacobian of $C$ at point
$\bar{\scriptstyle W}$ has no eigenvalues with zero real part.

It is interesting to note the relationship between (\ref{eq:dwdt})
and (\ref{eq:firstderivative}) and obtain different local solving
methods used to find the nearest local optimal solution with
guaranteed convergence. For example, if $R({\scriptstyle W})=I$,
then it is a naive error back-propagation algorithm. If
$R({\scriptstyle W})=[J({\scriptstyle W})^T J({\scriptstyle W})]$
then it is the Gauss-Newton method and if $R({\scriptstyle
W})=[J({\scriptstyle W})^T J({\scriptstyle W})+\mu I]$ then it is
the Levenberg-Marquardt (LM) method.


\subsection{TRUST-TECH based Algorithm} \label{sec:algorithm} The proposed algorithm uses a promising starting point ($A^*$) as input and outputs the best local minimum of the neighborhood in the
weight space.

%Figure \ref{fig:flowchart} shows the flowchart of our approach.
%
%
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/flowchart.ps, width=3.0in}
%} \caption{Flow chart of our method} \label{fig:flowchart}
%\end{figure}

\noindent \textbf{Input:} Initial guess($A^*$), Tolerance ($\tau$),
Step size ($s$)
\\\textbf{Output:} Best local minimum ($A_{ij}$) in the neighborhood
\\\textbf{Algorithm:}\\
{\it Step 1: Obtaining good initial guess ($A^*$):} The initial
guess for the algorithm can be obtained from global search methods
or from a purely random start. Some domain knowledge about the
specific dataset that the network is being trained on, might help in
eliminating non-promising set of initial weights.
\\{\it Step 2: Moving to the local minimum ($M$):}
Using an appropriate local solver (such as conjugate-gradient,
quasi-Newton or Levenberg-Marquardt), the local optimum $M$ is
obtained using $A^*$ as the initial guess. \\{\it Step 3:
Determining the search direction ($d_j$):} The eigenvectors $d_j$ of
the Jacobian are computed at $m_i$. These eigenvector directions
might lead to
promising regions of the subspace. Other search directions can also be chosen based on the specific problem that is being dealt. \\
{\it Step 4: Escaping from the local minimum: } Taking small step
sizes away from $m_i$ along the $d_j$ directions increases the
objective function value till it hits the stability boundary.
However, the objective function value then decreases after the
search trajectory moves away from the exit point. This new point is
used as initial guess and local solver is applied again (go to Step
2).
\\ {\it Step 5: Finding Tier-1 local minima ($A_{1i}$):} Exploring the neighborhood of the local optimal solution corresponding to
the initial guess leads to tier-1 local minima. Exploring from tier-$k$ local minima leads to tier-$k+1$ local minima. \\
{\it Step 6: Exploring Tier-$k$ local minima ($A_{kj}$):} Explore
all other tiers in the similar manner described above. From all these solutions, the best one is chosen to be the desired global optimum.\\
{\it Step 7: Termination Criteria:} The procedure can be terminated
when the best solution obtained so far is satisfactory (lesser than
$sol_{req}$) or a predefined maximum number of tiers is explored.

\begin{figure}
\centerline{
  \epsfig{figure=Figures/dia.ps, width=3.0in}
} \caption{Illustration of Tier-2 TRUST-TECH procedure for obtaining
neighborhood local minima. } \label{fig:Diagram}
\end{figure}

Fig.~\ref{fig:Diagram} illustrates two-tier TRUST-TECH methodology.
The `*' represents the initial guess. Dotted arrows represent the
convergence of the local solver. Solid arrows represent the gradient
ascent linear searches along eigenvector directions. `X' indicates a
new initial condition in the neighborhood stability region. $M$
represents the local minimum obtained by applying local methods from
'X'. $A_{1i}$ indicates Tier-1 local minima. $e_{1i}$ are the exit
points between $M$ and $A_{1i}$. Similarly, $A_{2j}$ and $e_{2j}$
are the second-tier local minima and their corresponding exit points
respectively.

\subsection{Implementation Details} \label{sec:implementation} All
programs were implemented in MATLAB v6.5 and run on Pentium IV 2.8
GHz machines. We will now describe some implementation issues of our
algorithm. It is effective to use TRUST-TECH methodology for those
promising solutions obtained from stochastic global methods. Hence,
our algorithm assumes that it is being invoked from a promising set
of initial parameters. Algorithm \ref{trustech} describes the
two-tier TRUST-TECH algorithm. $NET$ assumes to have a fixed
architecture with a single output node. $ss$ is the step size
required for moving out of the stability region to obtain the exit
point. $\tau$ is the tolerance of error used for the convergence of
the local method. $Weights$ give the initial set of weight parameter
values. $Train$ function implements the Levenberg-Marquardt method
that obtains the local optimal solution from the initial condition.
The procedure $Estimate$ computes the mean square error (MSE) value
of the network model. A threshold value ($Thresh$) is set based on
this MSE value. The procedure $Neighbors$ returns all the next tier
local optimal solutions from a given local solution. After obtaining
all the tier-1 solutions, Neighbors is again invoked (only for
promising solutions) to obtain the second-tier solutions. The
algorithm finally compares the initial solution, tier-1 and tier-2
solutions and returns the network corresponding to the lowest error
among all these solutions.


\begin{algorithm}
\caption{$TRUST\_TECH\_NET$($NET, Wts,ss,\tau$)} \label{trustech}
\begin{algorithmic}
\STATE $Wts=Train(NET,Wts,\tau)$ \STATE$Error=Estimate(NET, Wts)$

    \STATE $Thresh=c*Error$
\STATE$Wts1[~]=Neighbors(NET,Wts,ss,\tau)$ \FOR{$k=1$ to
$size(Wts1)$}

\IF{$Estimate(NET,Wts1[k])<Thresh$} \STATE
$Wts2[k][~]=Neighbors(NET,Wts1,ss,\tau)$ \ENDIF

\ENDFOR \STATE \bf Return $best(Wts,Wts1,Wts2)$
\end{algorithmic}
\end{algorithm}
\begin{algorithm}
\caption{$Wts[~]$  $Neighbors~$($NET, Wts$,~$ss$,~$\tau$)}
\label{Neighbors}
\begin{algorithmic}

    \STATE $[Wts,Hess]=Train(NET,Wts,\tau)$
\STATE $evec=Eig\_Vec (Hess)$ \STATE $Wts[~]=NULL$

\FOR{$k=1$ to $size(evec)$} \STATE $Old\_Wts= Wts$ \STATE $
ext\_Pt=Find\_Ext(NET,Old\_Wts,ss,evec[k])$

\IF{$(ext\_Pt)$} \STATE $New\_Wts=Move(NET,Old\_Wts,evec[k])$

    \STATE $New\_Wts=Train(NET,New\_Wts,\tau)$
    \STATE $Errors=Estimate(NET,New\_Wts)$
\STATE $Wts[~]=Append(Wts[~],New\_Wts,Errors)$

\ENDIF \ENDFOR \STATE \bf Return $Wts[~]$
\end{algorithmic}
\end{algorithm}

The approximate Hessian matrix used for updation in the
Levenberg-Marquardt method is utilized to obtain the search
direction. Since there is no optimal way of obtaining promising
search directions, the Eigen vectors of this Hessian matrix are used
as search directions. Along each search direction, the exit point is
obtained by evaluating the function value along that particular
direction. The step size for evaluation is chosen to be the average
step size taken during the convergence of the local procedure. The
function value increases initially and then starts to reduce
indicating the presence of exit point on the stability boundary.
$Move$ function ensures that a new point (obtained from the exit
point) is located in a different (neighboring) stability region.
From this new initial guess, the local method is applied again to
obtain the local optimal solution of the neighborhood stability
region. The search for exit points along these directions will be
stopped if exit points are not found after certain number of
function evaluations.

\begin{table}[htp]
\centering \caption{\protect\small Summary of Benchmark Datasets.
Dataset (D), Sample size (Q), Input features (n), Output classes
(p), No. of Hidden nodes (k), No. of search variables ((n+2)k+1)}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
%&   Sample &Input &   Output & Hidden&
%Search \\
%Dataset &   Size &Features &   Classes& Nodes&
%Variables \\
  D&Q &  n &   p & k&
(n+2)k+1\\
\hline

\hline Cancer & 683&9 &  2&    5 &  56 \\\hline Diabetes & 178&  8&
3 & 4& 61\\ \hline Image& 2310&19& 7 &   8 &169 \\ \hline
Ionosphere& 351&34 & 2& 9& 325 \\ \hline Iris  &150& 4 &  3&  3& 19 \\ \hline Sonar & 208& 60& 2&  8  & 497 \\
\hline Wine & 178& 13&  3 &   4& 61\\  \hline
\end{tabular}
\end{center}
\label{TB:data1}
\end{table}


\subsection{Experimental Results} \label{sec:results}
Our algorithm is evaluated using seven benchmark datasets in the UCI
machine learning repository \cite{Blake98}. Optimal architectures
have been fixed for the networks based on some heuristic training.
The main focus of our algorithm is to demonstrate the capability of
obtaining optimal weight parameters and improvements in the
generalization ability of the networks. Table~\ref{TB:data1}
summarizes the datasets. It gives the number of samples, input
features, output classes along with the number of hidden nodes of
the optimal architecture. These datasets have varying degrees of
complexity in terms of sample size, output classes and the class
overlaps. To demonstrate the generalization capability (and hence
the robustness) of the training algorithm, 10-fold cross validation
is performed on each dataset. The criteria of evaluation is given by
the classification accuracy of the network model in terms of the
percentage of misclassified samples in the test cases. Tables
~\ref{TB:results} and ~\ref{TB:results1} shows the improvements in
the train error and the test error using TRUST-TECH methodology when
multiple random starts (MRS) and MATLAB initialization
(Nguyen-Widrow (NW) algorithm \cite{Nguyen90}) is used. Five tier-1
and corresponding tier-2 solutions were obtained using the
TRUST-TECH strategy. For some of the datasets, there had been
considerable improvements in the classifier performance. Spiderweb
diagram (shown in Fig. \ref{fig:spider}) a pretentious way to
demonstrate the improvements in a tier-by-tier manner.

\begin{table}[htp]
\centering \caption{\protect\small Percentage improvements in the
classification accuracies over the training and test data using
TRUST-TECH with multiple random restarts. }
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 &\multicolumn{3}{c|}{Train Error}&\multicolumn{3}{c|}{Test Error}\\
\cline{2-7}
Dataset &MRS+LM&TRUST-TECH&Improvement&MRS+LM&TRUST-TECH&Improvement\\
\hline\hline

Cancer & 2.21  &  1.74   & 27.01 &  3.95   & 2.63 &   50.19 \\
\hline Image &9.37 &8.04  &  16.54  & 11.08  & 9.74  &  13.76 \\
\hline Ionosphere &2.35 &0.57 &312.28 & 10.25 &  7.96 &   28.77 \\
\hline Iris &1.25 &1.00 &25.00 &3.33 &2.67 &24.72 \\ \hline Diabetes
& 22.04 &20.69 &6.52 &23.83 &20.58& 15.79 \\ \hline Sonar& 1.56&
0.72 &116.67& 19.17 &12.98& 47.69 \\ \hline Wine &4.56& 3.58& 27.37&
14.94 &6.73 &121.99 \\ \hline



\end{tabular}
\end{center}
\label{TB:results}\end{table}

\begin{table}[htp]
\centering \caption{\protect\small Percentage improvements in the
classification accuracies over the training and test data using
TRUST-TECH with MATLAB initialization. }
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 &\multicolumn{3}{c|}{Train Error}&\multicolumn{3}{c|}{Test Error}\\
\cline{2-7}
Dataset &NW+LM&TRUST-TECH&Improvement&NW+LM&TRUST-TECH&Improvement\\
\hline\hline

Cancer & 2.25  &  1.57 &42.99& 3.65 &   3.06 &   19.06 \\
\hline  Image  & 7.48  &  5.17  &  44.82 &  9.39  &  7.40   & 26.90\\
\hline Ionosphere & 1.56 &0.92 &   69.57 &  8.67   & 6.54  &  32.57\\
\hline Iris &1.33   & 0.67   & 100.00 & 3.33 &   2.67  &  25.00  \\
\hline Diabetes & 21.41 &19.55 &9.53 &23.70 &21.09& 12.37 \\ \hline
Sonar& 2.35 &0.42 &456.96 & 17.26 &  14.38  & 20.03 \\ \hline  Wine
& 7.60 &1.62 &370.06 & 14.54 &4.48 &224.82 \\ \hline
\end{tabular}
\end{center}
\label{TB:results1}\end{table}




\begin{figure*}[htp]
   \centering
   \subfigure[Wine Dataset]{\includegraphics[width = 2.25 in]{Figures/wine.ps}}
   \subfigure[Diabetes Dataset]{\includegraphics[width = 2.25 in]{Figures/pima.ps}}
   \subfigure[Cancer Dataset]{\includegraphics[width = 2.25 in]{Figures/cancer.ps}}
   \subfigure[Image Dataset]{\includegraphics[width = 2.25 in]{Figures/image.ps}}

   \caption{\label{fig:spider} Spider web diagrams showing the tier-1 and tier-2 improvements using TRUST-TECH method on various benchmark datasets. The circle in the middle of the plot represents the starting local optimal solution. The basic two
dimensions are chosen arbitrarily for effective visualization and
the vertical axis represents the percentage improvement in the
classification accuracy. The basis two axes are chosen arbitrarily
and the vertical axis represents the improvements in the classifier
accuracy. The five blue vertical lines surrounding the center circle
are the best five local minima obtained from a tier 1 search across
all folds. The five best second-tier improvements are plotted using
red lines. }
 \end{figure*}


==> orig/supervised.tex <==
\section{Supervised Learning - Training Neural Networks}

In this section, we demonstrate the ability of the stability region based methods to obtain multiple local minima on the error surface during the training procedure of artificial neural networks (ANN) \cite{Chiang06}. ANNs are powerful statistical machine
learning tools that are widely used in several domains of science
and engineering for problems like function approximation, timeseries
prediction, medical diagnosis, character recognition, load
forecasting, speaker identification, risk management etc. They were
developed in analogy to the human brain for the purpose of improving
conventional learning capabilities. These networks serve as
excellent approximators of nonlinear continuous functions
\cite{Leung03}. However, using an artificial neural network to model
a system involves in dealing with certain difficulties in achieving
the best representation of the classification problem. The two
challenging tasks in the process of learning using ANNs are network
architecture selection and optimal training. In deciding the
architecture, a larger network will always provide better prediction
accuracy for the data available \cite{Branke95}. However, such a
large network that is too complicated to model and also it might be
customized to some given problem and hence will lose its
generalization capability for the unseen data. Also, every
additional node into the network translates to increased hardware
cost.

Hence, it is vital to develop algorithms that can exploit the power
of a given network architecture and this can be achieved by
obtaining the global minimum of the error on the training data along
with the cross validation procedure. The main goal of optimal
training of the network is to find a set of weights that achieves
the global minimum of the mean square error (MSE) \cite{Haykin99}.
We will consider a simple one hidden layer neural network with $n$
(number of features) input nodes, $k$ hidden nodes and $1$ output
node. Thus, each network has $nk$ weights and $k$ biases to the
hidden layer, and $k$ weights and one bias to the output node.
Hence, training a neural network effectively is necessarily a search
problem of dimension $s=(n+2)k + 1$. The network is trained to
deliver the output value ($Y_i$) of the the $i^{th}$ sample at the
output node which will be compared to the actual target value
($t_i$). The local minima problem is one of the thoroughly studied
aspects of neural networks \cite{Gori92}. To avoid this problem,
some global methods like multiple random starts, genetic algorithms,
simulated annealing etc. can identify promising regions of the
weight space, but are time-consuming and are essentially stochastic
in nature. Expecting such stochastic algorithms to fine-tune the
training weights will be even more time consuming. Thus, there is a
necessity to efficiently search for good solutions in promising
regions of the solution space. The main focus of this is to develop a robust training
algorithm for obtaining the optimal set of weights of an artificial
neural network by searching the parameter subspace in a systematic
manner using the concepts of stability regions that were presented earlier.

\subsection{Background}
\label{sec:background}

The performance of a network is usually gauged by measuring the mean
square error (MSE) of its outputs from the expected targets. The
goal of optimal training is to find a set of parameters that
achieves the global minimum of the MSE
\cite{Bishop95,Shang96,Leung03}. For a $n$-dimensional dataset, the
MSE over $Q$ samples in the training set is given by:

\begin{equation}\label{eq:MSE}
    C(W) =\frac{1}{Q}\sum_{i=1}^Q \left[t(i)-y(X,W)\right]^2\\
\end{equation}

where $t$ is the target output, $X$ is the input vector and $W$ is
the weight vector. The MSE as a function of the parameters will
adopt a complex topology with several local optimal solutions. The
network's weights and thresholds must be set so as to minimize the
prediction error made by the network. Since it is not possible to
analytically determine the global minimum of the error surface, the
neural network training is essentially an exploration of the error
surface for an optimal set of parameters that attain this global
minimum.

Training algorithms can be broadly classified into `{\it local}' and
`{\it global}' methods. Local methods begin at some initial guesses
and deterministically lead to a nearby local minimum. From an
initial random configuration of weights and thresholds, the local
training methods incrementally seek for improved solution until they
reach local minima. Typically, some form of the gradient information
at the current point on the error surface is calculated and used to
make a downhill move. Based on the movement towards improved
solutions, local methods can be subdivided into two categories: (1)
Line search methods that minimize the function repeatedly along some
descent directions until the local minimum is reached (e.g. Newton's
method, BFGS method and conjugate gradient methods). (2) Trust
region methods where the surface is assumed to be a simple model
(like a parabola) such that the minimum can be located directly if
the model assumption is good (e.g. Levenberg-Marquardt(LM) method).
More details on these methods are described in \cite{Haykin99}.
%
%\begin{figure*}[htp]
%\centerline{
%  \epsfig{figure=Figures/arch.ps, width=6.5in}
%} \caption{Block Diagram of the architecture of our method.}
%\label{fig:block}
%\end{figure*}


All these local methods discussed so far assume that they already
have an initial guess to begin with. Due to the high non-linearity
of the error surface, the quality of the final solution depends
significantly on the initial set of parameters available. In
practice, most of these methods are typically combined with
stochastic global methods which yield a promising set of parameters
in the weight space. These global methods explore the entire error
surface and thus the chance of attaining a near-global optimal
solution is high. Advanced techniques like Genetic algorithms and
simulated annealing are applied in combination with standard BP
inorder to allow for more promising solutions and avoid being stuck
at local minima \cite{Reeves93}. Inspite of their (asymptotic)
guarantees in convergence to the global minimum, even for simple
learning tasks, these usually exhibits are very slow. Also, these
methods can explore the entire solution space effectively and obtain
promising local optimal solutions, but they lack fine-tuning
capability to obtain a precise final solution and require a local
methods to be employed. From both of the methods mentioned above,
one can realize that there is a clear gap between these methods and
our approach tries to communicate with both local and global
methods.

%Fig. \ref{fig:block} shows the block diagram of the TRUST-TECH
%methodology.

 Probably, the algorithms that resemble our methodology
are TRUST \cite{Cetin93} and dynamic tunneling
\cite{RoyChowdhury99}. These methods attempt to move out of the
local minimum in a stochastic manner. The training algorithm
proposed here differs from these methods by
deterministically escaping out of the local minimum and
systematically exploring multiple local minima on the error surface
in a tier-by-tier manner in order to advance towards the global
minimum. This approach is based on the fundamental concepts of
stability regions that were established in \cite{Chiang96,Lee04}.
 Basically, a global method yields initial points in
certain promising regions of the search space. These promising
initial points are used to search the neighborhood subspace in a
systematic manner. TRUST-TECH relies on a robust, fast local method
to obtain a local optimal solution. It explores the subspace in a
tier-by-tier manner by transforming the function into its
corresponding dynamical system and exploring the neighboring
stability regions. Thus, it gives a set of promising local optimal
solutions from which a global minimum is selected. In this manner,
TRUST-TECH can be treated as an effective interface between the
global and local methods, which enables the communication between
these two methods. It also allows the flexibility of choosing
different global and local methods depending on their availability
and performance for certain specific classification tasks. Also,
using our procedure, we will be able to truncate global methods at
early stages and not use them to fine-tune the solutions and thus
saving a lot of computational effort.

\subsection{Problem Formulation}
\label{sec:training}

\begin{table}[h]
\centering \caption{\protect\small Description of the notations
used}
\begin{center}
\begin{tabular}{cl}
\hline  Notation &   Description \\
 \hline

 $Q$ & Number of training samples\\
 $X$ & Input vector\\
 $W$ & Weight vector\\
 $n$ & Number of features\\
 $k$ & Number of hidden nodes\\
 $w_{0j}$ & weight for $j^{th}$ hidden and the output node\\
 $w_{ij}$ & weight for $i^{th}$ input and $j^{th}$ hidden node \\
 $b_0$ & bias of the output node \\
 $b_j$ & bias of the $j^{th}$ hidden node \\
 $t_i$ & target value of the $i^{th}$ input sample\\
 $y$ & output of the network\\
 $e_i$ & Error for the $i^{th}$ input sample\\

 \hline

\end{tabular}
\end{center}
\label{TB:nota}
\end{table}
Table \ref{TB:nota} gives the important notations used here. The final nonlinear mapping of the network model is
given by:
\begin{equation*}\label{eq:finalresult}
    y(W,X) =\phi_2\left( \sum_{j=1}^k w_{0j} \phi_1\left(\sum_{i=1}^n w_{ij}x_i+b_{j}\right)+b_{0}\right)
\end{equation*}
where $\phi_1$ and $\phi_2$ are the activation functions of the
hidden nodes and the output nodes respectively. $\phi_1$ and
$\phi_2$ can be same functions or can be different functions. We
have chosen to use $\phi_2$ to be sigmoidal and $\phi_1$ to be
linear. Results in the literature \cite{Gorse97}, suggest that this
set of activation functions yield the best results for feedforward
neural networks. The task of the network is to learn associations
between the input-output pairs
{$(X_1,t_1),(X_2,t_2),...,(X_Q,t_Q)$}. Without loss of generality,
lets construct the following weight vector :
\begin{equation*}\label{eq:Wvec}
{\scriptstyle
W=}(w_{01},w_{02},..,w_{0k},..,w_{n1},w_{n2},..,w_{nk},b_0,b_1,b_2..,b_k)^T
\end{equation*}
which includes all the weights and biases that are to be computed.
Hence, the problem of training neural networks is $s$-dimensional
unconstrained minimization problem where $s=(n+2)k+1$. The mean
squared error which is to be minimized can be written as
\begin{equation}\label{eq:JW}
    C({\scriptstyle W}) = \frac{1}{Q} \sum_{i=1}^{Q} e_i^2({\scriptstyle
  W})
\end{equation}
where the error $ e_i({\scriptstyle W}) = t_i-y({\scriptstyle
W},{\scriptstyle X_i})$. The error cost function $C(\cdot)$ averaged
over all training data is a highly nonlinear function of the
synaptic vector ${\scriptstyle W}$ Ignoring the constant for
simplicity, it can be shown that
\begin{eqnarray}
    \nabla C({\scriptstyle W}) = J^T({\scriptstyle W})e({\scriptstyle
    W})\\
\nabla^2 C({\scriptstyle W}) = J^T({\scriptstyle W})J({\scriptstyle
W})+S({\scriptstyle W}) \label{eq:firstderivative}
\end{eqnarray}
where $J({\scriptstyle W})$ is the Jacobian matrix
\[ J({\scriptstyle W}) = ~ \left[ \begin{array}{ccccc} \frac{\partial
e_1}{\partial {\scriptstyle W_1}} & \frac{\partial e_1}{\partial
{\scriptstyle W_2}} &.&.& \frac{\partial e_1}{\partial {\scriptstyle
W_s}}\vspace{0.05in}
\\\frac{\partial
e_2}{\partial {\scriptstyle W_1}} & \frac{\partial e_2}{\partial
{\scriptstyle W_2}} &.&.& \frac{\partial e_2}{\partial {\scriptstyle
W_s}}\vspace{0.05in}
\\ .&.&. &    &.\\
.&.& & .   &.\vspace{0.05in}\\
\frac{\partial e_Q}{\partial {\scriptstyle W_1}} & \frac{\partial
e_Q}{\partial {\scriptstyle W_2}} &.&.& \frac{\partial e_Q}{\partial
{\scriptstyle W_s}}\vspace{0.05in}
\end{array} \right]\]
and
\begin{equation}\label{eq:secondderivative}
    S({\scriptstyle W}) = \sum_{i=1}^{Q} e_i({\scriptstyle
  W}) \nabla^2 e_i({\scriptstyle W})\end{equation}
Generally, if we would like to minimize $J({\scriptstyle W})$ with
respect to the parameter vector ${\scriptstyle W}$, any variation of
Newton's method can be written as
\begin{equation}\label{eq:firstderivative}
\begin{split}
    \Delta {\scriptstyle W} &= -\left[\nabla^2 C({\scriptstyle W})\right]^{-1}~\nabla C({\scriptstyle W}) \\
    &=-\left[J^T({\scriptstyle W})J({\scriptstyle W})+S({\scriptstyle W})\right]^{-1} J^T({\scriptstyle W})e({\scriptstyle W}) \\
\end{split}
\end{equation}
\subsection{Stability Region based Approach }
\label{sec:trans} In this work, we exploit the geometric and
topological structure of the error surface to explore multiple local
optimal solutions in a systematic manner. Firstly, we describe the
transformation of the original problem into its corresponding
nonlinear dynamical system and then propose a new algorithm for
finding multiple local optimal solutions.


%\begin{lem}\label{def:criticalpoint}
%$\bar{\scriptstyle W}$ is said to be a {\it critical point} if it
%satisfies the condition $ \nabla C(\bar{\scriptstyle W})=0$
%\end{lem}
%We construct the following {\it gradient system} in order to locate
%critical points of the objective function (\ref{eq:problem}):
%
%%\begin{equation}
%%\dot{x}(t) = f(x(t))\label{eq:nonlineardynamicalsystems}
%%\end{equation}
%
%\begin{equation}
% \dot{\scriptstyle W}(t)=-\nabla f(\scriptstyle W)\label{eq:gradientsystem}
%\end{equation}

\subsubsection{Problem Transformation}
This section mainly deals with the transformation of the original
likelihood function into its corresponding nonlinear dynamical
system and introduces some terminology pertinent to comprehend our
algorithm. This transformation gives the correspondence between all
the critical points of the error surface and that of its
corresponding gradient system. To analyze the geometric structure of
the error surface, we build a {\it generalized gradient system}
described by
\begin{equation}\label{eq:dwdt}
    \frac{d{\scriptstyle W}}{dt} = -grad_R ~C({\scriptstyle W})= -R({\scriptstyle W})^{-1}\nabla C({\scriptstyle W})
\end{equation}
where the error function $C$ is assumed to be twice differentiable
to guarantee unique solution for each initial condition
${\scriptstyle W}(0)$ and $R({\scriptstyle W})$ is a positive
definite symmetric matrix (also known as {\it Reimannian metric})
for all ${\scriptstyle W} \in \Re^s$. It is interesting to note the relationship between (\ref{eq:dwdt})
and (\ref{eq:firstderivative}) and obtain different local solving
methods used to find the nearest local optimal solution with
guaranteed convergence. For example, if $R({\scriptstyle W})=I$,
then it is a naive error back-propagation algorithm. If
$R({\scriptstyle W})=[J({\scriptstyle W})^T J({\scriptstyle W})]$
then it is the Gauss-Newton method and if $R({\scriptstyle
W})=[J({\scriptstyle W})^T J({\scriptstyle W})+\mu
I]$ then it is the Levenberg-Marquardt method.\\

\subsubsection{Algorithm} \label{sec:algorithm} The proposed algorithm uses a promising starting point ($A^*$) as input and outputs the best local minimum of the neighborhood in the weight space.

%Figure \ref{fig:flowchart} shows the flowchart of our approach.
%
%
%
%\begin{figure}[htp]
%\centerline{
%  \epsfig{figure=Figures/flowchart.ps, width=3.0in}
%} \caption{Flow chart of our method} \label{fig:flowchart}
%\end{figure}
\textbf{Input:} Initial guess($A^*$), Tolerance ($\tau$), Step size
($s$)
\\\textbf{Output:} Best neighborhood local minimum ($A_{ij}$)
\\\textbf{Algorithm:}\\
{\it Step 1: Obtaining good initial guess ($A^*$):} The initial
guess for the algorithm can be obtained from other global search
methods or from a purely random start. Some domain knowledge about
the specific dataset that is being trained on, might help in
eliminating non-promising set of initial weights.
\\{\it Step 2: Moving to the local minimum ($m_i$):}
Using an appropriate local solver, the local optimum $m_i$ is
obtained using the $A^*$ as initial guess. The starting point will
be $x_i$ for the later stages.\\{\it Step 3: Determining the search
direction ($d_j$):} The eigenvectors $d_i$ of the Jacobian are
computed at $m_i$. These eigenvector directions might lead to
promising regions of the subspace. Other search directions can also be chosen based on the specific problem that is being dealt. \\
{\it Step 4: Escaping from the local minimum: } Taking small step
sizes away from $m_i$ along $d_i$ directions increases the objective
function value till it hits the stability boundary. However, the
objective function value then decreases after the search trajectory
passes the exit point on the stability boundary. $x_i$ is used as
initial guess and local solver is applied again (go to Step 2).
\\ {\it Step 5: Finding Tier-1 local minima ($A_{1i}$):} Exploring the neighborhood of the optimum solution local to
the initial guess leads to tier 1 local optima. Exploring from tier
$k$ local optima leads to tier $k+1$ local optima. \\
{\it Step 6: Exploring Tier-$k$ local minima ($A_{kj}$):} Explore
all other tiers in a similar manner described above. Selecting the
best solution from all these tiers, the global optimum of desired quality can be obtained.\\
{\it Step 7: Termination Criteria:} The procedure can be terminated
when the best solution obtained so far is satisfactory (lesser than
$sol_{req}$) or a predefined maximum number of tiers is explored.\\

\begin{figure}
\centerline{
  \epsfig{figure=Figures/dia.ps, width=3.2in}
} \caption{Illustration of Tier-2 TRUST-TECH procedure for obtaining
neighborhood local minima. } \label{fig:Diagram}
\end{figure}


Fig.~\ref{fig:Diagram} illustrates two tier TRUST-TECH methodology.
The `*' represents the initial guess. Dotted arrows represent the
convergence of the local solver. Solid arrows represent the gradient
ascent linear searches along eigenvector directions. `X' indicates a
new initial condition in the neighborhood stability region. $M$
represents the local minimum obtained by applying local methods from
'X'. $A_{1i}$ indicates Tier-1 local minima. $e_{1i}$ are the exit
points between $M$ and $A_{1i}$. Similarly, $A_{2j}$ and $e_{2j}$
are the second-tier local minima and their corresponding exit points
respectively.

%The following issues are discussed in detail : (i) Architecture and
%local methods, (ii) Initialization Schemes and (iii) TRUST-TECH.
\subsection {Implementation Details}
\label{sec:implementation} All programs were implemented in MATLAB
v6.5 and run on Pentium IV 2.8 GHz machines. We will now describe
some implementation issues of our algorithm.

\subsubsection{Network Architecture and Training}
As described in the introduction section, we have chosen to
demonstrate the capability of our newly proposed algorithm on a
network with single hidden layer and an output layer with only one
output node. This architecture is not complicated and has the
capability to precisely demonstrate the problems with the existing
approaches. Each hidden node has a tangent-sigmoid transfer function
and the output node has a pure linear transfer function. The number
of nodes in the hidden layer is determined by increasing number of
nodes, and selecting the number of nodes that achieves a compromise
between minimal error value and minimal number of nodes. The trust
region based Levenberg-Marquardt algorithm is chosen because of
efficiency in terms of time complexity and space requirements. It
utilizes the approximation of the Jacobian in its iterative gradient
descent, which will be used for generating promising directions in
TRUST-TECH. Two different initialization schemes were implemented.
The most basic global method which is multiple random starts with
initial set of parameters between -1 and 1. More effective global
method namely Nguyen-Widrow (NW) algorithm \cite{Nguyen90} has also
been used to test the performance of our algorithm. The NW algorithm
is implemented as the standard initialization procedure in MATLAB.
In both cases, the best initial set of parameters in terms of
training error is chosen and improved with our TRUST-TECH algorithm.

%\subsection{Initialization Schemes}

\subsubsection{TRUST-TECH}
\begin{algorithm}
\caption{$TRUST\_TECH$($NET, Wts,ss,\tau$)} \label{trustech}
\begin{algorithmic}
\STATE $Wts=Train(NET,Wts,\tau)$ \STATE$Error=Estimate(NET, Wts)$

    \STATE $Thresh=c*Error$
\STATE$Wts1[~]=Neighbors(NET,Wts,ss,\tau)$ \FOR{$k=1$ to
$size(Wts1)$}

\IF{$Estimate(NET,Wts1[k])<Thresh$} \STATE
$Wts2[k][~]=Neighbors(NET,Wts1,ss,\tau)$ \ENDIF

\ENDFOR \STATE \bf Return $best(Wts,Wts1,Wts2)$
\end{algorithmic}
\end{algorithm}
It is effective to use TRUST-TECH methodology for those promising
solutions obtained from stochastic global methods. Hence, our
algorithm assumes that it is being invoked from a promising set of
initial parameters. Algorithm \ref{trustech} describes the two-tier
TRUST-TECH algorithm. $NET$ assumes to have a fixed architecture
with a single output node. $ss$ is the step size required for moving
out of the stability region to obtain the exit point. $\tau$ is the
tolerance of error used for the convergence of the local method.
$Weights$ give the initial set of weight parameter values. $Train$
function implements the Levenberg-Marquardt method that obtains the
local optimal solution from the initial condition. The procedure
$Estimate$ computes the mean square error (MSE) value of the network
model. A threshold value ($Thresh$) is set based on this MSE value.
The procedure $Neighbors$ returns all the next tier local optimal
solutions from a given local solution. After obtaining all the
tier-1 solutions, Neighbors is again invoked (only for promising
solutions) to obtain the second-tier solutions. The algorithm
finally compares the initial solution, tier-1 and tier-2 solutions
and returns the network corresponding to the lowest error among all
these solutions.
\begin{algorithm}
\caption{$Wts[~]$  $Neighbors~$($NET, Wts$,~$ss$,~$\tau$)}
\label{Neighbors}
\begin{algorithmic}

    \STATE $[Wts,Hess]=Train(NET,Wts,\tau)$
\STATE $evec=Eig\_Vec (Hess)$ \STATE $Wts[~]=NULL$

\FOR{$k=1$ to $size(evec)$} \STATE $Old\_Wts= Wts$ \STATE $
ext\_Pt=Find\_Ext(NET,Old\_Wts,ss,evec[k])$

\IF{$(ext\_Pt)$} \STATE $New\_Wts=Move(NET,Old\_Wts,evec[k])$

    \STATE $New\_Wts=Train(NET,New\_Wts,\tau)$
    \STATE $Errors=Estimate(NET,New\_Wts)$
\STATE $Wts[~]=Append(Wts[~],New\_Wts,Errors)$

\ENDIF \ENDFOR \STATE \bf Return $Wts[~]$
\end{algorithmic}
\end{algorithm}

The approximate Hessian matrix used for updation in the
Levenberg-Marquardt method is utilized to obtain the search
direction. Since there is no optimal way of obtaining promising
search directions, the Eigen vectors of this Hessian matrix are used
as search directions. Along each search direction, the exit point is
obtained by evaluating the function value along that particular
direction. The step size for evaluation is chosen to be the average
step size taken during the convergence of the local procedure. The
function value increases initially and then starts to reduce
indicating the presence of exit point on the stability boundary.
$Move$ function ensures that a new point (obtained from the exit
point) is located in a different (neighboring) stability region.
From this new initial guess, the local method is applied again to
obtain the local optimal solution of the neighborhood stability
region. The search for exit points along these directions will be
stopped if exit points are not found after certain number of
function evaluations.

\begin{table}[htp]
\begin{small}
\centering \caption{\protect\small Summary of Benchmark Datasets.
Dataset (D), Sample size (Q), Input features (n), Output classes
(p), No. of Hidden nodes (k), No. of search variables ((n+2)k+1)}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
%&   Sample &Input &   Output & Hidden&
%Search \\
%Dataset &   Size &Features &   Classes& Nodes&
%Variables \\
  D&Q &  n &   p & k&
(n+2)k+1\\
\hline

\hline Cancer & 683&9 &  2&    5 &  56 \\\hline Diabetes & 178&  8&
3 & 4& 61\\ \hline Image& 2310&19& 7 &   8 &169 \\ \hline
Ionosphere& 351&34 & 2& 9& 325 \\ \hline Iris  &150& 4 &  3&  3& 19 \\ \hline Sonar & 208& 60& 2&  8  & 497 \\
\hline Wine & 178& 13&  3 &   4& 61\\  \hline
\end{tabular}
\end{center}
\end{small}
\label{TB:data1}
\end{table}

\begin{table*}[htp]
\begin{tiny}
\centering \caption{\protect\small Percentage improvements in the
classification accuracies over the training and test data using
TRUST-TECH with multiple random restarts. }
\begin{center}

\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 &\multicolumn{3}{c|}{Train Error}&\multicolumn{3}{c|}{Test Error}\\
\cline{2-7}
Dataset &MRS+BP&TRUST-TECH&Improvement&MRS+BP&TRUST-TECH&Improvement\\
\hline\hline

Cancer & 2.21  &  1.74   & 27.01 &  3.95   & 2.63 &   50.19 \\
\hline Image &9.37 &8.04  &  16.54  & 11.08  & 9.74  &  13.76 \\
\hline Ionosphere &2.35 &0.57 &312.28 & 10.25 &  7.96 &   28.77 \\
\hline Iris &1.25 &1.00 &25.00 &3.33 &2.67 &24.72 \\ \hline Diabetes
& 22.04 &20.69 &6.52 &23.83 &20.58& 15.79 \\ \hline Sonar& 1.56&
0.72 &116.67& 19.17 &12.98& 47.69 \\ \hline Wine &4.56& 3.58& 27.37&
14.94 &6.73 &121.99 \\ \hline



\end{tabular}
\end{center}
\end{tiny}
\label{TB:results}\end{table*}


\begin{table*}[htp]
\begin{tiny}
\centering \caption{\protect\small Percentage improvements in the
classification accuracies over the training and test data using
TRUST-TECH with MATLAB initialization. }
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
 &\multicolumn{3}{c|}{Train Error}&\multicolumn{3}{c|}{Test Error}\\
\cline{2-7}
Dataset &NW+BP&TRUST-TECH&Improvement&NW+BP&TRUST-TECH&Improvement\\
\hline\hline

Cancer & 2.25  &  1.57 &42.99& 3.65 &   3.06 &   19.06 \\
\hline  Image  & 7.48  &  5.17  &  44.82 &  9.39  &  7.40   & 26.90\\
\hline Ionosphere & 1.56 &0.92 &   69.57 &  8.67   & 6.54  &  32.57\\
\hline Iris &1.33   & 0.67   & 100.00 & 3.33 &   2.67  &  25.00  \\
\hline Diabetes & 21.41 &19.55 &9.53 &23.70 &21.09& 12.37 \\ \hline
Sonar& 2.35 &0.42 &456.96 & 17.26 &  14.38  & 20.03 \\ \hline  Wine
& 7.60 &1.62 &370.06 & 14.54 &4.48 &224.82 \\ \hline



\end{tabular}
\end{center}
\end{tiny}
\label{TB:results1}\end{table*}



\begin{figure*}[htp]
   \centering
   \subfigure[Wine Dataset]{\includegraphics[width = 2.45 in]{Figures/wine.ps}}
   \subfigure[Diabetes Dataset]{\includegraphics[width = 2.45 in]{Figures/pima.ps}}
   \subfigure[Cancer Dataset]{\includegraphics[width = 2.45 in]{Figures/cancer.ps}}
   \subfigure[Image Dataset]{\includegraphics[width = 2.45  in]{Figures/image.ps}}

   \caption{\label{fig:spider} Spider web diagrams showing the tier-1
and tier-2 improvements using TRUST-TECH
   method on various benchmark datasets. }
 \end{figure*}
\subsection{Experimental Results}
\label{sec:results}
%\subsection{Benchmark Datasets}
Our algorithm is evaluated using seven benchmark datasets in the UCI
machine learning repository \cite{Blake98}. Optimal architectures
have been fixed for the networks based on some heuristic training.
The main focus of our algorithm is to demonstrate the capability of
obtaining optimal weight parameters and improvements in the
generalization ability of the networks. Table~\ref{TB:data1}
summarizes the datasets. It gives the number of samples, input
features, output classes along with the number of hidden nodes of
the optimal architecture. These datasets have varying degrees of
complexity in terms of sample size, output classes and the class
overlaps. To demonstrate the generalization capability (and hence
the robustness) of the training algorithm, 10-fold cross validation
is performed on each dataset. The criteria of evaluation is given by
the classification accuracy of the network model in terms of the
percentage of misclassified samples in the test cases. Tables
~\ref{TB:results} and ~\ref{TB:results1} shows the improvements in
the train error and the test error using TRUST-TECH methodology when
multiple random starts (MRS) and matlab initialization is used. Five
tier-1 and corresponding tier-2 solutions were obtained using the
TRUST-TECH strategy. For some of the datasets, there had been
considerable improvements in the classifier performance. Spiderweb
diagram shown in Fig. \ref{fig:spider} a pretentious way to
demonstrate the improvements in a tier-by-tier manner.

Fig.\ref{fig:spider} shows spider web diagrams showing the tier-1
and tier-2 improvements using TRUST-TECH method on various benchmark datasets. The circle in the middle of the plot
represents the starting local optimal solution. The basic two
dimensions are chosen arbitrarily for effective visualization and
the vertical axis represents the percentage improvement in the
classification accuracy. The two basic axes are chosen arbitrarily
and the vertical axis represents the improvements in the classifier accuracy. The distances between each tier are normalized to unity and the improvements are averaged out across 10 folds. The five blue vertical lines surrounding the center circle are the best five local minima
obtained from a tier 1 search across all folds. The five best
second-tier improvements are plotted using red lines. It should be
noted that the best first tier solution need not give the best
second tier solution. Also, the second tier solution is as good as
or better than the first tier solution.


%Essentially, each dataset is partitioned into ten folds of
%approximately equal size. Let these folds are denoted by
%$T_1,T_2,...T_{10}$. Each time, the test set will be $T_i$ in which
%the the target labels will be deleted. The validation set is $T_j$
%for $j=(i+1) ~mod~ 10$ which will be used for early stopping. The
%training set is obtained from all the rest of the folds. The final
%MSE is the average of all the the errors obtained across each of the
%ten folds.
%\subsection {Error Estimation}

%Usually, training error is much lower than the test error because
%the network is modeled according to the training data and this data
%will be accurately classified compared to the unseen (test) data. We
%obtain all the network parameters including the architecture and the
%set of weights based on the training data. Once the final model is
%fixed, the accuracy on the test data will provide an estimate of the
%generalization capability of the network models.

%\subsection{Classification Accuracy}


%\begin{table*}[htp]
%\centering \caption{\protect\small Improvements in the
%classification accuracies over the training and test data using
%TRUST-TECH. }
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline &   Input &   Output & Sample &Hidden&
%Search \\
%Dataset &   Features &   Classes& Size &Nodes&
%Variables \\ \hline Cancer & 9 &  2&   683& 5 &  56 \\
%\hline Image& 19& 7 &  2310& 8 &169 \\ \hline Ion& 34 & 2& 351& 9&
%325 \\ \hline Iris  & 4 &  3& 150& 3& 19 \\ \hline Sonar &  60& 2& 208& 8  & 497 \\
%\hline Wine &  13&  3 &  178& 4& 61\\ \hline
%
%\end{tabular}
%\end{center}
%\label{TB:data}
%\end{table*}


%\begin{table*}[htp]
%\centering \caption{\protect\small Description of Benchmark
%Datasets.  }
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline &   Input &   Output & Sample &Hidden&
%Search \\
%Dataset &   Features &   Classes& Size &Nodes&
%Variables \\ \hline Cancer & 9 &  2&   683& 5 &  56 \\
%\hline Image& 19& 7 &  2310& 8 &169 \\ \hline Ion& 34 & 2& 351& 9&
%325 \\ \hline Iris  & 4 &  3& 150& 3& 19 \\ \hline Sonar &  60& 2& 208& 8  & 497 \\
%\hline Wine &  13&  3 &  178& 4& 61\\ \hline
%
%\end{tabular}
%\end{center}
%\label{TB:data}
%\end{table*}


%\subsection{Visualization}

%
%\begin{figure}[htbp]
%\centering
%\begin{tabular}{cc}
%%\vspace{-0.5in}
%\epsfig{figure=Figures/wine.ps,width=0.9\columnwidth} &
%\epsfig{figure=Figures/pima.ps,width=0.9\columnwidth} \\
%(a) {\small Wine Dataset} & (b) {\small Diabetes Dataset} \\
%\epsfig{figure=Figures/cancer.ps,width=0.9\columnwidth} &
%\epsfig{figure=Figures/image.ps,width=0.9\columnwidth} \\
%(a) {\small Cancer Dataset} & (b) {\small Image Dataset} \\
%\end{tabular}
%\caption{\label{fig:spider} Spider web diagrams showing the tier-1
%and tier-2 improvements using TRUST-TECH
%   method on various benchmark datasets. The basis two axes are chosen arbitrarily and the
%   vertical axis represents the improvements in the classifier
%   accuracy. The distances between each tier are normalized to
%   unity.}
%\end{figure}


%\subsection{Conclusion}
%\label{sec:conclusion}

This method provides an optimal set of training parameters for a
neural network model thus allowing improved classification
accuracies. Because of its non-probabilistic nature, multiple runs
of our algorithm from any given initial guess will provide exactly
the same result. The proposed method also allows the user to have
the flexibility of choosing different global and local techniques
for training.
%\appendix
%\section*{APPENDIX-A: Description of Datasets} \label{sec:appendix-A}
%%\textbf{} \\
%\textbf {\it Cancer : }  Each instance has one of 2 possible
%classes: benign or malignant. A total of 683 cases are available in
%which 444 are benign and 239 are malignant. 9 attributes describing
%the tumor are used for classification.\\
%
%\textbf  {\it Diabetes :} The dataset gives information about the
%patients who have some signs of diabetes according to World Health
%Organization criteria. Each sample has 8 real valued attributes. A
%total of 768 samples with 500 negative cases and 268 positive cases
%are
%available.\\
%
%\textbf {\it Image : }This dataset contains images which were drawn
%randomly from a database of 7 outdoor images. The images were hand
%segmented to create a classification for every pixel. There are 19
%attributes that describe each instance (which is a 3x3 region) of a
%given image. A total of 2310 samples were considered. \\
%
%\textbf {\it Ionosphere : }This radar data was collected by a system
%consisting a phased array of 16 high-frequency antennas with total
%transmitted power on the order of 6.4 kilowatts. The targets were
%free electrons in the ionosphere. A total of 351 instances with 34
%attributes. The classification task here is to separate good
%radar signals from that of the bad ones.\\
%
%\textbf {\it Iris : }The data set contains 3 classes of 50 instances
%each, where each class refers to a type of iris plant. It is
%relatively simple dataset where one class is linearly separable from
%the other two, but the other two have significant overlap and are
%not linearly separable from each other. The four attributes
%considered for classification are sepal length, sepal width, petal
%length and petal width. All
%attributes are measured in centimeters. \\
%
%\textbf {\it Sonar : } This data set is used for the classification
%of sonar signals. The task is to discriminate between sonar signals
%bounced off a metal cylinder and those bounced off a roughly
%cylindrical rock. The dataset contains a total of 208 samples (111
%for mines and 97 for rocks). The data set contains signals obtained
%from a variety of different aspect angles, spanning 90 degrees for
%the cylinder and 180 degrees for the rock. Each pattern is a set of
%60 numbers in the range 0.0 to 1.0 that represents the energy within
%a particular frequency band, integrated over a certain period of
%time. \\
%
%\textbf {\it Wine : }These data are the results of a chemical
%analysis of wines derived from three different cultivars. The
%analysis determined the quantities of 13 constituents found in each
%of the three types of wines. A total of 178 samples with the
%following distribution (59,71,48).\\


==> orig/theory-global.tex <==

\section{Problem Formulation and Transformations} \label
{sec:overview} This section deals with the transformation of the
nonlinear function into a dynamical system. It also gives the
correspondence between all the critical points of a $n$-dimensional
nonlinear surface and that of its corresponding dynamical system.
The main purpose of this transformation is to get more information
about the topology of the nonlinear surface. The knowledge of
stability regions and stability boundaries that is available in the
dynamical system literature is one of the vital components of our
algorithm. Our method is based on some of the fundamental results on
stability regions of nonlinear dynamical systems
\cite{Chiang96a,Reddy07c}. Here, we will describe all the necessary
components required to understand our algorithm and make this paper
self-contained.

\subsection{Mathematical Preliminaries} \label{sec:math} Let us consider an
unconstrained search problem on an energy surface defined by the
objective function
\begin{equation}
 f(x)\label{eq:problem}
\end{equation}
where $f(x)$ is assumed to be in $C^2(\Re^n,\Re)$.
\begin{lem}\label{def:criticalpoint}
$\bar{x}$ is said to be a {\it critical point} of (\ref{eq:problem})
if it satisfies the following condition
\begin{equation}
 \nabla f(x)=0\label{eq:criticalpoint}
\end{equation}
\end{lem}

Now, we will define {\it Saddle points} which are the vital elements
for understanding our methodology. The saddle points are critical
points whose gradient is zero and Hessian of the nonlinear function
has only one negative eigenvalue \cite{Reddy06}. Intuitively, this
means that a saddle point is a maximum along one direction but a
minimum along all other orthogonal directions. Mathematically, a
critical point is said to be {\it nondegenerate} if at the critical
point $\bar{x}\in \Re^n$, $d^T\nabla_{xx}^{2}f(\bar{x})d \not=
0$\hspace{0.05in} ($\forall d \not= 0$). Now, we construct the
following {\it negative gradient system} in order to locate critical
points of the objective function (\ref{eq:problem}):

\begin{equation}
 \frac{dx}{dt}=F(x)=-\nabla f(x)\label{eq:gradientsystem}
\end{equation}

where the state vector $x$ belongs to the Euclidean space $\Re^n$,
and the vector field $F : \Re^n \rightarrow \Re^n$ satisfies the
sufficient condition for the existence and uniqueness of the
solutions. The solution curve of Eq. (\ref{eq:gradientsystem})
starting from x at time $t=0$ is called a {\it trajectory} and it is
denoted by $\Phi(x,\cdot) : \Re \rightarrow \Re^n$. A state vector
$x$ is called an {\it equilibrium point} of Eq.
(\ref{eq:gradientsystem}) if $F(x)=0$.

\begin{lem}\label{def:stableequilibriumpoint}
An equilibrium point is said to be {\it hyperbolic} if the Jacobian
of $F$ at point $x$ has no eigenvalues with zero real part. A
hyperbolic equilibrium point is called a (asymptotically) {\it
stable equilibrium point} (SEP) if all the eigenvalues of its
corresponding Jacobian have negative real part. Conversely, it is an
{\it unstable equilibrium point} if some eigenvalues have a positive
real part.
\end{lem}

An equilibrium point is called a {\it type-k equilibrium point} if
its corresponding Jacobian has exact $k$ eigenvalues with positive
real part. When $k=0$, the equilibrium point is (asymptotically)
stable and it is called a {\it sink} (or {\it attractor}). If $k=n$,
then the equilibrium point is called a {\it source} (or {\it
repeller}).

From the implementation point of view, it is not required to
construct this gradient system. However, to understand the details
of our method, it is necessary to obtain this gradient system. This
gradient system and the decomposition points on the practical
stability boundary of the stable equilibrium points will enable us
to define {\it Tier-1 stable equilibrium point}.

\begin{lem}\label{def:tier1}
For a given stable equilibrium point ($x_s$), a {\it Tier-1 stable
equilibrium point} is defined as a stable equilibrium point whose
stability boundary intersects with the stability boundary of $x_s$.
\end{lem}


A dynamical system is completely {\it stable} if every trajectory of
the system leads to one of its stable equilibrium points. The {\it
stable} ($W^s(\tilde{x})$) and {\it unstable} ($W^u(\tilde{x})$)
manifolds of an equilibrium point, say $\tilde{x}$, is defined as:
\begin{center}
\begin{eqnarray}
W^s(\tilde{x}) = \{ x \in \Re^n ~:~
\lim_{t\to\infty}\Phi(x,t)=\tilde{x}\} \\
W^u(\tilde{x}) = \{ x \in \Re^n ~:~
\lim_{t\to-\infty}\Phi(x,t)=\tilde{x}\} \label{eq:unstablemanifold}
\end{eqnarray}
\end{center}


The {\it stability region} (also called {\it region of attraction})
of a stable equilibrium point $x_s$ of a dynamical system
(\ref{eq:gradientsystem}) is denoted by $A(x_s)$ and is

\begin{equation}
A(x_s) = \{ x \in \Re^n ~:~ \lim_{t\to\infty}\Phi(x,t)=x_s\}
\label{eq:stabilityregion}
\end{equation}\vspace{0.05in}

The boundary of stability region is called the {\it stability
boundary} of $x_s$ and will be denoted by $\partial A(x_s)$. It has
been shown that the stability region is an open, invariant and
connected set. From the topological viewpoint, the stability
boundary is a ($n-1$) dimensional closed and invariant set.

The {\it practical stability region} of a stable equilibrium point
$x_s$ of a nonlinear dynamical system (\ref{eq:gradientsystem}),
denoted by $A_p(x_s)$ and is
\begin{equation}
A_p(x_s) =int~\overline{A(x_s)} \label{eq:stablemanifold}
\end{equation}
where $\bar{A}$ denotes the closure of A and $int~\bar{A}$ denotes
the interior of $\bar{A}$. $int~\overline{A(x_s)}$ is an open set.
The boundary of practical stability region is called the {\it
practical stability boundary} of $x_s$ and will be denoted by
$\partial A_p(x_s)$.

It has been shown that the practical stability boundary $\partial
A_p(x_s)$ is equal to $\partial \bar{A}(x_s)$ \cite{Chiang96}. The
practical stability boundary is a subset of its stability boundary.
It eliminates the complex portion of the stability boundary which
has no ``contact" with the complement of the closure of the
stability region. A complete characterization of the practical
stability boundary for a large class of nonlinear dynamical systems
can be found.

\begin{lem}\label{def:decompositionpoint}
A type-1 equilibrium point $x_d$ (k=1) on the practical stability
boundary of a stable equilibrium point $x_s$ is called a {\it
decomposition point}.
\end{lem}


The task of finding multiple local optimal solutions on the
nonlinear surface is transformed into the task of finding multiple
stable equilibrium points on its corresponding gradient system. The
advantage of our approach is that this transformation into the
corresponding dynamical system will yield more knowledge about the
various dynamic and geometric characteristics of the original
surface and leads to the development a powerful method for finding
improved solutions. In this paper, we are particularly interested in
the properties of the local optimal solutions and their one-to-one
correspondence to the stable equilibrium points.

\subsection{Theoretical Background}
\label{sec:theory}

To comprehend the transformation, we need to define {\it Lyapunov
function}. A smooth function $V(\cdot) : \Re^n \rightarrow \Re$
satisfying $\dot{V}(\Phi(x,t))~<~0~,~\forall ~x \notin $ \{set of
equilibrium points (E)\} and t $\in \Re^+ $ is termed as Lyapunov
function.

\begin{thm}\label{th:lyapunov}\cite{Chiang96}: $F(x)$ is a
Lyapunov function for the negative quasi-gradient system
(\ref{eq:gradientsystem}).
\end{thm}
%\begin{proof}
Let $\Phi(x,t)$ denote the bounded trajectory starting at $x$.
consider the time derivative $\frac{d}{dt} f(\Phi(x,t))$ along the
trajectory. It is clear that\\
$\frac{d}{dt} f(\Phi(x,t))=~-~(\nabla f(\Phi(x,t)))^T~(\nabla
f(\Phi(x,t)))~ \leq ~0$ \\
moreover, $\frac{d}{dt} f(\Phi(x,t))=0$ if, and only if, $x \in E$.
Therefore, $f(x)$ is an energy function of the negative
quasi-gradient system (\ref{eq:gradientsystem}). This completes the
proof.
%\end{proof}

%The stability region of a stable equilibrium point can be completely
%characterized for a fairly large class of nonlinear systems.
%Consider the gradient system described by (\ref {eq:gradientsystem})
%satisfying the following assumptions:
%\begin {itemize}
%{\item (A1) - The critical elements on the stability boundary are
%hyperbolic and finite in number.} {\item (A2) - The stable and
%unstable manifolds of the critical elements on the stability
%boundary satisfy the transversality condition.}
%
%{\item (A3) - Every trajectory on the stability boundary approaches
%one of the critical elements as $t\to\infty$.}
%
%\end{itemize}
%
%We present the conditions for an equilibrium point to be on the
%$\partial A(x_s)$. This is a key step in the complete
%characterization of $\partial A(x_s)$.

%\cite{Chiang88}
%
%\begin{thm}\label{th:cond} Let $A(x_s)$ be the stability region of nonlinear dynamical system (\ref
%{eq:gradientsystem}). Let $\sigma \neq x_s$ be a hyperbolic critical
%element of system (\ref {eq:gradientsystem}). If assumptions
%(A1)-(A3) are
%satisfied, then \\
%(1)  $\sigma\in\partial A$ if and only if $W^u(\sigma) \cap A(x_s) \neq  \emptyset $. \\
%(2)  $\sigma\in\partial A$ if and only if $W^s(\sigma) \subset \partial A(x_s)$. \\
%
%\end{thm}


%\cite{Chiang96a}

\begin{thm}\label{th:characterization}{\it (Characterization of stability
boundary)\cite{Chiang96a}:} Consider a nonlinear dynamical system
described by (\ref {eq:gradientsystem}). Let $\sigma_i$, i=1,2,...
be the equilibrium points on the stability boundary $\partial
A(x_s)$ of a stable equilibrium point, say $x_s$. Then
%\subseteq
\begin{equation}
\partial A(x_s) \subseteq \bigcup_{\sigma_i\in\partial A} W^s(\sigma_i).
\label{eq:charstabilityregion}
\end{equation}
\end{thm}
%satisfying assumption (A1)
Theorem \ref{th:characterization} completely characterizes the
stability boundary for nonlinear dynamical systems by asserting that
the stability boundary is the union of the stable manifolds of all
critical elements on the stability boundary. This theorem gives an
explicit description of the geometrical and dynamical structure of
the stability boundary. This theorem can be extended to the
characterization of the practical stability boundary in terms of the
stable manifold of the decomposition point.


\begin{thm}{\it (Characterization of practical stability
boundary):} Consider a nonlinear dynamical system described by (\ref
{eq:gradientsystem}). Let $\sigma_i$ , i=1,2,... be the dynamic
decomposition points on the practical stability boundary $\partial
A_p(x_s)$ of a stable equilibrium point, say $x_s$. Then

\begin{equation}
\partial A_p(x_s) \subseteq \bigcup_{\sigma_i\in\partial A_p} \overline{W^s(\sigma_i)}.
\label{eq:charpracstabilityregion}
\end{equation}
\label{th:characterization1}
\end{thm}


Theorem \ref{th:characterization1} asserts that the practical
stability boundary is contained in the union of the closure of the
stable manifolds of all the dynamic decomposition points on the
practical stability boundary. Hence, if the dynamic decomposition
points can be identified, then an explicit characterization of the
practical stability boundary can be established using
(\ref{eq:charpracstabilityregion}).

\begin{thm}\label{th:um}{\it (Unstable manifold of type-1 equilibrium
point)\cite{Lastras98}:} Let $x_s^1$ be a stable equilibrium point
of the gradient system (\ref{eq:gradientsystem}) and $x_d$ be a
type-1 equilibrium point on the practical stability boundary
$\partial A_p(x_s)$. Assume that there exist $\epsilon$ and $\delta$
such that $\| \nabla f(x) \| > \epsilon$ unless $x\in
B_\delta(\hat{x}), \hat{x} \in \{x: \nabla f(x)=0\}$. There exists
another stable equilibrium point $x_s^2$ to which the one
dimensional unstable manifold of $x_d$ converges. Conversely, if
$\overline{A_p(x_s^1)}\bigcap\overline{A_p(x_s^2)}\not=\emptyset$,
then there exists a dynamic decomposition point $x_d$ on $\partial
A_p(x_s^1)$.
\end{thm}


Theorem \ref{th:um} is imperative to understand some of the
underlying concepts behind the development of our method. It
associates the notion of stable equilibrium points, practical
stability regions ($A_p(x_s)$), practical stability boundaries
($\partial A_p(x_s)$) and type-1 equilibrium points. The unstable
manifold ($W^u$) of the dynamic decomposition point $x_d^1$
converges to the two stable equilibrium points $x_s^1$ and $x_s^2$.
Also, it should be noted that $x_d^1$ is present on the stability
boundary of $x_s^1$ and $x_s^2$.

We must show that under the transformation from (\ref{eq:problem})
to (\ref{eq:gradientsystem}), the properties of the critical points
remain unchanged. Theorem \ref{th:cpc} illustrates the
correspondence of the critical points of the original system.



\begin{thm}\label{th:cpc}{\it (Critical Points and their correspondence): }
An equilibrium point of (\ref{eq:gradientsystem}) is hyperbolic if,
and only if, the corresponding critical point is nondegenerate.
Moreover, if $\bar{x}$ is a hyperbolic equilibrium point of
(\ref{eq:gradientsystem}), then
\begin {enumerate}
\item {$\bar{x}$ is a stable equilibrium point of
(\ref{eq:gradientsystem}) if and only if $\bar{x}$ is an isolated
local minimum for (\ref{eq:problem})}

\item {$\bar{x}$ is a source of (\ref{eq:gradientsystem}) if and
only if $\bar{x}$ is an isolated local maximum for
(\ref{eq:problem})}

\item {$\bar{x}$ is a decomposition point of
(\ref{eq:gradientsystem}) if and only if $\bar{x}$ is a saddle point
for (\ref{eq:problem})}
\end {enumerate}
\end{thm}
%\begin{proof}
First part of the proof is published in \cite{Chiang96}. $f(x)$ is a
Lyapunov function \cite{Chiang88} for the negative gradient system
(\ref{eq:gradientsystem}). Hence, every trajectory within the
stability region $A(\bar{x})$ converges to $\bar{x}$ and the
function value $f(x)$ decreases along every nontrivial trajectory.
So, $\bar{x}$ is a stable equilibrium point of
(\ref{eq:gradientsystem}) if and only if, there exists a
neighborhood $N$ such that $f(x)$ reaches local minimum at
$x=\bar{x}$. In a similar manner, we can prove that $\bar{x}$ is a
source of (\ref{eq:gradientsystem}) if and only if $\bar{x}$ is an
isolated local maximum for (\ref{eq:problem}) by inverting the
dynamical system (to make the stable equilibrium point a source) and
the energy function (new energy function for the new dynamical
system).

To prove that $\bar{x}$ is a decomposition point of
(\ref{eq:gradientsystem}) if and only if $\bar{x}$ is a saddle point
for (\ref{eq:problem}), one has to consider the properties of the
second derivatives. Since, all the critical points of
(\ref{eq:problem}) and all the equilibrium points of
(\ref{eq:gradientsystem}) are the same and Hessian of the original
function $f(x)$ and the gradient of (\ref{eq:gradientsystem}) at
these points are the same, the corresponding eigen values and eigen
vectors of are equal. This concludes the proof.

%\end{proof}


\section{TRUST-TECH based Algorithm}
\begin{figure}
\centerline{
  \epsfig{figure=Figures/diagram3.ps, width=2.5in}
} \caption {Diagram illustrates the TRUST-TECH based method of
escaping from the original solution ($A$) to the neighborhood local
optimal solutions ($a_{1i}$) through the corresponding exit points
($e_{1i}$). The dotted lines indicate the local convergence of the
local solver.} \label{fig:diagram}
\end{figure}

Our approach takes advantage of TRUST-TECH (TRansformation Under
STability-reTaining Equilibria CHaracterization) to compute
neighborhood local optimal solutions on the surface using stability
regions. Originally, the basic idea of our algorithm was to find
decomposition points on the practical stability boundary. Since,
each decomposition point connects two local optima uniquely, it is
important to obtain the saddle points from the given solution and
then move to the next solution through this decomposition point. The
details of a stability boundary tracing algorithm to obtain
decomposition points on the stability boundary is presented in
\cite{Reddy06}. Though, this procedure gives a guarantee that the
local optimum is not revisited, the computational expense for
tracing the stability boundary and identifying the decomposition
point is high compared to the cost of applying the local solver
directly using the exit point without considering the decomposition
point. However, it is beneficial to use the saddle point tracing
procedure developed in \cite{Reddy06} for applications where the
local methods are relatively expensive. For most of the applications
that arise in machine learning domain, it is not necessary to obtain
the saddle point because of the fact that the local methods are
highly optimized for the specific problem in hand and in general,
these methods are much cheaper than tracing the boundary (which
often requires multiple gradient computations which might be
relatively expensive). This is just a implementation heuristic and
it depends on the practitioner where he wants to use the saddle
point method or the exit-point method. As shown in Fig.
\ref{fig:diagram}, from the original local optimal solution, various
exit points and their corresponding new local optimal solutions are
computed along each promising direction.

Our framework consists three stages namely: (i) global stage, (ii)
local stage and (iii) neighborhood-search stage. The last two stages
are repeated in the solution space to obtain promising solutions.
Global method obtains promising subspaces of the solution space. The
next stage is the local stage where the results from the global
methods are refined to the corresponding locally optimal parameter
set. Then, during the neighborhood search stage, the exit points are
computed and the neighborhood solutions are systematically explored
through these exit points. It is more effective to use our algorithm
at only these promising subspaces which are usually obtained by
stochastic global methods. This approach can be treated as a hybrid
between global methods for initialization and the local method. With
the saddle point method being approximated (to exit-pint method),
the various steps involved in our approach are clearly illustrated
in Algorithm~\ref{nexttieralg}.


\begin{algorithm}
\caption{TRUST-TECH based Algorithm} \label{nexttieralg}
\begin{algorithmic}
\STATE \textbf{Input:} Parameters $\Theta$, Data  $\mathcal{X}$,
tolerance $\tau$, Local Solver ($LS$)  \STATE \textbf{Output:}
$\widehat{\Theta}_{Max} $  \STATE \textbf{Algorithm:}

\STATE Apply global method and store the q promising solutions $
\Theta_{init}=\{\Theta_1,\Theta_2,..,\Theta_q\}$ ~~~~~~~~ Initialize
E= $\phi$

\WHILE{$\Theta_{init} \neq \phi$} \STATE Choose $\Theta_i \in
\Theta_{init}$, set $\Theta_{init}= \Theta_{init} \backslash
\{\Theta_i\}$ \STATE $LM_i=LS(\Theta_i,\mathcal{X},\tau)$~~~~~~~~~
$E=E \cup \{LM_i\}$ \STATE Generate promising direction vectors
$d_j$ from $LM_i$

\FOR {each $d_j$} \STATE Compute Exit Point ($X_j$) along $d_j$
starting from $LM_i$ by evaluating the nonlinear function

\STATE $New_j=LS(X_j+\epsilon \cdot d_j,\mathcal{X},\tau)$
\IF{$new_j \notin E$} \STATE $E=E \cup New_j$ \ENDIF

\ENDFOR
\ENDWHILE \STATE $\widehat{\Theta}_{Max} =max\{val(E_i)\}$

\end{algorithmic}
\end{algorithm}


In order to escape out of a found local optimum, our method needs to
compute certain promising directions based on the local behaviour of
the function. One can realize that generating these promising
directions is one of the important aspects of our algorithm.
Surprisingly, choosing random directions to move out of the local
optimum works well for this problem. One might also use other
directions like eigenvectors of the Hessian or incorporate some
domain-specific knowledge (like information about priors,
approximate location of cluster means, user preferences on the final
clusters) depending on the application that they are working on and
the level of computational expense that they can afford. We used
random directions in our work because they are very cheap to
compute. Once the promising directions are generated, exit points
are computed along these directions. {\it Exit points} are points of
intersection between any given direction and the practical stability
boundary of that local optimum along that particular direction. If
the stability boundary is not encountered along a given direction,
then there is a guarantee that one will not be able to find any new
local optimum in that direction. With a new initial guess in the
vicinity of the exit points, local method is applied again to obtain
a new local optimum. Sometimes, this new point ($X_j+\epsilon \cdot
d_j$) might have convergence problems. In such cases, TRUST-TECH can
also help the convergence by integrating the dynamical system and
obtaining another point that is much closer to the local optimal
solution.


==> orig/theory.tex <==
\section{Problem Formulation and Transformations} \label
{sec:overview}

Now, we will introduce some of the terminology that is required to understand
the theoretical insights of our approach. Most importantly, this section deals with the
transformation of the nonlinear function into a dynamical system. It also gives the correspondence between all the
critical points of a $n$-dimensional nonlinear surface and that
of its corresponding dynamical system. Our method is based on some of the
fundamental results on stability regions of nonlinear dynamical
systems \cite{Chiang88,Chiang96a,Lee04}.

\subsection{Mathematical Preliminaries} \label{sec:math} Before
presenting the details of our method, we review some fundamental
concepts of nonlinear dynamical systems. Let us consider an
unconstrained search problem on an energy surface defined by the
objective function

\begin{equation}
 f(x)\label{eq:problem}
\end{equation}

where $f(x)$ is assumed to be in $C^2(\Re^n,\Re)$.




\begin{lem}\label{def:criticalpoint}
$\bar{x}$ is said to be a {\it critical point} of (\ref{eq:problem})
if it satisfies the following condition
\begin{equation}
 \nabla f(x)=0\label{eq:criticalpoint}
\end{equation}
\end{lem}


\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/figure1a.ps, width=3.5in}
} \caption{The surface and contour plots of a two-dimensional energy
function.A saddle point ($x_d$) is located between two local minima
($x_s^1$ and $x_s^2$). $x_m^1$ and $x_m^2$ are two local minima
located in the orthogonal direction.} \label{fig:saddlepoint}
\end{figure}
Now, we will define {\it Saddle points} which are the vital elements for understanding our methodology. The saddle points are critical points whose gradient is zero and Hessian of
the nonlinear function has only one negative eigenvalue \cite
{Heidrich91}. Intuitively, this means that a saddle point is a
maximum along one direction but a minimum along all other orthogonal
directions \cite{Reddy06}. Fig. 1 shows a saddle point ($x_d$) located between two
local minima ($x_s^1$ and $x_s^2$) and two local maxima ($x_m^1$ and
$x_m^2$). As shown in the figure, the saddle point is a maximum
along the direction of the vector joining the two local minima and a
minimum along its orthogonal direction (or the direction of the
vector joining the two local maxima). The direction in which the
saddle point is the maximum is usually unknown in most of the
practical problems and is the direction of interest.



A critical point is said to be {\it nondegenerate} if at the
critical point $\bar{x}\in \Re^n$, $d^T\nabla_{xx}^{2}f(\bar{x})d
\not= 0$\hspace{0.05in} ($\forall d \not= 0$). Now, we construct the following {\it negative gradient system} in order
to locate critical points of the objective function
(\ref{eq:problem}):

%\begin{equation}
%\dot{x}(t) = f(x(t))\label{eq:nonlineardynamicalsystems}
%\end{equation}

\begin{equation}
 \frac{dx}{dt}=-\nabla f(x)\label{eq:gradientsystem}
\end{equation}

where the state vector $x$ belongs to the Euclidean space $\Re^n$,
and the vector field $f : \Re^n \rightarrow \Re^n$ satisfies the
sufficient condition for the existence and uniqueness of the
solutions. The solution curve of Eq. (\ref{eq:gradientsystem})
starting from x at time $t=0$ is called a {\it trajectory} and it is
denoted by $\Phi(x,\cdot) : \Re \rightarrow \Re^n$. A state vector
$x$ is called an {\it equilibrium point} of Eq.
(\ref{eq:gradientsystem}) if $f(x)=0$.

\begin{lem}\label{def:stableequilibriumpoint}
An equilibrium point is said to be {\it hyperbolic} if the Jacobian
of $f$ at point $x$ has no eigenvalues with zero real part. A
hyperbolic equilibrium point is called a (asymptotically) {\it
stable equilibrium point} (SEP) if all the eigenvalues of its
corresponding Jacobian have negative real part. Conversely, it is an
{\it unstable equilibrium point} if some eigenvalues have a positive
real part.

\end{lem}


An equilibrium point is called a {\it type-k equilibrium point} if
its corresponding Jacobian has exact $k$ eigenvalues with positive
real part. When $k=0$, the equilibrium point is (asymptotically)
stable and it is called a {\it sink} (or {\it attractor}). If $k=n$,
then the equilibrium point is called a {\it source} (or {\it
repeller}).
%
A dynamical system is completely {\it stable} if every trajectory of
the system leads to one of its stable equilibrium points. The {\it
stable} ($W^s(\tilde{x})$) and {\it unstable} ($W^u(\tilde{x})$)
manifolds of an equilibrium point, say $\tilde{x}$, is defined as:
\begin{center}
\begin{eqnarray}
W^s(\tilde{x}) = \{ x \in \Re^n ~:~
\lim_{t\to\infty}\Phi(x,t)=\tilde{x}\} \\
W^u(\tilde{x}) = \{ x \in \Re^n ~:~
\lim_{t\to-\infty}\Phi(x,t)=\tilde{x}\} \label{eq:unstablemanifold}
\end{eqnarray}
\end{center}

The stable and unstable manifolds of an equilibrium point are said
to satisfy the {\it transversality} condition if either they do not
intersect at all, or at every intersection point $x_0$ between these
two manifolds, the tangent spaces of $W^s(x_0)$ and $W^u(x_0)$ span
$\Re^n$. This is shown in Eq. (\ref{eq:transversality})

\begin{equation}
T(W^s(x_0)) \oplus T(W^u(x_0))=\Re^n \label{eq:transversality}
\end{equation}
\begin{lem}\label{def:stabilityregion} The {\it stability region} (also called {\it region of
attraction}) of a stable equilibrium point $x_s$ of a dynamical
system (\ref{eq:gradientsystem}) is denoted by $A(X_s)$ and is

\begin{equation}
A(x_s) = \{ x \in \Re^n ~:~ \lim_{t\to\infty}\Phi(x,t)=x_s\}
\label{eq:stabilityregion}
\end{equation}\vspace{0.05in}
\end{lem}

The boundary of stability region is called the {\it stability
boundary} of $x_s$ and will be denoted by $\partial A(x_s)$. It has
been shown that the stability region is an open, invariant and
connected set \cite{Chiang88}. From the topological viewpoint, the
stability boundary is a (n-1) dimensional closed and invariant set.
A new concept related to the stability regions namely the {\it
quasi-stability region} (or {\it practical stability
region}), was developed in \cite{Chiang96a}.\\

\begin{lem}\label{def:practicalstabilityregion} The {\it practical stability
region} of a stable equilibrium point $x_s$ of a nonlinear dynamical
system (\ref{eq:gradientsystem}), denoted by $A_p(x_s)$ and is

\begin{equation}
A_p(x_s) =int~\overline{A(x_s)} \label{eq:stablemanifold}
\end{equation}


where $\bar{A}$ denotes the closure of A and $int~\bar{A}$ denotes
the interior of $\bar{A}$. $int~\overline{A(x_s)}$ is an open set.
The boundary of practical stability region is called the {\it
practical stability boundary} of $x_s$ and will be denoted by
$\partial A_p(x_s)$.
\end {lem}
\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/figure1b.ps, width=3.5in}
} \caption{Phase potrait of the gradient system corresponding to
Fig. \ref{fig:saddlepoint}. The solid lines represent the basin
boundary which shows that $\partial A_p(x_s^1) = \bigcup_{i=1}^{3}
\overline{W^s(x_d^i)}$. The local minima $x_s^1$ and $x_s^2$
correspond to the stable equilibrium points of the gradient system.
The saddle point ($x_d^1$) corresponds to the decomposition point of
the gradient system.}\label{fig:saddlepoint1}
\end{figure}

It has been shown that the practical stability boundary $\partial
A_p(x_s)$ is equal to $\partial \bar{A}(x_s)$. The practical
stability boundary is a subset of its stability boundary. It
eliminates the complex portion of the stability boundary which has
no ``contact" with the complement of the closure of the stability
region. A complete characterization of the practical stability
boundary for a large class of nonlinear dynamical systems can be
found in \cite{Chiang88}.

\begin{lem}\label{def:decompositionpoint}
A type-1 equilibrium point $x_d$ (k=1) on the practical stability
boundary of a stable equilibrium point $x_s$ is called a {\it
decomposition point}.
\end{lem}


The task of finding multiple local maxima on the log-likelihood
surface is transformed into the task of finding multiple stable
equilibrium points on its corresponding gradient system. The
advantage of our approach is that this transformation into the
corresponding dynamical system will yield more knowledge about the
various dynamic and geometric characteristics of the original
surface and leads to the development a powerful method for finding
improved solutions. In this paper, we are particularly interested in
the properties of the local optimal solutions and their one-to-one
correspondence to the stable equilibrium points.

\subsection{Theoretical Background}
\label{sec:theory}

To comprehend the transformation, we need to define {\it energy
function}. A smooth function $V(\cdot) : \Re^n \rightarrow \Re^n$
satisfying $\dot{V}(\Phi(x,t))~<~0~,~\forall ~x \notin $ \{set of
equilibrium points (E)\} and t $\in \Re^+ $ is termed as energy
function.

\begin{thm}\label{th:lyapunov}\cite{Chiang96}: $f(x)$ is a
lyapunov function for the negative quasi-gradient system
(\ref{eq:gradientsystem}).
\end{thm}


The stability region of a stable equilibrium point can be completely
characterized for a fairly large class of nonlinear systems.
%Consider the gradient system described by (\ref {eq:gradientsystem})
%satisfying the following assumptions:
%\begin {itemize}
%{\item (A1) - The critical elements on the stability boundary are
%hyperbolic and finite in number.} {\item (A2) - The stable and
%unstable manifolds of the critical elements on the stability
%boundary satisfy the transversality condition.}
%
%{\item (A3) - Every trajectory on the stability boundary approaches
%one of the critical elements as $t\to\infty$.}
%
%\end{itemize}
%
%We present the conditions for an equilibrium point to be on the
%$\partial A(x_s)$. This is a key step in the complete
%characterization of $\partial A(x_s)$.

%\cite{Chiang88}
%
%\begin{thm}\label{th:cond} Let $A(x_s)$ be the stability region of nonlinear dynamical system (\ref
%{eq:gradientsystem}). Let $\sigma \neq x_s$ be a hyperbolic critical
%element of system (\ref {eq:gradientsystem}). If assumptions
%(A1)-(A3) are
%satisfied, then \\
%(1)  $\sigma\in\partial A$ if and only if $W^u(\sigma) \cap A(x_s) \neq  \emptyset $. \\
%(2)  $\sigma\in\partial A$ if and only if $W^s(\sigma) \subset \partial A(x_s)$. \\
%
%\end{thm}


%\cite{Chiang96a}

\begin{thm}\label{th:characterization}{\it (Characterization of stability
boundary):} Consider a nonlinear dynamical system
described by (\ref {eq:gradientsystem}) which satisfy assumptions
(A1)-(A3). Let $\sigma_i$, i=1,2,... be the equilibrium points on
the stability boundary $\partial A(x_s)$ of a stable equilibrium
point, say $x_s$. Then

\begin{equation}
\partial A(x_s) = \bigcup_{\sigma_i\in\partial A} W^s(\sigma_i).
\label{eq:charstabilityregion}
\end{equation}
\end{thm}

Theorem \ref{th:characterization} completely characterizes the
stability boundary for nonlinear dynamical systems satisfying
assumptions (A1)-(A3) by asserting that the stability boundary is
the union of the stable manifolds of all critical elements on the
stability boundary. This theorem gives an explicit description of
the geometrical and dynamical structure of the stability boundary.
This theorem can be extended to the characterization of the
practical stability boundary in terms of the stable manifold of the
decomposition point.

\begin{thm}{\it (Characterization of practical stability
boundary)\cite{Chiang96a}:} Consider a nonlinear dynamical system
described by (\ref {eq:gradientsystem}) which satisfy assumptions
(A1)-(A3). Let $\sigma_i$ , i=1,2,... be the decomposition points on
the practical stability boundary $\partial A_p(x_s)$ of a stable
equilibrium point, say $x_s$. Then

\begin{equation}
\partial A_p(x_s) = \bigcup_{\sigma_i\in\partial A_p} \overline{W^s(\sigma_i)}.
\label{eq:charpracstabilityregion}
\end{equation}
\label{th:characterization1}
\end{thm}


Theorem \ref{th:characterization1} asserts that the practical
stability boundary is contained in the union of the closure of the
stable manifolds of all the decomposition points on the practical
stability boundary. Hence, if the decomposition points can be
identified, then an explicit characterization of the practical
stability boundary can be established using
(\ref{eq:charpracstabilityregion}).

\begin{thm}\label{th:um}{\it (Unstable manifold of type-1 equilibrium
point)\cite{Lastras98}:} Let $x_s^1$ be a stable equilibrium point
of the gradient system (\ref{eq:gradientsystem}) and $x_d$ be a
type-1 equilibrium point on the practical stability boundary
$\partial A_p(x_s)$. Assume that there exist $\epsilon$ and $\delta$
such that $\| \nabla f(x) \| > \epsilon$ unless $x\in
B_\delta(\hat{x}), \hat{x} \in \{x: \nabla f(x)=0\}$. If assumptions
(A1)-(A3) are satisfied, then there exists another stable
equilibrium point $x_s^2$ to which the one dimensional unstable
manifold of $x_d$ converges. Conversely, if
$\overline{A_p(x_s^1)}\bigcap\overline{A_p(x_s^2)}\not=\emptyset$,
then there exists a decomposition point $x_d$ on $\partial
A_p(x_s^1)$.
\end{thm}

Theorem \ref{th:um} is imperative to understand some of the
underlying concepts behind the development of our method. It
associates the notion of stable equilibrium points, practical
stability regions ($A_p(x_s)$), practical stability boundaries
($\partial A_p(x_s)$) and type-1 equilibrium points. As shown in
fig.~\ref {fig:saddlepoint1}, The unstable manifold ($W^u$) of the
decomposition point $x_d^1$ converges to the two stable equilibrium
points $x_s^1$ and $x_s^2$. Also, it should be noted that $x_d^1$ is
present on the stability boundary of $x_s^1$ and $x_s^2$.

We also need to show that under the transformation from
(\ref{eq:problem}) to (\ref{eq:gradientsystem}), the properties of
the critical points remain unchanged. Theorem \ref{th:cpc}
illustrates the correspondence of the critical points of the
original system.

\begin{thm}\label{th:cpc}{\it (Critical Points and their correspondence): }
An equilibrium point of (\ref{eq:gradientsystem}) is hyperbolic if,
and only if, the corresponding critical point $f$ is nondegenerate.
Moreover, if $\bar{x}$ is a hyperbolic equilibrium point of
(\ref{eq:gradientsystem}), then
\begin {enumerate}
\item {$\bar{x}$ is a stable equilibrium point of
(\ref{eq:gradientsystem}) if and only if $\bar{x}$ is an isolated
local minimum for (\ref{eq:problem})}

\item {$\bar{x}$ is a source of (\ref{eq:gradientsystem}) if and
only if $\bar{x}$ is an isolated local maximum for
(\ref{eq:problem})}

\item {$\bar{x}$ is a decomposition point of
(\ref{eq:gradientsystem}) if and only if $\bar{x}$ is a saddle point
for (\ref{eq:problem})}
\end {enumerate}
\end{thm}


%\subsection{A Stability Boundary based Method}
%\label{sec:algorithm} Our method uses the theoretical
%concepts of dynamical systems presented in the previous section. The
%method described in this section finds the decomposition point when
%the two neighborhood local minima are given. Our method is
%illustrated on a two-dimensional LEPS potential energy surface
%\cite{Polanyi69}. The equations corresponding to the LEPS potential
%are given in the appendix. The two local minima are $A$ and
%$B$ and the decomposition point is $DP$.\\
%\\{\bf Given :} Two neighborhood local minima (A,B) \\
%{\bf Goal :} To obtain the corresponding decomposition point (DP)\\
%
%Step1: {\it Initializing the Search direction} : Since the location
%of the neighborhood local minima is already given, the initial
%search direction becomes explicit. The vector that joins
%the two given local minima ($A$ and $B$) is chosen to be the initial search direction. \\
%
%Step 2: {\it Locating the exit point ($X_{ex}$)} : (see fig.
%\ref{fig:myleps2}) Along the direction $AB$, starting from $A$, the
%function value is evaluated at different step intervals. Since the
%vector is between two neighborhood local minima, the function value
%will monotonically increase and decrease till it reaches the other
%local minimum ($B$). The
%point where the energy value attains its peak is called the {\it exit point}.\\
%
%
%
%\begin{figure}[htp]
%\centerline{ \epsfig{figure=Figures/myleps2.ps, width=3.5in}
%}\caption {Contour plot of a 2-D LEPS potential (described in
%appendix-A). Each line represents the values of a constant
%potential. $A$ and $B$ are the two local minima. $DP$ is the
%decomposition point to be computed. The search direction is the
%direction of the vector joining AB. The exit point ($X_{ex}$) is
%obtained by finding the peak of the function value along this
%vector. The dotted line indicates the stability boundary. The dashed
%line indicates the search direction.} \label{fig:myleps2}
%\end{figure}
%
%
%Step 3: {\it Moving along the stability boundary to locate the
%Minimum Gradient Point} : We used a novel {\it trajectory adjustment
%procedure} to move along the practical stability boundary. Once the
%exit point is identified, the consecutive points on the stability
%boundary can be identified by this trajectory-adjustment procedure.
%The exit point ($X_{ex}$) is integrated for a predefined number of
%times. Let $m'_1$ be the new point obtained after integration. The
%function value between $m'_1$ and the local minimum is evaluated and
%the peak value is obtained. Let the new boundary point along the
%vector $m'_1B$ starting from the point $m'_1$ and where the value
%attains the peak be $m_2$. This process is repeated and several
%points on the stability bondary are obtained. During this traversal,
%the value of the gradient along the boundary is noted and the
%process of moving along the boundary is terminated when the Minimum
%gradient point (MGP) is obtained. In summary, the trajectory of
%integration is being modified so that it moves towards the MGP and
%will not converge to one of the local minima. This is an intelligent
%TRUSTECH based scheme for following the stability boundary which is
%the {\it heart} of the proposed method. This step is named as the
%trajectory-adjustment procedure.
% If the value is
%immediately decreasing then it means that there is no peak in that
%search direction and hence the stability boundary will not be
%encountered in this direction. In this case, the search direction
%has to be modified. The simplest way to find the peak is to search
%in the exact opposite direction.
%
%Step 4: { \it Locating the Decomposition point (DP)} : The Minimum
%Gradient Point ($m_n$) obtained from the previous step will be
%present in the neighborhood of the decomposition point. A local
%minimizer to solve the system of nonlinear equations is applied with
%$m_n$ as initial guess and this will yield the decomposition point.
%A detailed survey about different Local minimizations
%applied to a wide variety of areas is given in \cite{Schlick02}. \\
%
%
%
%\begin{figure}[htp]
%\centerline{ \epsfig{figure=Figures/myleps3aa.ps, width=3.5in} }
%\caption {Illustration of the step 3 of our algorithm. $m_1$ is
%integrated till $m'_1$ is reached and traced back along the vector
%$m'_1B$ to get $m_2$, and so on... $m_n$ are the n points on the
%stability boundary. The $n^{th}$ point is the Minimum Gradient Point
%where the magnitude of the gradient ($G_M$) is the minimum. DP is
%the decomposition point.} \label{fig:energy}
%\end{figure}
%
%
%{\bf Remarks:}
%
%
%
%
%\begin{figure}[htp]
%\centerline{ \epsfig{figure=Figures/myleps3aa.ps, width=3.5in} }
%\caption {Illustration of the step 3 of our algorithm. $m_1$ is
%integrated till $m'_1$ is reached and traced back along the vector
%$m'_1B$ to get $m_2$, and so on... $m_n$ are the n points on the
%stability boundary. The $n^{th}$ point is the Minimum Gradient Point
%where the magnitude of the gradient ($G_M$) is the minimum. DP is
%the decomposition point.} \label{fig:energy}
%\end{figure}
%

%\begin{lem}\label{def:stableequilibriumpoint}
%A hyperbolic equilibrium point is called a (asymptotically) {\it
%stable equilibrium point} (SEP) if all the eigenvalues of its
%corresponding Jacobian have negative real part. Conversely, it is an
%{\it unstable equilibrium point} if some eigenvalues have a positive
%real part.
%\end{lem}
%
%An equilibrium point is called a {\it type-k equilibrium point} if
%its corresponding Jacobian has exact $k$ eigenvalues with positive
%real part. The {\it stable} ($W^s(\tilde{x})$) and {\it unstable}
%($W^u(\tilde{x})$) manifolds of an equilibrium point, say
%$\tilde{x}$, is defined as:
%\begin{center}
%\begin{eqnarray}
%W^s(\tilde{x}) = \{ x \in \Re^s ~:~
%\lim_{t\to\infty}\Phi(x,t)=\tilde{x}\} \\
%W^u(\tilde{x}) = \{ x \in \Re^s ~:~
%\lim_{t\to-\infty}\Phi(x,t)=\tilde{x}\} \label{eq:unstablemanifold}
%\end{eqnarray}
%\end{center}
%
%To comprehend the transformation, we need to define {\it energy function}. A smooth
%function $V(\cdot) : \Re^s \rightarrow \Re^s$ satisfying
%$\dot{V}(\Phi(\Theta,t))~<~0~,~\forall ~x \notin $ \{set of
%equilibrium points (E)\} and t $\in \Re^+ $ is termed as energy
%function.
%
%\begin{thm}\label{th:lyapunov}\cite{Chiang96}: $f(\Theta)$ is a
%energy function for the gradient system (\ref{eq:gradientsystem}).
%\end{thm}
%
%\begin{lem}\label{def:decompositionpoint}
%A type-1 equilibrium point $x_d$ (k=1) on the practical stability
%boundary of a stable equilibrium point $x_s$ is called a {\it
%decomposition point}.
%\end{lem}
%
%\begin{lem}\label{def:practicalstabilityregion} The {\it practical stability
%region} of a stable equilibrium point $x_s$ of a nonlinear dynamical
%system (\ref{eq:gradientsystem}), denoted by $A_p(x_s)$ and is the
%interior of closure of the stability region $A(x_s)$ which is given
%by :
%
%\begin{equation}
%A(x_s) = \{ x \in \Re^s ~:~ \lim_{t\to\infty}\Phi(x,t)=x_s\}
%\label{eq:stabilityregion}
%\end{equation}\vspace{0.05in}
%\end {lem}
%The boundary of practical stability region is called the {\it
%practical stability boundary} of $x_s$ and will be denoted by
%$\partial A_p(x_s)$. Theorem \ref{th:characterization1} asserts that
%the practical stability boundary is contained in the union of the
%closure of the stable manifolds of all the decomposition points on
%the practical stability boundary. Hence, if the decomposition points
%can be identified, then an explicit characterization of the
%practical stability boundary can be established using
%(\ref{eq:charpracstabilityregion}). This theorem gives an explicit
%description of the geometrical and dynamical structure of the
%practical stability boundary.
%
%\begin{thm}{\it (Characterization of practical stability
%boundary)\cite{Lee04}:} Consider a negative gradient system
%described by (\ref {eq:gradientsystem}). Let $\sigma_i$ , i=1,2,...
%be the decomposition points on the practical stability boundary
%$\partial A_p(x_s)$ of a stable equilibrium point, say $x_s$. Then
%\end{thm}
%

Our approach takes advantage of TRUST-TECH (TRansformation Under
STability-reTaining Equilibria CHaracterization) to compute
neighborhood local optimal solutions on the surface using stability
regions. Originally, the basic idea of our algorithm was to find
decomposition points on the practical stability boundary. Since,
each decomposition point connects two local optima uniquely, it is
important to obtain the saddle points from the given solution
and then move to the next solution through this decomposition
point. The details of a stability boundary tracing algorithm to obtain decomposition points on the stability boundary is presented in \cite{Reddy06}. Though, this procedure gives a guarantee that
the local maximum is not revisited, the computational expense for
tracing the stability boundary and identifying the decomposition
point is high compared to the cost of applying the local solver
directly using the exit point without considering the decomposition
point. However, it is beneficial to use the saddle point tracing procedure developed in
\cite{Reddy06} for applications where the local methods are very expensive. For most of the applications that arise in machine learning domain, it is not necessary to obtain the saddle point because of the fact that the local methods are highly optimized for the specific problem in hand and in general, these methods are much cheaper than tracing the boundary using gradient computation.





==> orig/unsupervised-global.tex <==

\section{Unsupervised Learning : Mixture Modeling}
\label{sec:trust-tech-em} In this section, we develop a TRUST-TECH
based algorithm for solving the problem of mixture modeling
\cite{Reddy08}. One of the most popular methods used for fitting
mixture models to the observed data is the {\it
Expectation-Maximization} (EM) algorithm which converges to the
maximum likelihood estimate of the mixture parameters locally
\cite{Demspter77}. Without loss of generality, we will consider the
problem of learning parameters of Gaussian Mixture Models (GMM).
Given the number of components and an initial set of parameters, EM
algorithm can be applied to compute the optimal estimates of the
parameters that maximize the likelihood of the data given the
estimates of these components. However, the main problem with the EM
algorithm is that it is a `{\it greedy}' method which is very
sensitive to the given initial set of parameters \cite{Reddy08}.
Although EM and its variants have been extensively used for learning
mixture models, several researchers have approached the problem by
identifying new techniques that give good initialization. Though
shown only for the case of multivariate Gaussian mixtures, our
technique can be effectively applied to any parametric finite
mixture model.

 Although EM and its variants have been extensively
used for learning mixture models, several researchers have
approached the problem by identifying new techniques that give good
initial points. More generic techniques like deterministic annealing
\cite {Rose98,Ueda98}, genetic algorithms
\cite{Pernkopf05,Martínez00} have been applied to obtain a good set
of parameters. Though, these techniques have asymptotic guarantees,
they are very time consuming and hence may not be used for most of
the practical applications. Some problem specific algorithms like
split and merge EM \cite{Ueda00}, component-wise EM
\cite{Figueiredo02}, greedy learning \cite{Verbeek03}, incremental
version for sparse representations \cite{neal98}, parameter space
grid \cite{Li99} are also proposed in the literature. Some of these
algorithms are either computationally very expensive or infeasible
when learning mixtures in high dimensional spaces \cite{Li99}.
Inspite of all the expense in these methods, very little effort has
been taken to explore promising subspaces within the larger
parameter space. Most of these algorithms eventually apply the EM
algorithm to move to a locally maximal set of parameters on the
likelihood surface. Simple approaches like running EM from several
random initializations, and then choosing the final estimate that
leads to the local maximum with higher value of the likelihood can
be successful to certain extent \cite{hastie96,Roberts98}.

\subsection{Mixture Models and the EM Algorithm}


\begin{table}[h]
\centering \caption{\protect Description of the Notations used}
\begin{center}
\begin{tabular}{cl}
\hline  Notation &   Description \\
 \hline

 d & number of features\\
 n & number of data points\\
 k & number of components\\
 s & total number of parameters\\
 $\Theta$ & parameter set\\
 $\theta_i$ & parameters of $i^{th}$ component\\
 $\alpha_i$ & mixing weights for $i^{th}$ component\\
 $\mathcal{X}$ & observed data\\
 $\mathcal{Z}$ & missing data\\
 $\mathcal{Y}$ & complete data\\
 t &  timestep for the estimates\\
 \hline
\end{tabular}
\end{center}
\label{TB:datanot}
\end{table}

Table~\ref{TB:datanot} gives the notations used in this section.
Lets assume that there are $k$ Gaussians in the mixture model. The
form of the probability density function is as follows :

\begin{equation}\label{eq:gaussian1}
    p(x|\Theta) =\sum_{i=1}^{k}{\alpha_i p(x|\theta_i)}
\end{equation}

\noindent where $x=[x_1,x_2,...,x_d]^T$ is the feature vector of $d$
dimensions. The $\alpha_k$'s represent the {\it mixing weights}.
$\Theta$ represents the parameter set ($\alpha_1, \alpha_2,...
\alpha_k,\theta_1,\theta_2,...\theta_k$) and $p$ is a univariate
Gaussian density parameterized by $\theta_i$(i.e. $\mu_i$ and
$\sigma_i$):

\begin{equation}\label{eq:gaussiandensity}
    p(x|\theta_i) =\frac{1}{\sqrt{(2\pi)}\sigma_i}e^{-\frac{(x-\mu_i)^2}{2\sigma_i^2}}
\end{equation}

Also, it should be noticed that being probabilities $\alpha_i$ must
satisfy

\begin{equation}\label{eq:probabi}
    0 \leq \alpha_i\leq 1 ~,~ \forall i=1,..,k,~ and ~~ \sum_{i=1}^k
    \alpha_i=1
\end{equation}

Given a set of n i.i.d samples
$\mathcal{X}=\{x^{(1)},x^{(2)},..,x^{(n)}\}$, the log-likelihood
corresponding to a mixture is

\begin{equation}\label{eq:log}
%\begin{split}
    log ~p(\mathcal{X}|\Theta)=log \prod_{j=1}^n
    ~p(x^{(j)}|\Theta)\\
     =\sum_{j=1}^n log \sum_{i=1}^k \alpha_i
    ~p(x^{(j)}|\theta_i)
%\end{split}
\end{equation}

The goal of learning mixture models is to obtain the parameters
$\widehat{\Theta}$ from a set of n data points which are the samples
of a distribution with density given by (\ref{eq:gaussian1}). The
{\it Maximum Likelihood Estimate } (MLE) is given by :
\begin{equation}\label{eq:MLE}
\widehat{\Theta}_{MLE} = arg \max_{\tilde{\Theta}} ~\{~log
~p(\mathcal{X}|\Theta)~\}
\end{equation}

where $\tilde{\Theta}$ indicates the entire parameter space. Since,
this MLE cannot be found analytically for mixture models, one has to
rely on iterative procedures that can find the global maximum of
$log~ p(\mathcal{X}|\Theta)$. The EM algorithm has been used
successfully to find the local maximum of such a function
\cite{McLachlan97}. The EM algorithm assumes $\mathcal{X}$ to be
$observed$ data. The missing part, termed as $hidden$ data, is a set
of {\it n} labels $\mathcal{Z}=\{\footnotesize{\bf
z}^{(1)},\footnotesize{\bf z}^{(2)},..,\footnotesize{\bf z}^{(n)}\}$
associated with $n$ samples, indicating which component produced
each sample \cite{McLachlan97}. Each label $\footnotesize{\bf
z}^{(j)}=[z_1^{(j)},z_2^{(j)},..,z_k^{(j)}]$ is a binary vector
where $z_i^{(j)}=1$ and $z_m^{(j)}=0$  $\forall m \neq i$, means the
sample $x^{(j)}$ was produced by the $i^{th}$ component. Now, the
complete log-likelihood i.e. the one from which we would estimate
$\Theta$ if the {\it complete data}
$\mathcal{Y}=~\{~\mathcal{X},\mathcal{Z}~\}$ is

\begin{equation*}\label{eq:beforecomplete}
    log ~p(\mathcal{X},\mathcal{Z}|\Theta)=\sum_{j=1}^n ~log \prod_{i=1}^k
    ~ [~\alpha_i~p(x^{(j)}|\theta_i)~]^{z_i^{(j)}}
\end{equation*}


\begin{equation}\label{eq:complete}
    log ~p(\mathcal{Y}|\Theta)=\sum_{j=1}^n \sum_{i=1}^k
    z_i^{(j)}~log~ [~\alpha_i~p(x^{(j)}|\theta_i)~]
\end{equation}
The nonlinear transformation gives the correspondence between all
the critical points of the $s$-dimensional likelihood surface and
that of its dynamical system. For the case of spherical Gaussian
mixtures with $k$ components, we have the number of unknown
parameters $s=3k-1$. For convenience, the maximization problem is
transformed into a minimization problem defined by the following
objective function :
\begin{equation}
%\begin{split}
~\max_\Theta ~\{~log ~p(\mathcal{X}|\Theta)~\}=~\min_\Theta
~\{~-~log
~p(\mathcal{X}|\Theta)~\}\\= \min_\Theta f(\Theta)\label{eq:problem1} %\end{split}
\end{equation}

\begin{thm}\label{def:cont}
$f(\Theta)$ is $C^2(\Re^s,\Re)$.
\end{thm}
\begin{proof}
Note from Eq.(\ref{eq:log}), we have
\begin{equation}\label{eq:otherlog1}
    f(\Theta)=-log ~p(\mathcal{X}|\Theta)
    =-\sum_{j=1}^n log \sum_{i=1}^k \alpha_i
    ~p(\bm{x}^{(j)}|\bm{\theta}_i)
\end{equation}

Each of the simple functions which appear in Eq.
(\ref{eq:otherlog1}) are twice differentiable and continuous in the
interior of the domain over which $f(\Theta)$ is defined. The
function $f(\Theta)$ is composed of arithmetic operations of these
simple functions and from basic results in analysis, we can conclude
that $f(\Theta)$ is twice continuously differentiable.

%This completes the proof.
\end{proof}

Lemma \ref{def:cont} and the preceeding arguments guarantee the
existence of the gradient system associated with $f(\Theta)$ for the
log-likelihood function in the case of spherical Gaussians and
allows us to construct the following negative gradient system :
\begin{equation}
\begin{split}
\textstyle{ \left[ \dot{\mu}_1(t)~..~\dot{\mu}_k(t)~\dot{\sigma}_1(t) ~..~\dot{\sigma}_k(t)~\dot{\alpha}_1(t) ~..~\dot{\alpha}_{k-1}(t)\right]^T}\\
=~-~\left[ \frac{\partial f}{\partial \mu_1}~..~\frac{\partial
f}{\partial \mu_k}~\frac{\partial f}{\partial
\sigma_1}~..~\frac{\partial f}{\partial \sigma_k}~\frac{\partial
f}{\partial \alpha_1}~..~\frac{\partial f}{\partial \alpha_{k-1}}
\right]^T  \label{def:loggrad}
\end{split}
\end{equation}


\subsection{Nonlinear Transformation}
This section mainly deals with the transformation of the original
log-likelihood function into its corresponding nonlinear dynamical
system and introduces some terminology pertinent to comprehend our
algorithm. This transformation gives the correspondence between all
the critical points of the $s$-dimensional likelihood surface and
that of its dynamical system. For the case of spherical Gaussian
mixtures with $k$ components, we have the number of unknown
parameters $s=3k-1$. For convenience, the maximization problem is
transformed into a minimization problem defined by the following
objective function :
\begin{equation}
%\begin{split}
~\max_\Theta ~\{~log ~p(\mathcal{X}|\Theta)~\}=~\min_\Theta
~\{~-~log
~p(\mathcal{X}|\Theta)~\}\\= \min_\Theta f(\Theta)\label{eq:problem1} %\end{split}
\end{equation}

%where $f(\Theta)$ is assumed to be in $C^2(\Re^s,\Re)$.

\begin{lem1}\label{def:cont}
$f(\Theta)$ is $C^2(\Re^s,\Re)$.
\end{lem1}
\begin{proof}

Note from Eq.(\ref{eq:log}), we have
\begin{equation}\label{eq:otherlog1}
    f(\Theta)=-log ~p(\mathcal{X}|\Theta)
    =-\sum_{j=1}^n log \sum_{i=1}^k \alpha_i
    ~p(\bm{x}^{(j)}|\bm{\theta}_i)
\end{equation}
Each of the simple functions which appear in Eq.
(\ref{eq:otherlog1}) are twice differentiable and continuous in the
interior of the domain over which $f(\Theta)$ is defined. The
function $f(\Theta)$ is composed of arithmetic operations of these
simple functions and from basic results in analysis, we can conclude
that $f(\Theta)$ is twice continuously differentiable.
\end{proof}

Lemma \ref{def:cont} and the preceeding arguments guarantee the
existence of the gradient system associated with $f(\Theta)$ for the
log-likelihood function in the case of spherical Gaussians and
allows us to construct the following negative gradient system :
\begin{equation}
\begin{split}
\textstyle{ \left[ \dot{\mu}_1(t)~..~\dot{\mu}_k(t)~\dot{\sigma}_1(t) ~..~\dot{\sigma}_k(t)~\dot{\alpha}_1(t) ~..~\dot{\alpha}_{k-1}(t)\right]^T}\\
=~-~\left[ \frac{\partial f}{\partial \mu_1}~..~\frac{\partial
f}{\partial \mu_k}~\frac{\partial f}{\partial
\sigma_1}~..~\frac{\partial f}{\partial \sigma_k}~\frac{\partial
f}{\partial \alpha_1}~..~\frac{\partial f}{\partial \alpha_{k-1}}
\right]^T  \label{def:loggrad}
\end{split}
\end{equation}


Developing a gradient system is one of the simplest transformation
possible. One can think of a more complicated nonlinear
transformations as well. We will now describe three main guidelines
that must be satisfied by the transformation:

\begin{itemize}
\item{The original log-likelihood function must be a Lyapunov function for the dynamical system.}
\item{The location of the critical points must be preserved under this transformation.}
\item{The system must be completely stable. In other words, every trajectory $\Phi(x,t)$ must be bounded.}
\end{itemize}
%
%\subsection{TRUST-TECH based Expectation Maximization}
%\label{sec:algorithm}
%
%Our framework consists three stages namely: (i) global stage, (ii)
%local stage and (iii) neighborhood-search stage. The last two stages
%are repeated in the solution space to obtain promising solutions.
%Global method obtains promising subspaces of the solution space. The
%next stage is the local stage (or the EM stage) where the results
%from the global methods are refined to the corresponding locally
%optimal parameter set. Then, during the neighborhood search stage,
%the exit points are computed and the neighborhood solutions are
%systematically explored through these exit points.
%
%It is beneficial to use the TRUST-TECH based algorithm at the
%promising subspaces. In this sense, the neighborhood-search stage
%can act as a interface between global methods for initialization and
%the EM algorithm which gives the local maxima. This approach differs
%from traditional local methods by computing multiple local maxima in
%the neighborhood region. This also enhances user flexibility in
%choosing between different sets of good clusterings. Though global
%methods can identify promising subsets, it is important to explore
%this more thoroughly especially in problems like parameter
%estimation.
%
%
%\begin{algorithm}
%\caption{TRUST-TECH based EM Algorithm} \label{nexttieralg}
%\begin{algorithmic}
%\STATE \textbf{Input:} Parameters $\Theta$, Data  $\mathcal{X}$,
%tolerance $\tau$, Step $S_p$  \STATE \textbf{Output:}
%$\widehat{\Theta}_{MLE} $  \STATE \textbf{Algorithm:}
%
%\STATE Apply global method and store the q promising solutions $
%\Theta_{init}=\{\Theta_1,\Theta_2,..,\Theta_q\}$ ~~~~~~~~ Initialize
%E= $\phi$
%
%\WHILE{$\Theta_{init} \neq \phi$} \STATE Choose $\Theta_i \in
%\Theta_{init}$, set $\Theta_{init}= \Theta_{init} \backslash
%\{\Theta_i\}$ \STATE $LM_i=EM(\Theta_i,\mathcal{X},\tau)$~~~~~~~~~
%$E=E \cup \{LM_i\}$ \STATE Generate promising direction vectors
%$d_j$ from $LM_i$
%
%\FOR {each $d_j$} \STATE Compute Exit Point ($X_j$) along $d_j$
%starting from $LM_i$ by evaluating the log-likelihood function given
%by (\ref {eq:log})
%
%\STATE $New_j=EM(X_j+\epsilon \cdot d_j,\mathcal{X},\tau)$
%\IF{$new_j \notin E$} \STATE $E=E \cup New_j$ \ENDIF
%
%\ENDFOR
%
%   \ENDWHILE
%\STATE $\widehat{\Theta}_{MLE} =max\{val(E_i)\}$
%\end{algorithmic}
%\end{algorithm}
%
%
%In order to escape out of a found local maximum, our method needs to
%compute certain promising directions based on the local behaviour of
%the function. One can realize that generating these promising
%directions is one of the important aspects of our algorithm.
%Surprisingly, choosing random directions to move out of the local
%maximum works well for this problem. One might also use other
%directions like eigenvectors of the Hessian or incorporate some
%domain-specific knowledge (like information about priors,
%approximate location of cluster means, user preferences on the final
%clusters) depending on the application that they are working on and
%the level of computational expense that they can afford. We used
%random directions in our work because they are very cheap to
%compute. Once the promising directions are generated, exit points
%are computed along these directions. {\it Exit points} are points of
%intersection between any given direction and the practical stability
%boundary of that local maximum along that particular direction. If
%the stability boundary is not encountered along a given direction,
%then there is a guarantee that one will not be able to find any new
%local maximum in that direction. With a new initial guess in the
%vicinity of the exit points, EM algorithm is applied again to obtain
%a new local maximum. Sometimes, this new point ($X_j+\epsilon \cdot
%d_j$) might have convergence problems. In such cases, TRUST-TECH can
%help the convergence by integrating the dynamical system and
%obtaining another point that is much closer to the local optimal
%solution. However, this is not done here because of the fact that
%the computation of gradient for log-likelihood function is
%expensive.
%


\subsection{Results and Discussion} \label{sec:results}

The TRUST-TECH based EM algorithm has been tested on three synthetic
and two real datasets as described in \cite{Reddy08}.
Table~\ref{TB:results5} summarizes our results over 100 runs. The
mean and the standard deviations of the log-likelihood values are
reported. The traditional EM algorithm with random starts is
compared against our algorithm on both synthetic and real data sets.
Our algorithm not only obtains higher likelihood value but also
produces it with high confidence. The low standard deviation of our
results indicates the robustness of obtaining the global maximum.
Our method assumes that the underlying distribution of the data is
mixture of Gaussians. Table~\ref{TB:compresults5} gives the results
of TRUST-TECH-EM compared with other methods like split and merge EM
and k-means+EM proposed in the literature.


\begin{table*}[htp]
\centering \caption{\protect\small Performance of our algorithm on
an average of 100 runs on various synthetic and real datasets}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\small Dataset &\small Samples &\small  Clusters & \small Features &\small   EM (mean $\pm$ std) & \small TRUST-TECH-EM (mean $\pm$ std)\\
\hline Spherical & 40& 5 & 2  & 38.07$\pm$2.12 & 43.55$\pm$0.6 \\
\hline Elliptical & 900& 3 & 2  &  -3235$\pm$0.34 & -3078.7$\pm$0.03 \\
\hline Full covariance 1& 500& 4 & 2  & -2345.5 $\pm$175.13 & -2121.9$\pm$ 21.16 \\
\hline Full covariance 2& 2000& 4 & 2  & -9309.9 $\pm$694.74 & -8609.7 $\pm$37.02 \\
\hline Iris & 150& 3 & 4  & -198.13$\pm$27.25 &-173.63$\pm$11.72\\
\hline Wine & 178& 3 & 13  & -1652.7$\pm$1342.1& -1618.3$\pm$1349.9\\
\hline
\end{tabular}
\end{center}
\label{TB:results5}
\end{table*}


\begin{table}[htp]
\centering \caption{\protect\small Comparison of TRUST-TECH-EM with
other methods}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Method & Elliptical & Iris\\
\hline RS+EM & -3235 $\pm$ 14.2 & -198 $\pm$ 27\\
\hline K-Means+EM & -3195 $\pm$ 54&-186 $\pm$ 10\\
\hline SMEM &-3123 $\pm$ 54&-178.5 $\pm$ 6\\
\hline TRUST-TECH-EM &-3079 $\pm$ 0.03 &-173.6 $\pm$ 11\\
\hline
\end{tabular}
\end{center}
\label{TB:compresults5}
\end{table}


==> orig/unsupervised.tex <==
\section{Unsupervised Learning - Model-based Clustering}
In this section, we will develop a stability region based algorithm for solving the problem of mixture modeling. Finite mixtures allow a probabilistic model-based approach to
unsupervised learning \cite{McLachlan88} which plays an important
role in predictive data mining applications. One of the most popular
methods used for fitting mixture models to the observed data is the
{\it Expectation-Maximization} (EM) algorithm which converges to the
maximum likelihood estimate of the mixture parameters locally
\cite{Demspter77,Figueiredo02}. The usual steepest descent,
conjugate gradient, or Newton-Raphson methods are too complicated
for use in solving this problem \cite{Xu96}. EM has become a popular
method since it takes advantages of problem specific properties. EM
based approaches have been successfully used to solve problems that
arise in various other applications \cite {Nigam00,Carson02}.

Without loss of generality, we will consider the problem of learning parameters of
Gaussian Mixture Models (GMM). Fig~\ref{fig:gmm} shows data
generated by three Gaussian components with different mean and
variance. Note that every data point has a probabilistic (or soft)
membership that gives the probability with which it belongs to each
of the components. Points that belong to component 1 will have high
probability of membership for component 1. On the other hand, data
points belonging to components 2 and 3 are not well separated. The
problem of learning mixture models involves not only estimating the
parameters of these components but also finding the probabilities
with which each data point belongs to these components. Given the
number of components and an initial set of parameters, EM algorithm
can be applied to compute the optimal estimates of the parameters
that maximize the likelihood of the data given the estimates of
these components. However, the main problem with the EM algorithm is
that it is a `{\it greedy}' method which is very sensitive to the
given initial set of parameters \cite{Reddy06b}. To overcome this problem, a novel
two phase algorithm based on stability region analysis is proposed.
The main research concerns that motivated the new algorithm
presented in this paper are :
\begin {itemize}
\item{EM algorithm for mixture modeling converges to a local maximum
of the likelihood function very quickly.}

\item{There are many other promising local optimal solutions in
the close vicinity of the solutions obtained from the methods that
provide good initial guesses of the solution.}

\item{Model selection criteria usually assumes that the global
optimal solution of the log-likelihood function can be obtained.
However, achieving this is computationally intractable.}

\item{Some regions in the search space do not contain any promising solutions.
The promising and non-promising regions coexist and it becomes
challenging to avoid wasting computational resources to search in
non-promising regions.}

\end{itemize}


Of all the concerns mentioned above, the fact that most of the local
maxima are not distributed uniformly \cite{Ueda98} makes it
important for us to develop algorithms that not only help us to
avoid searching in the low-likelihood regions but also emphasize the
importance of exploring promising subspaces more thoroughly. This
subspace search will also be useful for making the solution less
sensitive to the initial set of parameters. Here, we
propose a novel two phase stability region based expectation maximization (SREM) algorithm for estimating the parameters of
mixture models. Using concepts of dynamical systems and EM algorithm
simultaneously to exploit the problem specific features of the
mixture models, our algorithm obtains the optimal set of parameters
by searching for the global maximum on the likelihood surface in a
systematic manner.

\begin{figure}
\centerline{
  \epsfig{figure=Figures/gmm1.ps, width=2.5in}
} \caption{Data generated by three Gaussian components. The problem
of learning mixture models is to obtain the parameters of these
Gaussian components and the membership probabilities of each
datapoint.} \label{fig:gmm}
\end{figure}

\subsection{Relevant Background}
\label{sec:background}  Although EM and its variants have been
extensively used for learning mixture models, several researchers
have approached the problem by identifying new techniques that give
good initialization. More generic techniques like deterministic
annealing \cite {Ueda98}, genetic algorithms \cite{Pernkopf05} have
been applied to obtain a good set of parameters. Though, these
techniques have asymptotic guarantees, they are very time consuming
and hence cannot be used for most of the practical applications.
Some problem specific algorithms like split and merge EM
\cite{Ueda00}, component-wise EM \cite{Figueiredo02}, greedy
learning \cite{Verbeek03}, incremental version for sparse
representations\cite{neal98}, parameter space grid \cite{Li99} are
also proposed in the literature. Some of these algorithms are either
computationally very expensive or infeasible when learning mixtures
in high dimensional spaces \cite{Li99}. Inspite of all the expense
in these methods, very little effort has been taken to explore
promising subspaces within the larger parameter space. Most of these
algorithms eventually apply the EM algorithm to move to a locally
optimal set of parameters on the likelihood surface. Simpler
practical approaches like running EM from several random
initializations, and then choosing the final estimate that leads to
the local maximum with higher value of the likelihood are also
successful to certain extent \cite{Roberts98}.

The dynamical system of the log-likelihood function
reveals more information on the neighborhood stability regions and
their corresponding local maxima \cite{Chiang96}. Hence, the
difficulties of finding good solutions when the error surface is
very rugged can be overcome by adding stability region based
mechanisms to escape out of the convergence zone of the local
maxima. Though this method might introduce some additional cost, one
has to realize that existing approaches are much more expensive due
to their stochastic nature. Specifically, for a problem in this
context, where there is a non-uniform distribution of local maxima,
it is difficult for most of the methods to search neighboring
regions \cite{Zhang04}.

\subsection{Preliminaries}
\label{sec:problem} We now introduce some necessary preliminaries on
mixture models, EM algorithm and stability regions. First, we
describe the notation used in this section:

\begin{table}[h]
\centering \caption{\protect\small Description of the Notations
used}
\begin{center}
\begin{tabular}{cl}
\hline  Notation &   Description \\
 \hline

 d & number of features\\
 n & number of data points\\
 k & number of components\\
 s & total number of parameters\\
 $\Theta$ & parameter set\\
 $\theta_i$ & parameters of $i^{th}$ component\\
 $\alpha_i$ & mixing weights for $i^{th}$ component\\
 $\mathcal{X}$ & observed data\\
 $\mathcal{Z}$ & missing data\\
 $\mathcal{Y}$ & complete data\\
 t &  timestep for the estimates\\
 \hline
\end{tabular}
\end{center}
\label{TB:data}
\end{table}

\subsubsection{Mixture Models}

Lets assume that there are $k$ Gaussians in the mixture model. The
form of the probability density function is as follows:

\begin{equation}\label{eq:gaussian}
    p(x|\Theta) =\sum_{i=1}^{k}{\alpha_i p(x|\theta_i)}
\end{equation}

where $x=[x_1,x_2,...,x_d]^T$ is the feature vector of $d$
dimensions. The $\alpha_k$'s represent the {\it mixing weights}.
$\Theta$ represents the parameter set ($\alpha_1, \alpha_2,...
\alpha_k,\theta_1,\theta_2,...\theta_k$) and $p$ is a univariate
Gaussian density parameterized by $\theta_i$(i.e. $\mu_i$ and
$\sigma_i$):

\begin{equation}\label{eq:gaussiandensity}
    p(x|\theta_i) =\frac{1}{\sqrt{(2\pi)}\sigma_i}e^{-\frac{(x-\mu_i)^2}{2\sigma_i^2}}
\end{equation}

Also, it should be noticed that being probabilities $\alpha_i$ must
satisfy

\begin{equation}\label{eq:probabi}
    0 \leq \alpha_i\leq 1 ~,~ \forall i=1,..,k,~ and ~~ \sum_{i=1}^k
    \alpha_i=1
\end{equation}

Given a set of n i.i.d samples
$\mathcal{X}=\{x^{(1)},x^{(2)},..,x^{(n)}\}$, the log-likelihood
corresponding to a mixture is

\begin{equation}\label{eq:log}
\begin{split}
    log ~p(\mathcal{X}|\Theta)&=log \prod_{j=1}^n
    ~p(x^{(j)}|\Theta)\\
    & \quad =\sum_{j=1}^n log \sum_{i=1}^k \alpha_i
    ~p(x^{(j)}|\theta_i)
\end{split}
\end{equation}

The goal of learning mixture models is to obtain the parameters
$\widehat{\Theta}$ from a set of n data points which are the samples
of a distribution with density given by (\ref{eq:gaussian}). The
{\it Maximum Likelihood Estimate } (MLE) is given by :
\begin{equation}\label{eq:MLE}
\widehat{\Theta}_{MLE} = arg \max_{\tilde{\Theta}} ~\{~log
~p(\mathcal{X}|\Theta)~\}
\end{equation}

where $\tilde{\Theta}$ indicates the entire parameter space. Since,
this MLE cannot be found analytically for mixture models, one has to
rely on iterative procedures that can find the global maximum of
$log~ p(\mathcal{X}|\Theta)$. The EM algorithm described in the next
section has been used successfully to find the local maximum of such
a function \cite{McLachlan97}.

\subsubsection{Expectation Maximization}

The EM algorithm assumes $\mathcal{X}$ to be $observed$ data. The
missing part, termed as $hidden$ data, is a set of {\it n} labels
$\mathcal{Z}=\{\footnotesize{\bf z}^{(1)},\footnotesize{\bf
z}^{(2)},..,\footnotesize{\bf z}^{(n)}\}$ associated with $n$
samples, indicating which component produced each sample
\cite{McLachlan97}. Each label $\footnotesize{\bf
z}^{(j)}=[z_1^{(j)},z_2^{(j)},..,z_k^{(j)}]$ is a binary vector
where $z_i^{(j)}=1$ and $z_m^{(j)}=0$  $\forall m \neq i$, means the
sample $x^{(j)}$ was produced by the $i^{th}$ component. Now, the
complete log-likelihood (i.e. the one from which we would estimate
$\Theta$ if the {\it complete data}
$\mathcal{Y}=~\{~\mathcal{X},\mathcal{Z}~\}$ is

\begin{equation*}\label{eq:beforecomplete}
    log ~p(\mathcal{X},\mathcal{Z}|\Theta)=\sum_{j=1}^n ~log \prod_{i=1}^k
    ~ [~\alpha_i~p(x^{(j)}|\theta_i)~]^{z_i^{(j)}}
\end{equation*}


\begin{equation}\label{eq:complete}
    log ~p(\mathcal{Y}|\Theta)=\sum_{j=1}^n \sum_{i=1}^k
    z_i^{(j)}~log~ [~\alpha_i~p(x^{(j)}|\theta_i)~]
\end{equation}

The EM algorithm produces a sequence of estimates
$\{\widehat{\Theta}(t),t=0,1,2,...\}$ by alternately applying the
following two steps until convergence:

\begin {itemize}
\item{{\bf E-Step : } Compute the conditional expectation of the
hidden data, given $\mathcal{X}$ and the current estimate
$\widehat{\Theta}(t)$. Since $log~p(\mathcal{X,Z}|\Theta)$ is linear
with respect to the missing data $\mathcal{Z}$, we simply have to
compute the conditional expectation $\mathcal{W} \equiv
E[\mathcal{Z|X},\widehat{\Theta}(t)]$, and plug it into $log ~p
(\mathcal{X,Z}|\Theta)$. This gives the $Q$-function as follows:


 \begin{equation}\label{eq:qfunc}
\begin{split}
    Q(\Theta|\widehat{\Theta}(t))&\equiv
   E_Z[log~p(\mathcal{X},\mathcal{Z})|\mathcal{X},\widehat{\Theta}(t)]
 \end{split}
\end{equation}

Since $\mathcal{Z}$ is a binary vector, its conditional expectation
is given by :

\begin{equation}\label{eq:conditionw}
\begin{split}
    w_i^{(j)}& \equiv E~[~z_i^{(j)}|\mathcal{X},\widehat{\Theta}(t)~] \\
& \quad = Pr~[~z_i^{(j)}=1|x^{(j)},\widehat{\Theta}(t)~]\\
& \quad =
    \frac{\widehat{\alpha}_i(t) p(x^{(j)}|\widehat{\theta}_i(t))}{\sum_{i=1}^{k}{\widehat{\alpha}_i(t) p(x^{(j)}|\widehat{\theta}_i(t))}}
\end{split}
\end{equation}

where the last equality is simply the Bayes law ($\alpha_i$ is the a
priori probability that $z_i^{(j)}=1$), while $w_i^{(j)}$ is the a
posteriori probability that $z_i^{(j)}=1$ given the observation
$x^{(j)}$.}

\item{{\bf M-Step : } The estimates of the new parameters are
updated using the following equation :

\begin{equation}\label{eq:update}
    \widehat{\Theta} (t+1) = arg \max_{\Theta}\{Q(\Theta,\widehat{\Theta}(t))\}
\end{equation}
}
\end{itemize}
\subsubsection{EM for GMMs}

Several variants of the EM algorithm have been extensively used to
solve this problem. The convergence properties of the EM algorithm
for Gaussian mixtures are thoroughly discussed in \cite{Xu96}. The
$Q-function$ for GMM is given by:

 \begin{equation}\label{eq:qfuncgmm}
 \begin{split}
 Q(\Theta|\widehat{\Theta}(t))= \sum_{j=1}^{n}\sum_{i=1}^{k} & w_i^{(j)}[log\frac{1}{\sigma_i\sqrt{2\pi}} \\&\quad-\frac{(x^{(j)}-\mu_i)^2}{2\sigma_i^2}+log ~\alpha_i]
\end{split}
\end{equation}

where
 \begin{equation}\label{eq:expectz}
w_i^{(j)}=\frac{\frac{\alpha_i(t)}{\sigma_i(t)}e^{-\frac{1}{2\sigma_i(t)^2}(x^{(j)}-\mu_i(t))^2}}{\sum_{i=1}^k
\frac{\alpha_i(t)}{\sigma_i(t)}e^{-\frac{1}{2\sigma_i(t)^2}(x^{(j)}-\mu_i(t))^2}}
 \end{equation}

The maximization step is given by the following equation :
 \begin{equation}\label{eq:max}
    \frac{\partial }{\partial \Theta_k} Q(\Theta|\widehat{\Theta}(t))= 0
\end{equation}
where $\Theta_k$ is the parameters for the $k^{th}$ component.
Because of the assumption made that each data point comes from a
single component, solving the above equation becomes trivial. The
updates for the maximization step in the case of GMMs are given as
follows:

\begin{eqnarray*}
\begin{split}
&\mu_i(t+1) = \frac{\sum_{j=1}^{n}w_i^{(j)}x^{(j)}}{\sum_{j=1}^{n}w_i^{(j)}}\\
&  \sigma_i^2(t+1) = \frac{\sum_{j=1}^{n}w_i^{(j)} (x^{(j)}-\mu_i(t+1))^2}{\sum_{j=1}^{n}w_i^{(j)}}\\
&\alpha_i(t+1)=\frac{1}{n}\sum_{j=1}^{n}w_i^{(j)} \label{eq:update}
\end{split}
\end{eqnarray*}

\subsubsection{Stability Regions}
This section mainly deals with the transformation of the original
log-likelihood function into its corresponding nonlinear dynamical
system and introduces some terminology pertinent to comprehend our
algorithm. This transformation gives the correspondence between all
the critical points of the $s$-dimensional likelihood surface and
that of its dynamical system. For the case of spherical Gaussian
mixtures with $k$ components, we have the number of unknown
parameters $s=3k-1$. For convenience, the maximization problem is
transformed into a minimization problem defined by the following
objective function :

\begin{equation}
\begin{split}
~\max_\Theta ~\{~log
~p(\mathcal{Y}|\Theta)~\}&=~\min_\Theta ~\{~-~log
~p(\mathcal{Y}|\Theta)~\}\\& \quad = \min_\Theta f(\Theta)\label{eq:problem} \end{split}
\end{equation}

where $f(\Theta)$ is assumed to be in $C^2(\Re^s,\Re)$.


 The gradient system for the log-likelihood
function in the case of spherical Gaussians is constructed as
follows :


\[ \textstyle{ \left[ \dot{\mu}_1(t)~..~\dot{\mu}_k(t)~\dot{\sigma}_1(t) ~..~\dot{\sigma}_k(t)~\dot{\alpha}_1(t) ~..~\dot{\alpha}_{k-1}(t)\right]^T}
\]
\newline
\[=~   -~\left[ \frac{\partial f}{\partial
\mu_1}~..~\frac{\partial f}{\partial \mu_k}~\frac{\partial
f}{\partial \sigma_1}~..~\frac{\partial f}{\partial
\sigma_k}~\frac{\partial f}{\partial \alpha_1}~..~\frac{\partial
f}{\partial \alpha_{k-1}} \right]^T \]

where \\


\begin{eqnarray}
\begin{split}
&\frac{\partial f}{\partial \mu_i} = \sum_{j=1}^{n}w_i^{(j)}\frac{(x^{(j)}-\mu_i)}{2\sigma_i^2}~~~~~~~~~~~~~~~~~\forall i=1,..,k\\
&\frac{\partial f}{\partial
\sigma_i}=\sum_{j=1}^{n}w_i^{(j)}\left[-\frac{1}{\sigma_i}+\frac{(x^{(j)}-\mu_i)^2}{\sigma_i^3}
\right] ~~~\forall
i=1,..,k\\
& \frac{\partial f}{\partial \alpha_i} = \frac{1}{\alpha_i}\sum_{j=1}^{n}w_i^{(j)} ~~~~~~~~~~~~~~~~~~~~~~~~~\forall i=1,..,k-1\\
\label{eq:update}
\end{split}
\end{eqnarray}

For simplicity, we show the construction of the gradient system for
the case of spherical Gaussians. It can be easily extended to the
full covariance Gaussian mixture case. It should be noted that only
(k-1) $\alpha$ values are considered in the gradient system because
of the unity constraint. The dependent variable $\alpha_k$ is
written as follows:

\begin{equation}
 \alpha_k=1-\sum_{j=1}^{k-1} \alpha_j\label{eq:alphak}
\end{equation}

\begin{figure}
   \centering
   \subfigure[Parameter Space]{\includegraphics[width = 2.5 in]{Figures/algo1.ps}}\qquad
   \subfigure[Function Space]{\includegraphics[width = 2.5 in]{Figures/algo2.ps}}\qquad
   \caption{\label{fig:algo}Various stages of our algorithm in (a) Parameter space - the solid lines indicate the practical stability boundary.
Points highlighted on the stability boundary are the decomposition
points. The dotted arrows indicate the convergence of the EM
algorithm. The dashed lines indicate the stability region phase.
$x_1$ and $x_2$ are the exit points on the practical stability
boundary (b) Different variables in the function space.
   }
 \end{figure}


\subsection{Our Algorithm}
\label{sec:algorithm}

Our framework consists mainly of two phases which are repeated in
the promising subspaces of the parameter search space. It is more
effective to use our algorithm at only these promising subspaces
which are usually obtained by stochastic global methods. The first
phase is the local phase (or the EM phase) where the promising
solutions are refined to the corresponding locally optimal parameter
set. The second phase which is the main contribution of this paper,
is the stability region phase, where the exit points are computed
and the neighborhood solutions are systematically explored through
these exit points. Fig. \ref{fig:algo} shows the different steps of
our algorithm both in (a) the parameter space and (b) the function
space.



This approach can be treated as a hybrid between global methods for
initialization and the EM algorithm which gives the local maxima.
One of the main advantages of our approach is that it searches the
parameter space more deterministically. This approach differs from
traditional local methods by computing multiple local solutions in
the neighborhood region. This also enhances user flexibility by
allowing the users to choose between different sets of good
clusterings. Though global methods give promising subspaces, it is
important to explore this subspace more thoroughly especially in
problems like parameter estimation. Algorithm \ref{nexttieralg}
describes our approach.


\begin{algorithm}
\caption{Stability Region based EM Algorithm} \label{nexttieralg}
\begin{algorithmic}
\STATE \textbf{Input:} Parameters $\Theta$, Data  $\mathcal{X}$,
tolerance $\tau$, Step $S_p$  \STATE \textbf{Output:}
$\widehat{\Theta}_{MLE} $  \STATE \textbf{Algorithm:}

\STATE Apply global method and store the q promising solutions $
\Theta_{init}=\{\Theta_1,\Theta_2,..,\Theta_q\}$ ~~~~~~~~ Initialize
E= $\phi$

\WHILE{$\Theta_{init} \neq \phi$} \STATE Choose $\Theta_i \in
\Theta_{init}$, set $\Theta_{init}= \Theta_{init} \backslash
\{\Theta_i\}$ \STATE $LM_i=EM(\Theta_i,\mathcal{X},\tau)$~~~~~~~~~
$E=E \cup \{LM_i\}$ \STATE Generate promising direction vectors
$d_j$ from $LM_i$

\FOR {each $d_j$} \STATE Compute Exit Point ($X_j$) along $d_j$
starting from $LM_i$ by evaluating the log-likelihood function given
by (\ref {eq:log})

\STATE $New_j=EM(X_j+\epsilon \cdot d_j,\mathcal{X},\tau)$
\IF{$new_j \notin E$} \STATE $E=E \cup New_j$ \ENDIF

\ENDFOR

   \ENDWHILE
\STATE $\widehat{\Theta}_{MLE} =max\{val(E_i)\}$

\end{algorithmic}
\end{algorithm}


In order to escape out of this local maximum, our method needs to
compute certain promising directions based on the local behaviour of
the function. One can realize that generating these promising
directions is one of the important aspects of our algorithm.
Surprisingly, choosing random directions to move out of the local
maximum works well for this problem. One might also use other
directions like eigenvectors of the Hessian or incorporate some
domain-specific knowledge (like information about priors,
approximate location of cluster means, user preferences on the final
clusters) depending on the application that they are working on and
the level of computational expense that they can afford. We used
random directions in our work because they are very cheap to
compute. Once the promising directions are generated, exit points
are computed along these directions. {\it Exit points} are points of
intersection between any given direction and the practical stability
boundary of that local maximum along that particular direction. If
the stability boundary is not encountered along a given direction,
it is very likely that one might not find any new local maximum in
that direction. With a new initial guess in the vicinity of the exit
points, EM algorithm is applied again to obtain a new local maximum.

\subsection{Implementation Details}
\label{sec:implementation}

Our program is implemented in MATLAB and runs on Pentium IV 2.8 GHz
machine. The main procedure implemented is $TT\_EM$ described in
Algorithm ~\ref{nexttier}. The algorithm takes the mixture data and
the initial set of parameters as input along with step size for
moving out and tolerance for convergence in the EM algorithm. It
returns the set of parameters that correspond to the Tier-1
neighboring local optimal solutions. The procedure $eval$ returns
the log-likelihood score given by (\ref{eq:log}). The $Gen\_Dir$
procedure generates promising directions from the local maxima. Exit
points are obtained along these generated directions. The procedure
$update$ moves the current parameter to the next parameter set along
a given $k^{th}$ direction $Dir[k]$. Some of the directions might
have one of the following two problems: (i) Exit points might not be
obtained in these directions. (ii) Even if the exit point is
obtained it might converge to a less promising solution. If the exit
points are not found along these directions, search will be
terminated after $Eval\_MAX$ number of evaluations. For all exit
points that are successfully found, $EM$ procedure is applied and
all the corresponding neighborhood set of parameters are stored in
the $Params[~]$ \footnote{To ensure that the new initial points are
in the different stability regions, one should move along the
directions `$\epsilon$' away from the exit points.}. Since,
different parameters will be of different range, care must be taken
while multiplying with the step sizes. It is important to use the
current estimates to get an approximation of the step size with
which one should move out along each parameter in the search space.
Finally, the solution with the highest likelihood score amongst the
original set of parameters and the Tier-1 solutions is returned.

\begin{algorithm}
\caption{Params[~] $TT\_EM(Pset,Data,Tol,Step)$} \label{nexttier}
\begin{algorithmic}
\STATE$Val=eval(Pset)$ \STATE $Dir[~]=Gen\_Dir (Pset)$ \STATE
$Eval\_MAX=500$

\FOR{$k=1$ to $size(Dir)$} \STATE $Params[k]= Pset~~~~~~ExtPt=OFF$
\STATE $Prev\_Val=Val~~~~~~~~~Cnt=0$

\WHILE{$(!~ExtPt)~ \&\& ~(Cnt<Eval\_MAX)$} \STATE
$Params[k]=update(Params[k],Dir[k],Step)$ \STATE $Cnt~=~Cnt~+~1$
\STATE $Next\_Val~=~eval(Params[k])$

\IF{$(Next\_Val~>~Prev\_Val)$} \STATE $ExtPt=ON$ \ENDIF

\STATE $Prev\_Val=Next\_Val$
    \ENDWHILE
\IF{$count<Eval\_MAX$}
    \STATE $Params[k]=update(Params[k],Dir[k],ASC)$
\STATE $Params[k]=EM(Params[k],Data,Tol)$ \ELSE \STATE
$Params[k]=NULL$ \ENDIF \ENDFOR \STATE \bf Return
$max(eval(Params[~]))$
\end{algorithmic}
\end{algorithm}


\begin{figure*}[htp]
   \centering
   \subfigure[]{\includegraphics[width = 1.0 in]{Figures/init3.ps}}\qquad
   \subfigure[]{\includegraphics[width = 1.0 in]{Figures/initial3.ps}}\qquad
   \subfigure[]{\includegraphics[width = 1.0 in]{Figures/extpt3.ps}}\qquad
   \subfigure[]{\includegraphics[width = 1.0 in]{Figures/final3.ps}}\qquad
   \caption{\label{fig:diagcov}Parameter estimates at various
   stages of our algorithm on the three component Gaussian mixture
   model (a) Poor random initial guess (b) Local maximum
   obtained after applying EM algorithm with the poor initial
   guess (c) Exit point obtained by our algorithm (d) The final
   solution obtained by applying the EM algorithm to the initial
   point in the neighboring stability region.
   }
 \end{figure*}
\subsection{Results and Discussion}
\label{sec:results}

Our algorithm has been tested on both synthetic and real datasets.
The initial values for the centers and the covariances were chosen
uniformly random. Uniform priors were chosen for initializing the
components. For real datasets, the centers were chosen randomly from
the sample points.

\begin{figure}[htp]
\centerline{
  \epsfig{figure=Figures/SREM1.ps, width=2.9in}
} \caption{Graph showing likelihood vs Evaluations. A corresponds to
the original local maximum (L=-3235.0). B corresponds to the exit
point (L=-3676.1). C corresponds to the new initial point in the
neighboring stability region (L=-3657.3) after moving out by
`$\epsilon$'. D corresponds to the new local maximum (L=-3078.7).}
\label{fig:eval}
\end{figure}

\subsubsection{Synthetic Datasets}
A simple synthetic data with 40 samples and 5 spherical Gaussian
components was generated and tested with our algorithm. Priors were
uniform and the standard deviation was 0.01. The centers for the
five components are given as follows: $\mu_1=[0.3~0.3]^T$,
$\mu_2=[0.5~0.5]^T$, $\mu_3=[0.7~0.7]^T$, $\mu_4=[0.3~0.7]^T$ and
$\mu_5=[0.7~0.3]^T$.

The second dataset was that of a diagonal covariance case containing
$n=900$ data points. The data generated from a two-dimensional,
three-component Gaussian mixture distribution with mean vectors at
$[0 ~-2]^T, [0~ 0]^T,[0 ~2]^T$ and same diagonal covariance matrix
with values 2 and 0.2 along the diagonal \cite{Ueda98}. All the
three mixtures have uniform priors. Fig. \ref{fig:diagcov} shows
various stages of our algorithm and demonstrates how the clusters
obtained from existing algorithms are improved using our algorithm.
The initial clusters obtained are of low quality because of the poor
initial set of parameters. Our algorithm takes these clusters and
applies the stability region step and the EM step simultaneously to
obtain the final result. Fig. \ref{fig:eval} shows the value of the
log-likelihood during the stability region phase and the EM
iterations.


In the third synthetic dataset, a more complicated overlapping
Gaussian mixtures are considered \cite{Figueiredo02}. The parameters
are as follows: $\mu_1=\mu_2=[-4~ -4]^T$ , $\mu_3 =[2~2]^T$ and
$\mu_4=[-1~-6]^T$. $\alpha_1=\alpha_2=\alpha_3=0.3$ and
$\alpha_4=0.1$.
\begin{displaymath}
     \Sigma_1=\left[ \begin{array}{cc} 1 &0.5\\  0.5 & 1 \end{array}
     \right]~~~~~~~~~~~~~~~\Sigma_2=\left[ \begin{array}{cc} 6 &-2\\  -2 & 6 \end{array}
     \right]
 \end{displaymath}
\begin{displaymath}
    \Sigma_3=\left[ \begin{array}{cc} 2 &-1\\  -1 & 2 \end{array}
     \right]~~~~~~~~~~~~~~~ \Sigma_4=\left[ \begin{array}{cc} 0.125 &0\\  0 &0.125  \end{array}
     \right]
 \end{displaymath}


\begin{table*}[htp]
\begin{tiny}
\centering \caption{\protect\small Performance of our algorithm on
an average of 100 runs on various synthetic and real datasets}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dataset &Samples & Clusters & Features &  EM (mean $\pm$ std) & SREM (mean $\pm$ std)\\
\hline Spherical & 40& 5 & 2  & 38.07$\pm$2.12 & 43.55$\pm$0.6 \\
\hline Elliptical & 900& 3 & 2  &  -3235$\pm$0.34 & -3078.7$\pm$0.03 \\
\hline Full covariance 1& 500& 4 & 2  & -2345.5 $\pm$175.13 & -2121.9$\pm$ 21.16 \\
\hline Full covariance 2& 2000& 4 & 2  & -9309.9 $\pm$694.74 & -8609.7 $\pm$37.02 \\
\hline Iris & 150& 3 & 4  & -198.13$\pm$27.25 &-173.63$\pm$11.72\\
\hline Wine & 178& 3 & 13  & -1652.7$\pm$1342.1& -1618.3$\pm$1349.9\\
\hline
\end{tabular}
\end{center}
\end{tiny}
\label{TB:results}
\end{table*}

\subsubsection{Real Datasets}
Two real datasets obtained from the UCI Machine Learning repository
\cite{Blake98} were also used for testing the performance of our
algorithm. Most widely used Iris data with 150 samples, 3 classes
and 4 features was used. Wine data set with 178 samples was also
used for testing. Wine data had 3 classes and 13 features. For these
real data sets, the class labels were deleted thus treating it as
unsupervised learning problem. Table~\ref{TB:results} summarizes our
results over 100 runs. The mean and the standard deviations of the
log-likelihood values are reported. The traditional EM algorithm
with random starts is compared against our algorithm on both
synthetic and real data sets. Our algorithm not only obtains higher
likelihood value but also produces it with high confidence. The low
standard deviation of our results indicates the robustness of
obtaining the global maximum. In the case of the wine data, the
improvements with our algorithm are not much significant compared to
the other datasets. This might be due to the fact that the dataset
might not have Gaussian components. Our method assumes that the
underlying distribution of the data is mixture of Gaussians.
Table~\ref{TB:compresults} gives the results of SREM
compared with other methods like split and merge EM and k-means+EM
proposed in the literature.



\begin{table}[htp]
\centering \caption{\protect\small Comparison of SREM with
other methods}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Method & Elliptical & Iris\\
\hline RS+EM & -3235 $\pm$ 14.2 & -198 $\pm$ 27\\
\hline K-Means+EM & -3195 $\pm$ 54&-186 $\pm$ 10\\
\hline SMEM &-3123 $\pm$ 54&-178.5 $\pm$ 6\\
\hline SREM &-3079 $\pm$ 0.03 &-173.6 $\pm$ 11\\
\hline
\end{tabular}
\end{center}
\label{TB:compresults}
\end{table}


\subsubsection{Discussion}
It will be effective to use our algorithm for those solutions that
appear to be promising. Due to the nature of the problem, it is very
likely that the nearby solutions surrounding the existing solution
will be more promising. One of the primary advantages of our method
is that it can be used along with other popular methods available
and improve the quality of the existing solutions. In clustering
problems, it is an added advantage to perform refinement of the
final clusters obtained. Most of the focus in the literature was on
new methods for initialization or new clustering techniques which
often do not take advantage of the existing results and completely
start the clustering procedure ``{\it from scratch}". Though shown
only for the case of multivariate Gaussian mixtures, our technique
can be effectively applied to any parametric finite mixture model.

Table \ref{TB:convresults} summarizes the average number of
iterations taken by the EM algorithm for the convergence to the
local optimal solution. We can see that the most promising solution
produced by our SREM algorithm converges much faster. In
other words, our method can effectively take advantage of the fact
that the convergence of the EM algorithm is much faster for high
quality solutions. This is an inherent property of the EM algorithm
when applied to the mixture modeling problem. We exploit this
property of the EM for improving the efficiency of our algorithm.
Hence, for obtaining the Tier-1 solutions using our algorithm, the
threshold for the number of iterations can be significantly lowered.

\begin{table}[htp]
\centering \caption{\protect\small Number of iterations taken for
the convergence of the best solution. }
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Dataset & Avg. no. of  & No. of iterations \\
 &iterations & for the best solution\\
\hline Spherical &126& 73\\
\hline Elliptical &174& 86\\
\hline Full covariance &292&173\\
\hline
\end{tabular}
\end{center}
\label{TB:convresults}
\end{table}

Our algorithm can be easily extended to other widely used EM
related problems like k-means clustering,training Hidden Markov Models, Mixture of Factor Analyzers, Probabilistic Principal
Component Analysis, Bayesian Networks etc. We would also like to
extend these techniques to Markov Chain Monte Carlo methods like
Gibbs sampling for the estimation of mixture models.

